Frisbee: automated testing of Cloud-native applications in Kubernetes

As more and more companies are migrating (or planning to migrate) from on-premise to Cloud, their focus is to find anomalies and deficits as early as possible in the development life cycle. We propose Frisbee, a declarative language and associated runtime components for testing cloud-native applications on top of Kubernetes. Given a template describing the system under test and a workflow describing the experiment, Frisbee automatically interfaces with Kubernetes to deploy the necessary software in containers, launch needed sidecars, execute the workflow steps, and perform automated checks for deviation from expected behavior. We evaluate Frisbee through a series of tests, to demonstrate its role in designing, and evaluating cloud-native applications; Frisbee helps in testing uncertainties at the level of application (e.g., dynamically changing request patterns), infrastructure (e.g., crashes, network partitions), and deployment (e.g., saturation points). Our findings have strong implications for the design, deployment, and evaluation of cloud applications. The most prominent is that: erroneous benchmark outputs can cause an apparent performance improvement, automated failover mechanisms may require interoperability with clients, and that a proper placement policy should also account for the clock frequency, not only the number of cores.

==> sections/4_runtime.tex <==
\subsection{Service Deployment}
Some examples include log or data change watchers, monitoring adapters, and so on. A log watcher, for example, can be built once by a different team and reused across different applications. Another example of a sidecar container is a file or data loader that generates data for the main container.

\paragraph{Throttling Agent}
cgroup is a Linux feature that measures how much of the specified resources a container has used in the current interval, and throttles it if it has reached the given quota. When a new interval starts, the cgroup renews the container runtime metrics. Regarding RAM, the process will get out-of-memory errors if it exceeds the memory limit set on the cgroup.  The kernel provides the cgroup interface through a pseudo-filesystem called cgroupfs (/sys/fs/cgroup). For example, /sys/fs/cgroup/CPU,cpuacct/* lets us control CPU allocation, where /sys/fs/cgroup/blkio lets us configure IO policies on block devices. A pod is practically a parent cgroup whose allocated resources are shared by the containers running within the Pod. 


\paragraph{Network Agent}
A network link agent, such as Linux tc-tool~\cite{10.5555/1639809.1639898}, applies the different user-defined network QoS rules by manipulating packets coming in or going out of the shared network interface in the Pod. When an application sends a packet to the network interface, the Linux kernel first places the packet into a queue managed by TC. The behavior of this queue is configurable via a mechanism called `Queueing Discipline' or `qdisc'.  Network Emulator (NetEM) is a special qdisc that can delay, drop, or duplicate a packet, as required to match the desired network characteristics, i.e., latency, packet loss, and bandwidth. Qdisc compares the packet against the filtering rules for every incoming or outgoing packet and forwards it to the appropriate queue. New policies are created dynamically, which allows us to create per network policies and update those policies at runtime.


\paragraph{Debugger Agent}
A debugger agent is a tool that allows developers to pause a program and inspect the state over the network. This agent relies on the cgroup freezer for pausing and resuming a service container~\cite{cgroupfreezer}. Sequences of SIGSTOP and SIGCONT are not always sufficient for stopping and resuming tasks in user-space. While SIGSTOP cannot be caught, blocked, or ignored, it can be seen by waiting or ptracing parent tasks. SIGCONT is especially unsuitable since the task can catch it. By adding the task PID in /sys/fs/cgroup/freezer/.../tasks, the cgroup prevents the task from accessing any resource, thus forcing it into a quiescent state. Once the tasks are frozen, another task can walk /proc or invoke a kernel interface to gather information about the frozen tasks.

%[ Add fault in the clusterbus to bring Redis into a halt ]



\subsection{Workflow Management}


%\subsection{Operators}


%One of the reasons that Kubernetes is the leading Container Orchestration platform today is because it has standardized the .  Human operators who look after specific applications and services have deep knowledge of how the system ought to behave, how to deploy it, and how to react if there are problems.

% More specifically, In the Kubernetes API, a resource is an endpoint that stores a collection of API objects of a certain kind.  The controller will typically run outside of the control plane, much like any containerized application.

% Previously this knowledge only resided in the minds of test engineers, various combinations of shell scripts or automation software like Jenkins. It was outside of your Kubernetes cluster and hard to integrate. The Workflow operator implement and automate common Day-1 (installation, configuration, etc) and Day-2 (re-configuration, update, backup, failover, restore, etc.) activities in a piece of software running inside your Kubernetes cluster, by integrating natively with Kubernetes concepts and APIs.

%A controller tracks at least one Kubernetes resource type. These objects have a spec field that represents the desired state. The controller(s) for that resource are responsible for making the current state come closer to that desired state.

%The controller might carry the action out itself; more commonly, in Kubernetes, a controller will send messages to the API server that have useful side effects. You'll see examples of this below.

%

%It's useful to have simple controllers rather than one, monolithic set of control loops that are interlinked. Controllers can fail, so Kubernetes is designed to allow for that.

%Built-in controllers manage state by interacting with the cluster API server.

%Due to the low computing overhead and fast instance spawning time, \frisbee{} uses containers as the execution environment for services. The container image is a packaged executable that contains the program and the complete runtime (e.g., Java, Python), with all configuration files and dependencies pre-installed. A container is a normal user-space process that runs in a sandboxed environment~\cite{rosen2013resource} with a virtual network stack, a restricted filesystem, a private process hierarchy, and specific CPU and memory limits. 

%Containers are powered by two Linux kernel features: namespaces and cgroups. Namespaces isolate and limit the visibility a container has over host OS entities such as process trees, network interfaces, user IDs, and filesystem mounts. Containers share the host resources through OS-level virtualization. By default, a container has no constraints and can use all the resources of the physical machine it runs on, potentially starving other processes from resources. In order to limit that, Linux has a feature called cgroups to control resource allocations and impose per-resource restrictions. In \frisbee{}, we use cgroups to enforce constraints on CPU, RAM, block I/O, and network I/O. 

 %The debugger incorporates a web interface for interactive interrogation of the Pod. 


%Pod startup

%Let’s take a look at an Istio service mesh example. An Envoy sidecar proxies all incoming and outgoing traffic to the application container. So until it’s up and running, the application may fail to send or receive traffic. Readiness probes don’t help if the application is trying to talk outbound. It’s not always a breaking issue, because the container will probably be able to recover, but you’ll probably see error messages in the logs, or CrashLoopBackoffs when the application container fails to start. In some cases when the application is not resilient enough of restarts, or some startup scripts are not idempotent, it may not start at all.

%This issue is quite easy to solve with an ugly workaround, by adding a few seconds delay in the application container’s startup script. It is the recommended solution by Istio as well, but as said in this issue it is more of a hack, and quite painful to change every developer container in the mesh.

%With the Kubernetes Sidecar feature, the pod startup lifecycle will be changed, so sidecar containers will start after init containers finished, and normal containers will only be started once the sidecars become ready. It ensures that sidecars are up and running before the main processes start.





%For controlled placement, Kubernetes provides multiple ways to constrain a Pod to only run on a particular set of node (s). 





==> sections/7_related.tex <==
Cloud testing can refer either to testing cloud-based systems (test of the cloud) or to leveraging the cloud for testing purposes (testing in the cloud): both approaches (and their combination into testing of the cloud in the cloud) have drawn research interest. 


 %cloud-native applications, in a reproducible, scalable, and standardized manner, before the actual deployment. 

One possibility is to run tests on real Cloud platforms, like AWS, Azure, or GCP. In this approach, the application is executed on real devices, and the result of its execution is then examined. Although desirable, experimentation in real testbeds is usually costly and provides few means of understanding how the application works.

Simulators like CloudSim~\cite{10.1002/spe.995}, and derivatives such as iFogSim~\cite{DBLP:journals/corr/GuptaDGB16}, IoTSim-Edge~\cite{jha2020iotsim}, and EdgeCloudSim~\cite{sonmez2018edgecloudsim}, have been proposed as a cost-effective way to evaluate placement strategies for independent application services on machines distributed across Cloud, Edge, and IoT environments. Though reproducible and convenient, simulators study behaviors expressed as mathematical models with certain assumptions. Hence, they are inadequate for evaluating real systems. 

Emulators incur similar infrastructure costs with simulators while achieving better realism since they run real codes. There are mainly two types of emulators: 1) Full-system emulators, such as ModelNet~\cite{vishwanath2009modelnet} and DieCast~\cite{gupta2011diecast}, which use VMs as hosts to emulate heterogeneous nodes with various OSes, and 2) Container-based emulators, such as FogBed~\cite{coutinho2018fogbed}, EmuFog~\cite{mayer2017emufog}, and EmuEdge~\cite{zeng2019emuedge}, which leverage containers that share a single OS kernel to provide better scalability, required to emulate large-scale networks.

These tools can simulate the communication between real application components. However, since they are immediate descendants of network emulators (e.g.,  MiniNet~\cite{de2014using}), they cannot manipulate application components or the underlying runtime infrastructure. D-Cloud~\cite{banzai2010d} is a software testing framework that uses virtual machines in the cloud for failure testing of distributed systems. However, D-Cloud does not allow users to control network properties such as the latency between two machines. MockFog~\cite{hasenburg2019mockfog} and Fogify~\cite{symeonides2020fogify}, provide resource throttling and network shaping, and have implemented ad-hoc alterations on a running testbed. However, all of these approaches are based on Docker Swarm, which does not support the sidecar pattern, or automated control loops. This means that the experiment orchestration would need to be done manually via the Fogify API, and would require containers with monitoring tools pre-installed.

CNSBench~\cite{merenstein2021cnsbench} has native support for orchestration of different control and I/O workload combinations at Kubernetes. Although it supports consistent initialization of multiple workloads in parallel, it lacks support for synchronizing the finish of each workload. Argo~\cite{argo}, a workflow engine for Kubernetes, is exactly the opposite. It can automatically start one container after another, but only if the previous container has finished. Moreover, Argo workflows are designed to bring jobs to completion. Argo does not support operations on a running job (such as killing a service). 

Chaos Engineering such as Chaos-Mesh~\cite{chaomesh} are excellent for injecting various faults into the system, but do not provide the means for assessing the impact of a fault. This task is usually left to third-party tools. Services meshes, like Istio~\cite{istio}, provide both fault injection and observability of the fault. Their scope, however, is limited to the network level. In contrast, \frisbee{} operators at the application. That involves a broader range of failures (e.g., kills, partitions, I/O) and application-level monitoring (e.g., number of ingested keys, replication errors, etc.).



==> sections/8_discussion.tex <==
Although availability benchmarks have been long discussed, there is no existing industry-wide benchmark. The reason is that they 

\textit{Ether} will be an invaluable asset for researchers who want to experiment with topologies or evaluate new algorithms. With today's practises,  researchers either have to use simulators or intervene into the source code of real-world systems. \textit{Ether} brings the best of the two worlds. Like a simulator, it stresses the given components, both in isolation and in comparison to others. Like a real-world system, it stresses the given components (or their combination thereof), under realistic conditions (e.g., on the target infrastructure). In this context, it can also be used to practically teach students how the design choices of a distributed storage systems can affect the application performance and behavior. Prospects are also visible in the industry, for reducing by orders of magnitude the time from conceptualization to the release of a new storage system.


%Implementing a test suite. This is the main focus of this blog post. The Kubernetes E2E framework is written in Go. It relies on Ginkgo for managing tests and Gomega for assertions. These tools support “behavior driven development”, which describes expected behavior in “specs”. In this blog post, “test” is used to reference an individual Ginkgo.It spec. Tests interact with the Kubernetes cluster using client-go.

%Besides that, a complete experimenting platform hypothesizes around defined steady states, performs dynamic actions that alter the runtime environment, monitors the effects of actions in the system, validate these effects  via test cases, and automates the testing. 

==> sections/background.tex <==
%Our study focuses on characterizing failure events within ourorganization’s set of data centers. We next give an overview of datacenter networks and workload characteristics.



\subsection{Classification of Systems and Tradeoffs}

\subsubsection{RAID}
A common approach to ensuring data availability has been through RAID-based architectures. Striping data across multiple drives can protect against the failure of one or two drives, but performance can fall dramatically during rebuild operations, which can have negative impacts on business operations. Years of data center experience shows that drive failures are usually not isolated incidents: when one drive in a RAID group fails, the likelihood of other group member failing increases. 

Simply protecting against a complete hard drive failure such as with RAID, does not protect against the gradual failure of the bits stored on magnetic media. An Unrecoverable Read Error during a rebuild operation means data is now permanently lost, which places your business at risk. A media failure such as bit rot, where a portion of the drive surface or other media becomes unreadable, corrupts data thus making it impossible to retrieve the data in its original unaltered form. 

Additionally, as drive capacities have greatly increased, so too have rebuild times. What formerly took minutes can now take hours, or even days. In addition, this requires replacement of the failed drive ASAP, be it weekends, holidays or the middle of the night.


\subsubsection{Replication: Latency versus durability}
Replication is used to improve system availability (by directing traffic to a replica after a failure), avoid data loss(by recovering lost data from a replica), and improve performance (by spreading load across multiple replicas and by making low-latency access available to users around the world). However, there are different approaches to replication.

Synchronous replication ensures that updates are synced to the disk of all replicating nodes before the system returns success to the user. To keep the replicas consistent, the server blocks waiting for replication to finish. By doing so, system performance is impacted when replication nodes suffer high pressure or network latency. Furthermore, availability may be impacted if synchronously replicated updates cannot complete while some replicas are offline. 

Asynchronous replication avoids high write latency (in particular, making it suitable for wide area replication) but allows replicas to be stale. The advantages are that avoiding disk greatly improves write latency, and potentially improves throughput (if multiple updates to the same replica can be serviced by a single I/O network operation or can be condensed in memory). The disadvantage is risk of data corruption because transactions might be committed to the primary database but not to the replicas -- if more than half of the replicating node crash, the system will lose unsynced updates.

Multi-Raft approached, like TIDB, support the coexistence of consistency and asynchronized replication by acknowledging the result of success once data are written to the majority replicas. While not all replicas are consistent at the same time, read consistency is still ensured by blocking incoming read operation until replication is complete. In this way, even though a few replicas might get lost, the system still has the latest data. This method is better suited when numerous replicas are required, or when inter-node communication is slow (as happen on geo-replication scenarios). 


\subsubsection{Erasure Coding}
Object storage achieves data availability through advanced erasure coding whereby data is combined with parity information and then sharded and distributed across the storage pool. Since only a subset of the shards are needed to rehydrate the data, there is no rebuild time or degraded performance, and failed storage components can be replaced when convenient.

The combination of widely distributed erasure coded data (say with an 18/8 coding policy) and data scrubbing technology that continuously validates the data written on the media can enable you to achieve 15 nines of data durability. In simpler terms: for every 1,000 trillion objects, only one would not be readable. How’s that for data durability? It’s not surprising that hyperscale data centers and cloud services providers use object-based storage to meet the needs for the highest data availability and data durability.

 % Single-source, Multi-source replication


\subsubsection{Data Layout: Row versus Columns}
Efficient data access relies on "locality," which means putting all the data to access as close together as possible. By doing so, you avoid extra seek and cache inefficiency. Row and columnar formats, despite the factors of encoding and compression, essentially are about providing suitable on disk locality for different access patterns. However, the differences are not significant in memory.

In row-based storage all of a record’s fields are stored contiguously on disk. Row-based storage supports efficient access to an entire record (including low latency reads and insertion/update in a serving-oriented system), and is ideal if we typically access a few records in their entirety. Online transaction processing (OLTP) systems usually use row-oriented storage, like InnoDB and RocksDB.

Column-based storage puts fields of record in separate columns, making access to a subset of fields more efficient, particularly when the fields of multiple records are accessed. Online analytical processing (OLAP) systems and batch systems are typically based on column-oriented storage [Snowflake, BigQuery, or Redshift]. 




\subsubsection{Data sharding}
Different partitions can be placed on different nodes, and thus a large dataset can be distributed across many disks, and the query load can be distributed across many processors. 
One way of partitioning is to assign a continuous range of hashes of keys to each partition. The partition boundaries can be evenly spaced, or they can be chosen by some kind of algorithm like consistent hashing. Due to the hash, keys can be distributed fairly among the partitions, effectively reducing hot spots, though not totally avoiding them. Unfortunately, this method fails to do efficient range queries, compared to partitioning by key range.

The other way of partitioning is to assign a continuous range of keys to each partition. It needs to record the boundaries between the ranges to determine which partition contains a given key, and then requests can be sent to the appropriate node. One key feature of key range partition is that it is friendly to range scans. Meanwhile, for the split or merge of partitions, only meta-information about the range of a partition need to be changed, which avoids moving actual data in a large extent. However, the downside of the sorted order is that sequential reads and writes can lead to hot spots -- high load may end up on one partition but leave the other nodes idle. 


% Re-sharding

%Placement Driver (PD) server is a metadata cluster powered by etcd that manages and schedules TiKV.



\subsubsection{Architecture: Coprocessing versus Disaggregation}

TiDB pushes some data computation logic to TiKV Coprocessor. TiKV Coprocessor processes the computation for each Region. Each request sent to TiKV Coprocessor only involves the data of one Region.

TiFlash shares the computing workload in the same way as the TiKV Coprocessor does: TiDB pushes down the computing that can be completed in the storage layer. Whether the computing can be pushed down depends on the support of TiFlash. For details, see Supported pushdown calculations.





\subsubsection{Index: Global versus local}


\subsubsection{API: System calls, RPC, REST}





 
\subsubsection{Write versus Read}
If you need to update a row, the engine needs to achieve dedupe as fast as possible. It doesn't matter if the dedupe happens on writes or reads. Most analytical databases or Hadoop drop the support for it and in turn gain higher loading and reading performance. 


\subsubsection{Disk versus Filesystems versus Storage Engine}
\begin{itemize}
    \item Perform I/O directly to the block device
    \item Perform I/O to the filesystem
    \item Perform I/O through intermediate engine (e.g, rocksdb)
    \item Combinations (e.g, write logs used for the Raft consensus algorithm to a different location than data)
    \item block-oriented execution engine
\end{itemize}







\subsection{Multiple services on each pod}
We found that the traditional method of deploying a Redis database over Kubernetes, in which each Pod includes only a single Redis instance while preserving a dedicated CPU, is notably inefficient. Redis is exceptionally fast and in many cases can use just a fraction of the CPU resources to deliver the requested throughput. Furthermore, when running a Redis Cluster with multiple Redis Enterprise instances across multiple Pods, the Kubernetes network, with its multiple vSwitches, can quickly become the deployment’s bottleneck. Therefore, Redis took a different approach to managing Redis over the Kubernetes environment. Deploying multiple Redis database instances on a single Pod allows us to better utilize the hardware resources used by the Pod such as CPU, memory, and network while keeping the same level of isolation.

... Topology Details Matter ...

Collocated in a Pod: 

Collocated in a Server: 

Distributed across the Network: 

Narrow: 
    Lower partition risk
    Lower availability blast radius

Wider:
    More redundancy
    more bisection bandwidth -> durability (faster replication_
    more placement options



% https://www.mirantis.com/blog/multi-container-pods-and-container-communication-in-kubernetes/

########################## CLUSTER DOCKER/NAT support  ########################

# In certain deployments, Redis Cluster nodes address discovery fails, because
# addresses are NAT-ted or because ports are forwarded (the typical case is
# Docker and other containers).
#
# In order to make Redis Cluster working in such environments, a static
# configuration where each node knows its public address is needed. The
# following two options are used for this scope, and are:
#
# * cluster-announce-ip
# * cluster-announce-port
# * cluster-announce-bus-port
#
# Each instruct the node about its address, client port, and cluster message
# bus port. The information is then published in the header of the bus packets
# so that other nodes will be able to correctly map the address of the node
# publishing the information.
#
# If the above options are not used, the normal Redis Cluster auto-detection
# will be used instead.
#

#
# Example:
#
# cluster-announce-ip 10.1.1.5
# cluster-announce-port 6379
# cluster-announce-bus-port 6380

\subsection{Enterprise-like functionalities on community versions}
Auto resharding is only supported on Redis Enterprise. This includes resharding, shard migration, and setting up triggers for auto-balancing without impacting your application. If you are running on the Redis Community version, then you need to perform the maintenance operations manually. In this experiment, we use \frisbee{} to enable Auto resharding on the community version. We automate the aforementioned process by gradually increasing request load, 

%NDBench performs an exponential backoff algorithm and steps down the load based on preset % of SLA violation. This is needed because in some scenarios the data stores may be only slightly overloaded and may have passed the threshold at which they can continue to operate within SLA.

%https://severalnines.com/database-blog/hash-slot-resharding-and-rebalancing-redis-cluster


potential limitation of the current approach is that it conceals the relationship between a fault and a failure. For example, a fault in the disk is expected to cause an I/O failure but not a network failure.  We are currently working on a mechanism that will allow us to express both the presence and the type of an expected failure.  

%\subsection{Migrate clients to other domains}
%For example, when an AWS region is experiencing an outage, large numbers of
%clients simultaneously failover to other regions. 


\subsection{Redis Auto-scaling}
https://medium.com/swlh/scaling-redis-cluster-via-kubernetes-horizontal-pod-autoscaler-852541c01b29

%
%One of the plugins that NDBench support is AWS’s Dy-
%namoDB. DynamoDB works based on a provisioned capacity
%model and has an integrated auto-scaling feature. Auto-scaling
%%helps with automating the capacity management for the tables
%and global secondary indexes. In DynamoDB, the user can set
%the desired target utilization and the system will adjust the
%provisioned capacity accordingly. As part of our evaluation of
%different use cases we wanted to be mindful of how we design
%some of microservices that use DynamoDB as their data store.
%More specifically, we wanted to test how fast a table can be
%scaled up (or down) and whether we are going to see any
%server-side issues if we ramp up the traffic while the service
%is running. In our experiments we used 100,000 Writes Per
%Second and increased the write load to 200,000 Writes Per
%Second without pre-splitting the partitions, hence forcing the
%worst case behavior. NDBench allowed us to see how the auto-
%scaling worked in DynamoDB. We observed that auto-scaling
%was very efficient and in most cases would complete in a few
%minutes to seconds and with a worst case scenario about 1h
%as shown with the red arrow in Fig


%Auto-tuning
%At Netflix, each microservice generates different types of
%loads and the load is not always known before we create
%the data store cluster. Hence, we had to advise our engineers
%about the size of the cluster and the scalability limitations -
%for example in Cassandra we double our clusters if we want to
%scale horizontally to achieve equal distribution of the traffic.
%At the same time, we do not want to overspend by creating
%artificially large clusters.




%For example:
%\begin{enumerate}[label=(\roman*)]
%    \item We may want to \textbf{assign} Redis masters on machines with %high-capacity memory and SSDs.
%    \item We may want to \textbf{collocate} dependent services (e.g., a web server %and the Redis cache) to reduce the network latency among them.
%    \item 
%    \item We may want to \textbf{migrate} one server from one region to another to %simulate mobility scenarios
%\end{enumerate}



%The other and more important observation is that the aggregated average for the two cases (with/without failover) is almost identical. 

%However, it does not explain why the average in the two plots is identical. Moreover, there is another paradox. 



, but the conditions for alerting are different for each monitor.

Or maybe you've written a monitoring framework which is capable of gathering a bunch of metrics, then evaluating a few expressions to see if any metrics should be alerted upon



Or maybe you've written a monitoring framework which is capable of gathering a bunch of metrics, then evaluating a few expressions to see if any metrics should be alerted upon, but the conditions for alerting are different for each monitor.




\CHECKnote{
* The oracle is intended to catch events from immediate children of the workflow. That is, from the controllers, not from the services. This is because the semantics may change from controller to controller. The controller can implement its own test oracles. 
}

To achieve that, we expose assertions to the user that drive the conditional execution of the fail path. 



, but the conditions for alerting are different for each monitor.

Or maybe you've written a monitoring framework which is capable of gathering a bunch of metrics, then evaluating a few expressions to see if any metrics should be alerted upon



Or maybe you've written a monitoring framework which is capable of gathering a bunch of metrics, then evaluating a few expressions to see if any metrics should be alerted upon, but the conditions for alerting are different for each monitor.





Thus, it seems that Model Driven Engineering (MDE), and Model-Based Testing (MBT) would
be great choices to support the testing of cloud-native applications. 


However, CPS on IoT Cloud infrastructures demand us to man-
age 

https://dl.acm.org/doi/pdf/10.1145/3107091.31070939

We can use MDE to describe CPS elements and their potential uncertainties with formal models [15] to support most engineering activities, from requirement specification
to runtime analyses [4]. In this context, MDE techniques enable systematically mappings among modeling language concepts to support automatic integration.
However, for testing uncertainties of CPS in IoT Cloud infrastruc-
tures, it is not a straightforward engineering process from modeling
to code transformation, to test generation and execution. Various ac-
tivities need to deal with the elasticity, pay-per-use, on-demand pro-
visioning characteristics of IoT Cloud infrastructures and software
deployed atop such infrastructures. IoT and Cloud infrastructures
and technologies have introduced a lot of techniques for elastic
provisioning and execution of software components [1, 9]. During
the execution of applications in IoT Cloud infrastructures, many
operations can be performed dynamically but current MDE tools
have not supported well such elastic operations.


Puppet, for instance, is declarative: the sysadmin describes a desired end state and the tool attempts to reach it. Its domain-specific-language (DSL) is used for creating high-level descriptions of desired server state, as opposed to instructions and actions to be carried out.

by providing models abstracting possible configurations of IoT
and Cloud infrastructural elements and their possible dynamic
properties and uncertainties.

Model-based testing allows to generate a high number of test cases to be executed on the
cloud starting from an abstraction of the SUT. Different model-based testing frameworks have
been developed [12, 81, 82, 98], such as AUTOMATIC, which derives many different QoS config-
urations to be tested in the cloud [12]; and ATCloud, which generates test cases based on API
models [154]; or the proposal of Reference [82], which specifically addresses functional testing for
composed services. MIDAS [58] is a model-based scalable testing platform leveraging a Domain
Specific Language (DSL) based on the Unified Modeling Language (UML) and the UML Testing
Profile (UTP). EvoDroid [99] is another model-based framework that analyzes the source code of
an app and automatically extracts both a behavioral model and the APIs of externally referred
apps. EvoDroid then exploits these models to automatically generate the tests that are executed
concurrently in the cloud on several Android emulators.


Model-based testing allows to generate a high number of test cases to be executed on cloud starting from an abstration of teh SUT. 

Frameworks for declarative specifications exist (e.g, Pip~\cite{269028} P2Monitor~\cite{Singh06usingqueries}). P2 Monitor only works if the target system is written in the same language. Pip facilitates declarative checks, but a check is still written in over 40 lines on average. Also, there systems are not integrated with a failure service, and thus cannot thorough simulate abnormal operating conditions/ 

Overall, most existing work use approaches that could result in big implementations of the specifications. Managing hundreds of them becomes complicated, and they must also evolve as the system evolves. In practise, developers are reluctant to invest in writing detailed specifications~\cite{10.1145/1755913.1755937}, and hence the number of written specifications is typically small.



Pip classifies system behaviors as valid or invalid,
groups behaviors into sets that can be reasoned about,
and presents overall behavior in several forms suited to
discovering or verifying the correctness of system behav-
ior.

Bugs in distributed systems can affect structure, per-
formance, or both. A structural bug results in process-
ing or communication happening at the wrong place or
in the wrong order. A performance bug results in pro-
cessing taking too much or too little of any important
resource. For example, a request that takes too long may
indicate a bottleneck, while a request that finishes too
quickly may indicate truncated processing or some other
error. 

Bugs in distributed systems are often hard to find.
 We present Pip1, an infrastructure for comparing
actual behavior and expected behavior to expose struc-
tural errors and performance problems in distributed sys-
tems. Pip allows programmers to express, in a declara-
tive language, expectations about the system’s communi-
cations structure, timing, and resource consumption. Pip
includes system instrumentation and annotation tools to
log actual system behavior, and visualization and query
tools for exploring expected and unexpected behavior2.
Pip allows a developer to quickly understand and debug
both familiar and unfamiliar systems.





In the last years it has been a rise of software model checkers for distributed systems [CITE]. Model checkers work by exercising all possible sequences of events (e.g, different reordering of messages), and hereby pushing the target system into corner-case situations and unearthing hard-to-find bugs. This way, model checkers can express not only `invariant-like' specifications (i.e, check the state of the state), but also the events that to that state. However, these tools adhere white-box principle, thus requiring access to the source code. 



Finally, fsck can express
only “invariant-like” specifications (i.e., it only checks
the state of the file system, but not the events that lead
to the state). As we will see later, specifying recovery
requires “behavioral” specifications.

To scale dmck, we introduce semantic-aware model checking (SAMC), a white-box principle that takes simple semantic information of the target system and incorporates that knowledge into state-space reduction policies

Thelastfiveyearshaveseenariseofsoftware
modelcheckerstargetedfordistributedsystems[22,25,
43,50,51];forbrevity,wecategorizesuchsystemsas
dmck(distributedsystemmodelchecker).Dmckworks
byexercisingallpossiblesequencesofevents(e.g.,dif-
ferentreorderingsofmessages),andherebypushingthe
targetsystemintocorner-casesituationsandunearthing
hard-to-findbugs

A practical language to describe the expected behavior of the cloud-native application under dynamically changing operating conditions.

Dealing with the description of the testing lifecycle is where the main complexity lies. 

Some of them define common process steps, e.g., selecting the types of testing to be executed, executing the test scripts and reporting the test results [153], whereas others define specific steps for cloud based parallel test execution [92], such as specifying the test jobs and test deadlines, determining the number of virtual machines, computing test time/cost, partitioning of tasks based on the specified strategy and merging of test results. 





With existing approaches, specifications are cumbersome and difficult to write, and thus present a barrier to usage in practice [CITE]. Moreover, they are commonly implemented within the scope of a language-specific framework, thus providing limited coverage to multi-language applications.




 Argo~\cite{argo}, a workflow engine for Kubernetes, is exactly the opposite. It can automatically start one container after another, but only if the previous container has finished. Moreover, Argo workflows are designed to bring jobs to completion. Argo does not support operations on a running job (such as killing a service). 




\CHECKnote{AC: Testing cloud-native applications may involve complicated processes, that can not be implemented manually: First, ...}
When it comes to testing cloud-native applications, things become complex in comparison to the manual approach that engineers used to take to test other applications (e.g., the monolithic ones):



Different proposals focus on the specification of cloud-based testing processes. 




%    Argo also lets you add conditions, loops, and directed acyclic graphs (DAGs) in the pipeline.
    
%The templates called from a DAG or steps template can themselves be DAG or steps templates. This can allow for complex workflows to be split into manageable pieces.

%The DAG logic has a built-in fail fast feature to stop scheduling new steps, as soon as it detects that one of the DAG nodes is failed. Then it waits until all DAG nodes are completed before failing the DAG itself. The FailFast flag default is true, if set to false, it will allow a DAG to run all branches of the DAG to completion (either success or failure), regardless of the failed outcomes of branches in the DAG.


%These CRDs, and their relationship to other CRDs can define their lifecycle and trigger their implementation. 

%Before anything else, the controller performs the validation of the submitted description to detect misconfigurations. If there are no violations, the controller Instead of using annotations, you could store this type of information in an external database or directory, but that would make it much harder to produce shared client libraries and tools for deployment, management, introspection, and the like

%The controller then handles the \textbf{environment preparation}. 

%If the preparation is successful, the Workflow controller executes the workflow steps.

%Run CI/CD pipelines natively on Kubernetes without configuring complex software development products.


%To summarize, workflow specs are composed of a set of Argo templates where each template consists of an optional input section, an optional output section and either a container invocation or a list of steps where each step invokes another template.

%Other operational workflows such as Scale, Heal, Upgrade, Maintenance and others query the graph described by the template, query the service state, then execute a specific set of operations based on the graph and the context in which the workflow is executed. Interaction with the graph can read information and modify the service state.


%it allows users to express their interest in important events passed to the respective controllers, which decide what to do with it. 

% Events enable cont interacting with the workflow graph and discovery of relationships and state of objects. Additionally, events 


%The service state enables interacting with the service graph and discovery of relationships and state of components and services. Additionally, the service state allows passing 




-- API 




Wang et al. proposed Weevil [18] a tool for automating
experimentations over distributed testbeds. Weevil does not
specifically target cloud environments, but has a strong fo-
cus on managing the distributed aspects of experimentation,
and has a noticeable expressive power and flexibility. This
increases applicability of the tool, but also forces testers to
undergo a steep learning curve, complex setups and difficult
test maintenance. We gained experience with Weevil in our
previous research [10], [17]. Compared to Weevil, we support
a more focused, yet simpler, approach for test automation.



existing work on automated testing of infrastructure deployment and configuration [13] . Moreover, a number of testing approaches for domain-specific cloud applications are related to our work, for instance testing of elastic platforms for event stream processing [12], [14


elasticity of cloud-based systems, which
mainly deals with system testing, therefore, here we generally
do not consider tools for automated software testing in the
cloud, like, e.g., Cloud9 [4], that exploit the extensive resource
availability of clouds to parallelize/distribute software tests


%Second, we need to distinguish expected from unexpected failures. For example, to trigger the recovery actions of SUT we need to kill some of its services. If we model actions based on individual services, then the edge's assertion will fail as soon as we kill the service -- thus leading to the termination of the experiment. If we tolerate individually failing services, it is difficult to describe the number of failures we can tolerate in the graph. 




%The workflow controller handles the deployment of the modeled environment over Kubernetes, orchestrates the concurrent run of the constituent services, and undertakes actions that influence the running topology as specified in the workflow specification.

%By separating the scenario from the instrumentation code, \frisbee{} models are constructed early in the development cycle, which allows testing activities to start before the coding phase. 




% -- TiC 




% -- ToC 

These studies span from techniques to derive test cases from a formal specification, to automation tools  configure the testing environment, 

 Cloud testing tools and services are presented in several papers. AUToCLES is a Testing-As-A-Service tool of cloud-based elastic systems: given a JOpera specification of the SUT and a set of test cases defined using JMeter, AUToCLES instatiates the SUT, configures the testing environment, generates test input data, and executed the test cases.




% -- ToiC 





 


thus papers belonging to this category aim at checking the provided automatic cloud-based
functional services, as well as at validating their.




% Among others, define placement strategies in a more granular fashion than regions, to facilitate the injection of faults at the level of infrastructure, to automate the end-to-end monitoring of the system under evaluation, and to guarantee portability across various implementations. The same scenario designed on a workstation (e.g., microk8s, kubeedge), can be validated on an on-premise cluster (e.g., baremetal), and then run into Cloud-scale via Kubernetes-as-a-service (e.g., Azure Kubernetes). 



This view puts our development ecosystem in a unique position, as it has the characteristics necessary to be adapted to tailored-made solutions. The goal for our ecosystem is to become a catalyst to accelerate research in storage systems, by first simplifying the systems development.



account for the asynchrony between the service components and environments

it will be difficult to execute and run the comparatively larger End-to-End Tests for the Cloud-Native applications since it will involve testing every moving part of the Microservices architecture, will be slow, sometimes quite flaky, have to account for the asynchrony between the service components and environments,  

Even with Cloud provided resources, the remaining work can still be demanding for the system evaluator 



To the best of our knowledge, we re the first to address this in a more systematic way than ad-hoc approaches. 



\paragraph{Meeting the Chaos}


 


%Addressing these issues in production can be highly expensive, and we should try to solve them as early as possible in the development life cycle~\cite{abedi2017conducting,cavalli2015survey}.


\paragraph{Our Approach} 
We present \frisbee{}, a declarative language and associated runtime components for testing cloud-native applications on top of Kubernetes. 



%native experiment orchestration & scheduling

% This way, testing engineers and programmers can work independently, after having specified the experiment's workflow, free from the tedious tasks of writing scripts and selecting from a vast ecosystem of Kubernetes extensions. 





%To move tests earlier in the development lifecycle, we need an an environment not only  VV&T activities, but also to carry out empirical studies to evaluate the cost and benefits of new technologies.


%Adhoc approaches may work, but they take time to implement, time for users to learn, and induce technical debt as requirements change.
%

% Test design
% Test execution
% Test evaluation

%Elasticity
%testing in turn may have different objectives such as: to control different behaviors, to identify
%the resources to be (un)allocated, to coordinate events in parallel [8, 9], and of course to target
%scalability [17, 30, 40, 91].
%Reliability testing focuses on the observation of the system under test under the operational
%usage profile. Proposals focus on measuring the reliability level [59] or on achieving a specific
%reliability value also through API testing [39, 99, 154]




There is a lack of unified measuring approach of software portability in most computing platforms. This paper presents preliminary results of a systematic literature review, conducted to collect evidence on measuring software portability.


%focus is to design, build, and deploy applications that can capitalize on scalable Cloud infrastructures and technologies. However, to fully utilize these benefits, a new form of application development is needed. 


%\CHECKnote{Finding issues in production can be highly expensive and we should try to find them }

%Given specifications of the test suite and the system under test, AUToCLES implements testing as a service (TaaS): It automatically instantiates the SUT, configures the testing scaffoldings, and automatically executes test suites.



% We find numerous insights that warrant rethinking how we evaluate our applications. 


 %Our findings have strong implications for the design of file systems and applications 

% The \frisbee{} source code, the tests, and the scripts we used for conducting the experiments of this paper are available as open-source.



%Given Precondition

%When Action

%Then Result

To address this question, we present two advancements in the current state-of-the-art testing. 

Two arduous development tasks which inspired the evolution toward Kubernetes were setting up container clustering across multiple networks and automating deployment. A detailed list of services was scripted in-house, ad hoc, and at significant expense



There is an ongoing need to push testing functionality toward the earlier phases of development so that serious issues are identified and resolved before we push to production



For example, performance benchmarks are improved to serve dynamically changing request patterns, and testing in the cloud (TiC) approaches overcomes the limits of traditional testing approaches, allowing us 






CNSBench~\cite{merenstein2021cnsbench} has native support for orchestration of different control and I/O workload combinations at Kubernetes. Although it supports consistent initialization of multiple workloads in parallel, it lacks support for synchronizing the finish of each workload.


The problem is every aspect requires a different set of capabilities. Placement policies require interaction with the placement scheduler, runtime uncertainties require orchestrating events that alter the system under test (SUT), and abnormal conditions require fault-injection at the level of infrastructure.






However, the effort of developing a supporting tool is fairly high. 


In the Academy, the aim of producing a full-featured tool can hardly be afforded and must often be abandoned in favor of more modest goals.


In general, proof-of-concepts tools are developed. Besides the cost of development, one of the main setbacks is the exploratory aspect of a proof-of-concept tool. Sometimes, the kind of empirical insight provided by the tool is what is necessary to make fine-tuning adjustments in the theory.  In this context, proof-of-concept tools are very important, aiding the conduction of case studies and experiments





, is inaccurate. In order to foster the transfer of some new technology to industry, it is necessary to provide evidences that the new technology brings substantial, significant benefits over the current practices, if any.
With existing approaches, all these tasks are left to the system evaluator, and their implementation 






This approach aims to pinpoint bottlenecks arising from complex placement strategies, evaluate adaptation to runtime uncertainties that occur naturally to an Internet-facing system, such as dynamically changing request patterns, or conditions that only manifest under high load~\cite{mogul2006emergent}.

\CHECKnote{CONTINUE}

In this approach, the application is executed on real devices, and the result of its execution is then examined. Although desirable, experimentation in real testbeds is usually costly and provides few means of understanding how the application works.
 
 
 
 
 use synthetic load testing and analyze production metrics and look for outliers to help identify bottlenecks. 

More specifically, we set alerts so that 



Utilizing synthetic load testing enables engineers to test specific scenarios and identify potential bottlenecks, although this only covers contrived situations. In our approach, we combine synthetic load testing 

most cases, it is better to analyze production metrics and look for outliers to help identify trouble on the horizon.




The need for monitoring is well understood, so traditional monitoring solutions cover the traditional stack:

- application performance monitoring instruments your custom code to identify and pinpoint bottlenecks or errors
- infrastructure monitoring collects metrics about the host, such as CPU load and available memory




%systems intended for deployment in 
%For example, blocking mechanisms may cause the underutilization of available resources, thus increasing TCO proportionally to the number of affected resources. On the other hand, TCO may soar for systems with great write/read amplification factor, or chatty network protocols, that leads to overutilization of resources. 

%Events generally contain both a full runtime.Object that caused the event, as well as a direct handle to that object's metadata. This saves a lot of typecasting in code that works with Events.




 the condition in which, 

Once identified the bottleneck may be remedied bringing performance levels into an acceptable range. Remedies may include any number of optimizations but usually result in refactoring, caching and data optimization, threading and/or workload distribution. 












Therefore, it is crucial for testers to adopt a structured way for writing automated tests quickly and concisely.


Creating tests manually has several disadvantages, as pointed by different authors[CITE]. 

This is because Cloud-Native applications , and there are failure modes that are difficult to anticipate and trace. 


Cloud-native applications have the added challenge of never knowing just why kind of resources you are dealing with. There might be a particularly high load on your provider or you might have to deal with a proverbial “noisy neighbor.”




it is difficult to write a test case to verify that a program is correct in the face of 


done against known quantity of server resources. 


Second, the increased complexity of cloud applications implies numerous input combinations resulting in distinct system outputs, 


This, most manual tests cannot control network non-determinism; 



Moreover, 

% associate defects with root causes in distributed systems
% It can eliminate conflicts between developers and testers


Unfortunately, testing these applications is a challenging and multidisciplinary activity. We need several tools for modeling, deployment, control, and analytics to test and evaluate uncertainties that may occur through a system's lifecycle. 


 Cloud-native applications
 with several fault domains. Moreover, 

expose new fault domains and create the need for managing more highly fragmented services.

each part of the application is packaged in its own container, dynamically , and microservices-oriented to increase the overall agility and maintainability of applications. 


Traditionally, application development has been about building static and monolithic systems. Many developers are in the habit of bundling together discrete units (e.g., the app and the underlying database) in a virtual machine, and binding data (typically accounts) to a virtual machine as a way to manually “scale” the app to multiple deployments. If you did this, you would likely be stuck in the same pattern, with multiple single-replica deployments of your app on a cloud platform.




%modern software development practices, technologies, and 



% Clear testing goals are established, making it easier for testers and developers




%While existing benchmarks, such as YCSB~\cite{cooper2010benchmarking}, can help assess the performance of clients, they do not provide insights into system network traffic, I/O patterns, and resource utilization. This information is necessary for comparing system scalability (e.g., avoidance of hotspots), system continuity in the presence of failures~\cite{10.5555/1009382.1009743} (e.g., failure detection time and failover overhead), and the total cost of ownership (e.g., accounting for high memory requirements or increased I/O amplification).

Our system is designed to be intuitive and quick to learn, and you won’t have to waste time setting up any infrastructure before starting your testing. 


there is a lot of distributed monitoring and orchestration needed. Because of that, manual tests tend to be long with very low level details, 



Because of that, there are numerous aspects, such as failure modes or dynamically changing workloads, which engineers cannot adequately cover via the manual testing method.


which makes handcrafted tests hardly scalable or reusable across infrastructures. 

Finally, manual tests written in imperative style 


 This will make performance testing easier and more consistent.


In declarative testing, a test scenario focuses on what to accomplish. 






handling the logical dependencies between jobs, scheduling actions, and validate their impact. 


which engineers cannot adequately cover via the manual testing method.


Behavior can be described in terms of 




%actual behavior and expected behavior to expose structural errors and performance problems in distributed systems. 

%improving testing simplicity, speed of testing, and ease of testing evolution. 

%the mechanism used to retrieve and analyze results is often based on the practitioner's experience and intuition rather than a systemic approach

%An urgent question follows on the heels of these detriments: How can we test a cloud-native application before putting it into production?




, rather than on the imperative details of how to manipulate the state of an application under test and verify the final application state against an expected state. 




which makes it difficult to write test correctly. 

An imperative styled scenario is more appealing to a reader who wishes to understand the “Hows” of the system because it is generally detailed around the mechanism whereas a reader who just wants to understand the “Whats” of a system would prefer a declarative style.


it difficult to create new tests. 


you improve your tests by ensuring that they only fail when behavior — not a particular implementation —
comes down to specifying how to 

many bugs reflect discrepancies between a system's behavior and the programmer's assumptions about that behavior. If assumptions are written in code, it is likely to 


The imperative approach is simple and intuitive and reflects what manual testers do.

Instead of the imperative style, 

In short, the imperative programming paradigm comes down to specifying how you want to accomplish something while the declarative programming paradigm comes down to specifying what you want to accomplish.




If so, it’s very likely that you’ve been writing your tests imperatively. By writing your tests declaratively instead, you improve your tests by ensuring that they only fail when behavior — not a particular implementation — changes.






Declarative and data-centric languages have traditionally
been considered useful in very few domains, but things have
changed substantially in recent years. 


Let’s say the main idea up to this point was to make tests declarative by expressing them in terms of data instead of procedural code. We declare context, inputs, and expected outputs as data.


Tests in this way become a set of cases and expectations. This isn’t new — FitNesse proposed a similar approach, although within a specific tool and environment and within the idea of acceptance tests, putting a focus on different stakeholders and on a higher business perspective. 

The term \emph{model-based testing} refers to test case derivation from a model representing software behavior (Bertolino et al., 2005). 
\CHECKnote{Exist full-featured , but are framework-based and therefore not applicable to CLoud-native}

% Cheap and disposable testing environments with a coordinated deployment pipeline;

\CHECKnote{We can do it in Kubernetes, but Kubernetes abstractions are not ideal for experiments}

\CHECKnote{[MM] list of contributions ?} 



by spreading the application load across physical nodes, balancing requests across different instances, or migrating instances to another host if there is a shortage of resources. 

\item   For example, before we start loading a server with keys, we must be sure that the server is running, and before we start running queries, we need to be sure that all keys are ingested. The monitoring and instrumentation pipelines required to respect these logical 





their systems before the actual deployment. 

be used across development, testing, and production environments. 


provides a cheap and disposable environment






 for  W


can integrate their preferred fault-injection, inspection, and benchmarking tools, 

so to test their systems before the actual deployment.







  \item Reusable templates and patterns for unbiased and non-intrusive grey-box testing, \hl{that can be incorporated or followed as a whole so as to leverage the benefits of the scaffolding provided} by \frisbee{}.


 
 
 %\item \textbf{Executing Tests} Typically, test execution just call generated test cases, which issue calls on an existing SUT. However, in our CPS, before and during a test case, we may need to reconfigure and deploy test utilities and SUT. This activity thus cannot be done simply through typical MDE/MBT tools which are not integrated with techniques for on-demand deployment. It needs a combination of MBT-test unit and elastic execution techniquesin IoT and Cloud in order to deal with various situations related to (part of ) SUT and test utilities.
    
 
% without having to consider the execution environment or the underlying infrastructure



%Types can represent Nodes and Relationships helping to define connections between nodes of the model.


%\frisbee{} project aims at establishing the basis for a Kubernetes-based platform to carry out uniform and systematic validation, verification, and testing activities applied to cloud-native applications. \frisbee{} automates all steps , from deployment to validation and clean-up, bringing five critical aids to testers:
 
 
 A container allows you to run a program under a specific environment software (language version, libraries, third-parties), additionally to limiting the resources (CPU time, memory) used by the program.


Declarative testing is a test design paradigm which 


\CHECKnote{[MM] verify "grey-box" (vs. black-/white-box)}


\hl{that can be incorporated or followed as a whole so as to leverage the benefits of the scaffolding provided} by \frisbee{}. 
\CHECKnote{[MM] Circular description of what \frisbee{} is. Is it a "project", a "framework", a "runtime", a "toolset", something else ?!}






%\begin{itemize}
    %\item \textbf{Modeling}: Most effort in these types of activities can be achieved through the utilization of MDE tools.
    
    %\item \textbf{Deploying SUT}: In the cloud/IoT one can switch from one provider to another provider for certain services/IoT. Thus, in many cases, (part of) the SUT is just deployed before or during tests. Thus, here we need to incorporate techniques from elasticity and dynamic provisioning.
    
    %\item \textbf{Deploying Test Utilities}: Because of multiple providers, test utilities can be deployed at different systems. Furthermore, due to elasticity, we need to reconfigure test utilities.
    
%    \item \textbf{Validating Tests}
%\end{itemize}

 
 
 
The saturation point is the peak throughput where diminishing returns (e.g., due to thrashing) begin to take over. At this condition, after a sufficient increase in a causal force, no further increase in server utilization is possible. Therefore, it is an important metric when deploying a system, as it indicates the processing capacity of each instance. 

Additional challenges arise because distributed systems produce so many operation metrics that operators can easily overlook important trends. Expressions of this type are useful for detecting anomalies in the system, or detecting over/under utilization of resource. The latter is  In the evaluation Section, we demonstrate their usage for detecting bottlenecks in the system. 







allowing expressive Behavior-Driven Development ("BDD") style tests

using expressive Behavior-Driven Development ("BDD") style:

that can express the behaviour and the expected outcomes.


BDD is largely facilitated through the use of a simple domain-specific language (DSL) using natural-language constructs (e.g., English-like sentences) that can express the behaviour and the expected outcomes



Tests in this way become a set of cases and expectations.


Given method preconditions as declarative constraints, our framework systematically generates 


   Provides a better process to ordering your thinking. (First, do the imperative test. Then, generalise a function for the second case in terms of inputs, what they do, and your expectations.) Also spend some time thinking about different scenarios and how to express them in this test’s language.



 as data

 We declare . This, however, requires the presence of an automation framework. 


 Traditionally, many developers write unit test to validate that, for a particular concrete input, a program produces the expected result. In more complex end-to-end testing tests, developers  Developers often take both approaches, but there are many specifications to write, and if they are written in imperative languages (e.g., Java), the code is bloated. 



Moreover, imperative testing does not scale well as the size and complexity of the application increases.

Let’s say the main idea up to this point was to make tests declarative by expressing them in 



(typically with a black-box mindset)

provide the specification of expected behavior of the system under test. In the absence of such specifications, the only behaviors that can be automatically detected are those that interrupt testing (e.g., system failures).  



Manual testing is slow, expensive, and 




Benefits of the Declarative Approach

Designing declarative expressive tests:

    Gives higher readability
    Improves maintenance
 
 
 
    Exploits the full value of code reviews: Reviewing a big set of tests that have many lines of imperative and/or duplicated code takes extra mental effort beyond thinking about test coverage (in terms of possible scenarios not in LOC). This approach reduces that effort completely, allowing the reviewer to focus on missing cases and whether the current scenarios and expectations make sense from the domain point of view.


Oppositely, 
Behavior-Driven Development ("BDD") style tests


it often implies . As shown, the API may refer to the 's API or the 's API.  

\CHECKnote{continue}

allowing expressive 


 %The additional challenge is that constituent microservices, potentially written in different languages, may not always follow a common architectural pattern (e.g., circuit-breaker) or share the same software testing framework. 



The declarative programming paradigm enables the developer to describe what the application should accomplish rather than how to accomplish it, thus avoiding to include the control flow within the application.




designed for seamless integration with the 

's abstractions are the first for modeling real activity and validate the application's behavior, both under normal and unexpected conditions.

cloud-native applications 

Declarative testing frameworks already exist for detecting layout bugs in web applications~\cite{HALLE2016737}, or generating test inputs for given codeblocks to maximize their code coverage~\cite.

Firstly, the constituent microservices 

Moreover,  To the best of our knowledge, \frisbee{}'s abstractions are the first for modeling real activity and validate the application's behavior, both under normal and unexpected conditions.







automates all steps , from deployment to validation and clean-up,

The \frisbee{} project aims at establishing the basis of a Kubernetes-native platform to carry out a uniform and systematic testing of Cloud-native applications. 

\frisbee{} consists of the following layers:
\begin{itemize}
    \item \textbf{Application Layer:} 

    \item \textbf{Test Case Layer:} provides a declarative language that 
    
    \item \textbf{Framework Layer:} 
\end{itemize}


\begin{enumerate}
    

    
\end{enumerate}








for the validation, verification, and 

 This language 

and visualizing valid and invalid behaviors.

    
    \item A declarative language designed to focus 
    
    sequences of actions and  after its action
    



for the scalable, extensive  dynamic testing of cloud-native applications.

to carry out uniform and systematic testing activities applied to cloud-native applications. 

exploring, testing, and benchmarking Cloud-native applications. 

Our main contribution, is designing and implementing a platform for  While there various aspects of these systems can be tested individually, to our best knowledge Frisbee is the only design that integrates all (the 7 concepts) together, etc. ...

platform  The goal is to enable tests that 



We present \frisbee{}, a \frisbee{} removes the hurdles of systems deployment and testing complexity from the users, and provides abstractions for modeling arbitrary topologies and dynamic workflows.

 We support abstractions for services, groups of services, dependency management, placement policies, scheduling constraints, and conditional execution.  Our experiments demonstrate the interplay of:
\begin{enumerate*}[label=(\roman*)]
    \item logical grouping,
    \item dependency management,
    \item scheduling constraints,
    \item resource throttling,
    \item failure injection,
    \item informed placement, and 
    \item contextualized visualization of the application state.
\end{enumerate*}


\frisbee{} removes the hurdles of systems deployment and testing complexity from the users, and provides abstractions for modeling arbitrary topologies and dynamic workflows. We support abstractions for services, groups of services, dependency management, placement policies, scheduling constraints, and conditional execution.  Our experiments demonstrate the interplay of:
\begin{enumerate*}[label=(\roman*)]
    \item logical grouping,
    \item dependency management,
    \item scheduling constraints,
    \item resource throttling,
    \item failure injection,
    \item informed placement, and 
    \item contextualized visualization of the application state.
\end{enumerate*}



%However, testing cloud applications demand us to manage complexity throughout different activities for testing, from requirement specification, to development and deployment of both application and platform components, as well as elastic demands of these components at runtime. 


%We believe that this definition style results in deployments that are easier to understand, develop, test, and more resilient to architecture erosion. It also facilitates troubleshooting. It is easier to detect, reason and fix bugs when changes are systematically mastered (or edited) in a human-readable file, rather than investigating each component of the system to find the anomalies.




Therefore, YCSB is inappropriate for infinite horizon tests designed to expose failure conditions such as thread/memory leaks or sensitivity to OS disk cache hit ratios from long-running processes~\cite{DBLP:journals/corr/abs-1807-10792}.

due to the smaller window, periodic tasks such as flushing had a more significant effect which a larger window would otherwise amortize. 


We are currently working on an auto-tuning feature to perform an exponential backoff algorithm and steps down the load based on preset \% of SLA violation. This is needed because in some scenarios the data stores may be only slightly overloaded and may have passed the threshold at which they can continue to operate within SLA. Yet, we still have to investigate other metrics that may appear more suitable for finding the saturation point, such as percentile latencies exceeding a set limit, mutations dropped by a database or index document failures in a document store.

\CHECKnote{AC: The remainder of this section could be summarized in one paragraph. Do not tell us all the issues... We need to focus on how you used the same configuration to find the saturation point on different hardware. If you did find it, just mention that Frisbee allowed this to be done and what it is. If there were issues, tell us how Frisbee helped to find and solve them. Do not concentrate on other details.}

We present \frisbee{}, a Kubernetes-native platform for exploring, testing, and benchmarking Cloud-native applications. \frisbee{} removes the hurdles of systems deployment and testing complexity from the users and provides abstractions for modeling arbitrary topologies and dynamic workflows. We support abstractions for services templates, groups of services, dependency management, placement policies, scheduling constraints, and conditional execution.  Our experiments demonstrate the interplay of:
\begin{enumerate*}[label=(\roman*)]
    \item logical grouping,
    \item dependency management,
    \item scheduling constraints,
    \item resource throttling,
    \item failure injection,
    \item informed placement, and 
    \item contextualized visualization of the application state.
\end{enumerate*}


Using \frisbee{}, we extract numerous insights that can influence the way we evaluate our applications. The ability to run various mixes of I/O workloads showed us that inserting new keys into a running Redis server can greatly impact the performance of collocated clients. The contextualized visualization revealed insights about the metrics we should use to avoid invalid conclusions and unfair comparisons when reasoning about the performance baseline of a system. Workloads often exhibit artifacts that aggregated values tend to hide, such as slow operation and operation errors. Along with that, the chaos capabilities and the global view of the system state that \frisbee{} provides allowed us to simulate network partitions study the recovery mechanisms of Redis. By studying the mechanism from the perspective of the master node, the slave node, and the client, we found out that the benchmark (YCSB) does not support failover for Redis. Further, we used \frisbee{}'s ability to perform real-time analysis on performance metrics, which allowed us to discover the saturation point of a Redis server automatically. Finally, in a effort to use the same configuration to find the saturation point on different hardware, \frisbee{} ability to perform resource throttling appeared extremely helpful to scale down the problem to the capacity of the hardware. 



Lastly, we have already integrated \frisbee{} into the continuous testing pipelines of our team, so to run a repeatable set of performance tests whenever we make a commit to the code repository. Thus, beyond the functional testing, we have fast feedback that a change will not negatively impact deployed services.  As we believe that platforms like \frisbee{} will play an catalytic role in the design and evaluation of emerging applications, we have made the source publicly available. % at https://github.com/CARV-ICS-FORTH/frisbee.


finding the saturation point required us to 

Due to the limited space, we do not provide figures, but instead, we explain the challenges we met for replicating the experiment. 


\textbf{Premature completion of workloads:}
A faster CPU means that Redis can serve more requests in a given time, which means that a finite workload completes faster. In turn, this caused the first client to finish prematurely,  One solution would be to have a significantly larger workload. A better approach would be to run YCSB in an infinite loop, but this is not a support feature. 

\textbf{Reducing client threads:}
A side effect of the faster request processing is the increased demands in memory capacity. Redis consumed the entire memory before the experiment was over when we ran the test into the workstation. Thereby, we had to decrease the number of threads per client from four to one to mitigate this effect. This smoothened the rapid cliffs in the plot, but it did not allow us to reach a saturation point before the entire memory was consumed. 

\textbf{Reducing client resources:}
To further reduce the load generated by each client, we throttled the client's container to 0.5CPUs. This further smoothened the cliffs, but the memory was consumed again before the end of the experiment. The reason is that slower clients mean that we need more clients to reach the saturation point. We then realized that the problem is not about how we distribute the workload over time but instead that the scale of the experiment (total number of keys) was beyond the workstation's memory capacity. 

\textbf{Reducing Spacing between services:}
To reduce the scale of the experiment, we 



\CHECKnote{
Frisbee does not currently support dynamic exploration of inputs. If the user-given are wrong, or the experiment too large for the given infrastucture, \frisbee{} cannot do much







Kubernetes also provides the means for resources throttling, allowing us to selectively saturate devices (e.g., disks, memory, CPU) in a more deterministic manner than stressing workloads~\cite{gupta2011diecast}. 
}

==> sections/references.tex <==
https://pingcap.com/blog/building-automated-testing-framework-based-on-chaos-mesh-and-argo#verifying-chaos-impacts-test-cases

https://netflixtechblog.com/chap-chaos-automation-platform-53e6d528371f

https://storage.googleapis.com/pub-tools-public-publication-data/pdf/24017e52c907294589604a29a86f158828eda078.pdf


http://techgenix.com/chaos-mesh-chaos-engineering/


https://pingcap.com/blog/chaos-mesh-your-chaos-engineering-solution-for-system-resiliency-on-kubernetes

https://blog.mayadata.io/a-brief-introduction-to-kubernetes-and-chaos-testing

https://blog.container-solutions.com/comparing-chaos-engineering-tools




https://kubernetes.io/docs/reference/kubectl/cheatsheet/



https://kubernetes.io/docs/concepts/workloads/controllers/job/



https://medium.com/google-cloud/kubernetes-running-background-tasks-with-batch-jobs-56482fbc853



https://www.magalix.com/blog/kubernetes-patterns-the-batch-job-pattern



https://blog.container-solutions.com/comparing-chaos-engineering-tools


https://pingcap.medium.com/chaos-mesh-your-chaos-engineering-solution-for-system-resiliency-on-kubernetes-a95f7489d708


https://www.tutorialspoint.com/object_oriented_analysis_design/ooad_object_oriented_analysis.htm


https://pingcap.medium.com/chaos-mesh-your-chaos-engineering-solution-for-system-resiliency-on-kubernetes-a95f7489d708


https://itnext.io/getting-started-with-chaos-mesh-and-kubernetes-bfd98d25d481


https://www.continuitysoftware.com/wp-content/uploads/2014/05/2014-SA-Survey-Report.pdf

https://blog.synology.com/data-durability

https://www.datadoghq.com/blog/monitoring-mongodb-performance-metrics-wiredtiger/

https://hackernoon.com/platforms-on-k8s-with-golang-watch-any-crd-0v2o3z1q












Dear reviewers, 

Foremost, let me thank you for your constructive feedback. 

The research contribution of Frisbee is that it allows operators to define both the dynamic operating conditions, and the expected behavior of the system under these conditions.

Let me give you two examples that demonstrate the applicability of Frisbee.

== Example 1: dynamic nature of group membership ==

Assume a self-healing system that can presumably tolerate failing nodes by rebalancing the load to the remaining nodes.
Let us assume a system with 10 nodes, out of which at least 7 must be available at any given moment.
To implement this scenario, the operator should follow the next steps.
1) use a group of 10 nodes, with a tolerance of 3 failing nodes.
2) use a benchmark that sends requests to the servers (e.g., YCSB).
3) periodically kill the three nodes

If the experiment completes successfully, it means that no more than 3 nodes failed during the experiment.
If the experiment fails, it means that more than 3 nodes have failed during this experiment. In this case, there is probably an unexpected dependency between the nodes (e.g., blocking requests).

This experiment is based on the "Phase events", that transpire to the lifecycle of containers. 

== Example 2: handling bitrot ==

Assume a single-node key/value store that can presumably detect and repair bitrots on a disk.
To implement this scenario, the operator should follow the next steps.
1) use a single instance of the K/V
2) use a benchmark that performs READ-MY-WRITE requests, and validate the returned results. 
If it detects an error in the payload, it writes it to the output log. A sidecar agent subsequently parses the log, and the metrics are forwarded to Grafana.
The operator can define the maximum period for which errors can be tolerated.
3) use fault injection to create bitrots on the disk

If the experiment completes successfully, it means that the system successfully handled the failure.
If the experiment fails, the system failed to recover before the failure became visible to the end-user.


This experiment is based on the "Performance events", that transpire to the performance metrics collected by sidecar agents.


Next, let me address your point regarding Envoy sidecars. 
Indeed, Envoy can provide visibility on the network traffic, and support fault injection, at the level of the network. 
The difference is that Frisbee operates on application level, rather than the network level. 
That includes, a broader range of failures (e.g, kills, partitions, I/O), and application-level monitoring (e.g, number of ingested keys, replication errors, etc).


==> sections/sabouria.tex <==


 This is especially true when nodes are required to change their behavior dynamically, or when there are dependencies between the various phases of the testing. For example, running YCSB benchmark against a cluster of servers requires three distinct steps.
\begin{enumerate*}
    \item all the servers must be up and running 
    \item the servers must be preloaded with the keys
    \item run queries against the servers
\end{enumerate*}
Evidently, the next phase can be started only when the previous phase is complete. And since multiple servers are involved, distributed coordination is required for the consistent transition from one phase to another. 


This paper deals with testing distributed software systems. 


Internet of Things (IoT) represents a global market transition driven by a surge in connections among people, processes and things. The growth of commodity devices that integrate physical processes with digital connectivity has had profound effects on society–smart homes, personal monitoring devices, enhanced manufacturing and other IoT applications have changed the way we live, play, and work.  



The large variety has made it difficult for developers tochoose the appropriate system.



A sensor produces data concerning its surrounding environment, whereas an actuator operates in the reverse direction of a sensor. It consumes data and turns it into physical action.




\subsubsection{Multi-stage building}
With Dockerfile specified, IOTier puts the IoT application into its pipelines using Docker's multi-stage builds. Using the Dockerfile as the first stage of multi-stage build, IOTier prevents undue confusion by organizing the next stages as to install the necessary dependencies, improve building time, minimize the size of the final image, and improve run time performance.


 
 

\subsubsection{Multi-stage building}


From the Pod’s perspective, it exists in its own Ethernet namespace that needs to communicate with other network namespaces on the same Node. Thankfully, namespaces can be connected using a Linux Virtual Ethernet Device or veth pair consisting of two virtual interfaces that can be spread over multiple namespaces.



To connect Pod namespaces, we can assign one side of the veth pair to the root network namespace, and the other side to the Pod’s network namespace. Each veth pair works like a patch cable, connecting the two sides and allowing traffic to flow between them.



Interestingly, the application may reside on the device itself (ie: wearable).


“So for example, the agent is able to do some auto-discovery processing. If I’m running inside of a Docker Swarm or this agent is running inside of Kubernetes, all this data will be collected into our central platform, which can be installed on-prem also.”



The essence of containerization is distilled into three subsystems that collectively structure a distributed IoT emulator:



can inject chaos on the infrastructure layer

Timeouts are possibly the most dangerous edge case to overlook. Your service might get away with it on a controlled network, but it will not survive on the open Internet, especially (but not only) if maliciously attacked.

Propagation delays are proportional to the network distance between the sender and the receiver. Hence, to validate high-precision IoT performance with real-world network conditions, the virtual testbed must be aware of the topology and calculate the end-to-end impairments. 


Applying timeouts is a matter of resource control. Even if goroutines are cheap, file descriptors are always limited. A connection that is stuck, not making progress or is maliciously stalling should not be allowed to consume them.


[Tiers may be accommodated by a single-server, or run on different set of servers.]






Notably, for each class of resources (e.g, CPU, memory, storage, network), we provide real-world profiles acquired by state surveys, crow-sourcing, experimental values, and vendor specification.



Helios is a distributed, highly-scalable system used at Microsoft
for  that is designed to plug into relational engines.



The system collects close to a quadrillion events indexing approxi-
mately 16 trillion search keys per day from hundreds of thousands
of machines across tens of data centers around the world. Helios
use cases within Microsoft include debugging/diagnostics  in both
public and government clouds, workload characterization, cluster
health monitoring, deriving business insights and performing im-
pact analysis of incidents in other large-scale systems such as Azure
Data Lake and Cosmos. Helios also serves as a reference blueprint

for other large-scale systems within Microsoft. We present the sim-
ple data model behind Helios, which offers great flexibility and

control over costs, and enables the system to asynchronously in-
dex massive streams of data. We also present our experiences in

building and operating Helios over the last five years at Microsoft.




Controller-manager: used to schedule and manage the lifecycle of CRD objects

Chaos-daemon: runs as daemonset with privileged system permissions over network, Cgroup, etc. for a specific node

 
In traditional testing, such as unit tests, a component or unit of code is tested by providing defined input and validating the output of the unit.  


    \item type and number of services participate in the experiment. Services can be user applications, storage systems, processing systems, or any other application that seems fit to an IoT environment;
    
    \item performance chacteristics 
    
    physical resources allocated to services. 
    
    , so to mimic the performance characteristics of IoT constrained environments;
    \item groups of containers making a tier;
    \item characteristics of the nodes where the tiers are running;
    \item phases and phase-changing conditions effectively describe the plan's evolution over time.  
\end{itemize} 







\begin{table*}[!ht]
\centering
 \begin{tabular}{c c c c} 
 \hline
 Experiment & Path & Variable & Phases \\ [0.5ex] 
 \hline\hline
 Link type & Common & Link & (Single) Link changes between client-server \\ 
 Partition Size & Uncommon & \#Servers & (Single) client link to number of (unthrottled) servers \\
 Migration & Uncommon & \#Servers & (Multi) Servers added in phases \\
 Replication & Common & \#Links & (Single) 7560 \\
 Contention & Common & \#Clients & (Multi)  6344 \\ 
 Tiering & Common & Links & (Single)  6344 \\ [1ex] 
 \hline
 \end{tabular}
 \label{table:experiments}
\end{table*}


IP networks are stateless and packet-switched networks by design; in fact, this statelessness is one of the fundamental strengths of IP.    


In this respect, \ac{IOTIER} provide automated pipelines , and provide the means to correlate observed phenomena back to triggering events

throttles down physical machine resources to emulate the target profile, , orchestrates 



The primal idea of , evolved into compartmentalized experiments with the intent being to structure experiments into framed phases. 


 %Rigorously testing a network device or distributed service requires  complex, realistic network test environments. 
 
 
 


observability as to correlate anomalies to specific events, 



A Deployment pipeline is the process of taking code from version control and making it readily available to users of your application in an automated fashion.

 
Our goal is still to create an Impairment Node device that manipulates traffic between two of its Ethernet interfaces `eth0` and `eth1`, while managing it from a third interface (e.g. `eth2`).



 These table stores are typically designed for high scalablility by using semi-structured data format and weak semantics, and optimized for different priorities such as query speed, ingest speed, availability, and interactivity. Further, as these systems mature, lots of adavanced features, such as ingest speed-up techniques and function shipping filters from client to servers, have been developed to serve a wide range of applications and workloads. 
 
 

A task is the atomic unit of scheduling within a swarm. When you declare a desired service state by creating or updating a service, the orchestrator realizes the desired state by scheduling tasks. For instance, you define a service that instructs the orchestrator to keep three instances of an HTTP listener running at all times. The orchestrator responds by creating three tasks.


 used to run experiments against a hypothesis around complex distributed systems. 

Practitioners define a hypothesis and measurement criteria, then introduce deliberate stimuli into the system to verify the hypothesis. 




hypothesizing around placement policies and workloads,


 


As will be explained in Section~\ref{sec:plans}, phases are not mutually exclusive and may run concurrently. 




\begin{enumerate}
    \item type of IoT components 

    \item type of services, number of replicas, and allocated resources. Used to emulate IoT components
    \item overlay network for the service to connect to other services. Used to emulate IoT links.
    \item labels containing metadata for other subsystems
    \item an overlay network for the service to connect to other services in the swarm
    \item interconnected into complex virtual networks
    \item placement constrains
    \item Docker Compose labelling mechanism to declare policies for Docker objects, such as containers and networks. 
    \item specify network conditions and provide flexible network resource control between containers.
    \item To achieve that, it provides easy custom definitions for the IoT components, the way they are structured into tiers, the placement of computation and storage tasks across tiers, and the way experiments evolves over time. 
\end{enumerate} \todo[inline]{FIXME}





Affirming the idea of tiering as the rule rather than the exception, \ac{IOTIER} seeks to provide the necessary building blocks to create controlled testing environments that answer the following questions: 
\begin{itemize}
    \item What is the effect of network properties (e.g, bandwidth, latency) to the application performance?
    \item Under what circumstances can the core cloud perform better than an edge network and vice-versa?
    \item How do network QoS (unidirectional, bi-directional, asymmetric) affect data migration?
    \item How does Breadth-first and Depth-first tiering affect high-speed ingestions? 
    \item How should we place writers/readers to achieve optimal freshness/responsiveness 
    \item What should be the performance characteristics of IoT components (e.g, Edge devices, Gateways) to support constrained applications (e.g, haptics, video, voice). 
    \item Identify mistuned retry policies, CPU-intensive fallbacks, and unexpected interactions between devices and tiers.
\end{itemize} 
 
 
 
 
 

%Image you have 4 servers in 2 datacenters (east, west) and some of the servers have an SSD drive, while others don't.
%If you apply the following labels to the nodes:
%node-1: datacenter=us-east, disk=ssd
%node-2: datacenter=us-east, disk=ssd
%node-3: datacenter=us-west, disk=sas
%node-4: datacenter=us-west, disk=nl-sas
%If you would deploy a service with 2 replicas and you want to provide geographic redundancy, you would start that service as follows:



 




Both forms of DES contrast with continuous simulation in which the system state is changed continuously over time on the basis of a set of differential equations defining the rates of change of state variables. 




But simulators are neither real-time, nor they attempt to emulate the actual hardware  In contrast, an Emulator is a software that attempts to mimic all of the hardware features of an underlying infrastructure. 


the application architect must carefully distribute the application's computation and storage tasks across tiers.





 The modularity of the core ensures a scalable architecture, both in terms of the type of emulated models and their number. In turn, the decoupled execution of models enables the coexistence of both complex and simplified ones. 



EDIT: Other responses have pointed out that the goal of an emulation is to able to substitute for the object it is emulating. 


the financial and energy analysis of the potential technology investment, high-speed simulation tools for the evaluation and development of energy management algorithms (without prior infrastructure investment), and finally, support of occupant-oriented studies on potential energy savings.

The simulation will take care only of some aspect of the actual thing, usually those related to how a human being will perceive and control it. The simulator will not perform the functions of the real stuff, and cannot be sustituted to it.





Many organizations overlook the importance of emulating realistic and worst-case network scenarios in the lab. Failure to test variables such as application performance, effect of delay, and fail-over protection can have serious real-world implications.






Litmus takes a cloud-native approach to create, manage and monitor chaos. Chaos is orchestrated using the following Kubernetes Custom Resource Definitions (CRDs):

    ChaosEngine: A resource to link a Kubernetes application or Kubernetes node to a ChaosExperiment. ChaosEngine is watched by Litmus' Chaos-Operator which then invokes Chaos-Experiments
    ChaosExperiment: A resource to group the configuration parameters of a chaos experiment. ChaosExperiment CRs are created by the operator when experiments are invoked by ChaosEngine.
    ChaosResult: A resource to hold the results of a chaos-experiment. The Chaos-exporter reads the results and exports the metrics into a configured Prometheus server.
    
    
A custom resource is an extension of the Kubernetes API that is not necessarily available in a default Kubernetes installation. It represents a customization of a particular Kubernetes installation. However, many core Kubernetes functions are now built using custom resources, making Kubernetes more modular.








Immersion level 	Device 	Sensor 	Example use cases
0	real	real	(i) typical usage of the implemented IoT system
(ii) final product testing
1	real	virtual	(i) simulating edge conditions for the IoT system (e.g. extreme temperatures measured by sensors)
(ii) testing device capabilities
(iii) choosing appropriate sensors in the design phase
2	virtual	virtual	(i) low-cost simulation of multiple data sources
(ii) testing horizontal scalability of the system
(iii) testing applications working on the edge










 Although extant emulators and simulators address some of the aforementioned challenges, as of today, there is no tool that solves all of them. 
 

 



to keep pace with the  testing 

In this view, 


, without real-world repercussions. 






% RUN THE FULL STACK
% CREATE EXPERIMENT TIMELINES


    
    
    
    Thereby, \ac{IOTIER} facilitates the understanding of system's behavior under various circumstances, and enables engineers to build confidence in the system's capability to withstand unexpected conditions, or identify the key aspects that need improvement.
    
    
%We also have taken metrics from the European Telecommunications Standards Institute (ETSI) to build a set of IoT use cases referred to as public lighting scenarios.




\begin{figure}[ht]
    \includegraphics[width=\linewidth]{images/workflow.pdf}
    \caption{Workflow of IOTier}
    \label{fig:workflow}
\end{figure}






many tieried architectural aspects need to 

aimed to 

, should inevitably be designed with tiering in mind. 




In effect,  require  to be designed with tiering in mind. 

. Factors such as hardware in IoT components, inter-tier and intra-tier communication, as well as the software's tight coupling, create challenges that are like to hinder the functionality of IoT systems. 







The Internet of Things is on its way to become the biggest software development and testing opportunity of all time. IoT brings many new things to the table in terms of testing requirement , including quite a few unusual device types like home appliances, watch sensors etc. With such an eclectic mix of products in the IoT ecosystem, it becomes imperative for the QA team to come with an effective test strategy to meet the quality of these diverse products.


    
    Security and data privacy
    Support for data volume, variety, veracity etc.
    Too many IoT protocols to test like MQTT, XMPP, CoAP etc
    Diversity in the IoT apps and devices
    Large number of sensor interactions.



    Virtualization: The highly complex nature of the IoT ecosystem would make  Therefore, introducing sufficient amount of virtualization into the services on which IOT applications are built will result in faster turn around and reduced costs due to minimal dependency on the real-time environment. It would also lead to earlier detection of defects. 
    Building Labs that serve the entire digital portfolio to experiment and simulate real-time experiences which would help us inform smarter ways of testing.


    Device Interoperability Testing: This involves assessing the ability to seamlessly interoperate protocols and devices across different standards and specification. In a nutshell, it verifies the connectivity across all the devices and protocols in the IoT set up. Interoperability Testing in the Service Layer of the IoT framework becomes very crucial as IoT requires standards to enable platforms that are communicable, operable, and programmable across devices, regardless of make, model, manufacturer, or industry.

Example: If a user is using an iPad as well as a Mac for IoT application, the transactions done or data saved on iPad is “As-is” when accessed through Mac desktop. 

An IoT set up consists of a diverse mix of elements like Sensors, Applications, Network and Datacenter.  Therefore, it becomes very important for the QA group to determine the various type of testing that needs to be conducted on these different IOT elements. Needless to say, not all types of testing are applicable for the various IoT elements. 


We therefore ground our approach in simulating real-world environments, devices, and sensors [7] which, on the one hand, does not require custom hardware for application development, while on the other hand permits integration with existing IoT hardware devices depending on the maturity of the tested IoT system. In our concept, the following elements can be substituted by their virtual counterparts in the testbed:(i)environment: where real-world environments are replaced by simulated ones;(ii)sensors: where sensors are virtual and measurements simulated;(iii)devices: where devices are also virtual.

































For many companies without a library of relevant testing devices, the effectiveness of a QA campaign can be watered down by an inadequate test coverage.
2) Test Diversity

Testing an IoT involves more just testing the actual device. It also includes testing its mobile application on a variety of devices to uncover bugs that can lead to recalls, hurt brand image, or erode consumer confidence.

While some test methods can focus on evaluating key functions, others can be better utilized to assess other important aspects like UX or accessibility. Without the right testing expertise, it can extremely difficult to plan, design, and execute a proper test.
3) IoT Stability

The key to any IoT is its ability to connect to other devices via a Bluetooth connection and/or a wifi network. Connecting and staying connected to another device or network is complex. Connection issues can rendre an IoT useless if it prevented from communicating and sharing data.











The amount of IoT devices and their collaborative behavior causes new challenges to the scalability of traditional software testing, and the heterogeneity of IoT devices increases costs and the complexity of coordination of testing due to the number of variables. 





% -- Old systems (challenges with existing technology)

Traditional database management systems fall short in efficiently handling this diversity. The reasons are fundamental and have to do with their "flat" (single tier) architecture, and the design assumption that such systems will operate in high-performance servers over with stable and high-bandwidth networks.  Deploying into the wild Internet a data management system that is designed for data-centers, can cause intriguing failures that may jeopardize key aspects of a system's operation. This can consist of an overload of concurrent requests, unintended traffic storms due to write/read amplification, degraded performance due to impertinent networks, or cascading timeouts due to tight coupling of software.





The most common use case  of bridge network is when we have applications running in standalone  containers on the *same* Docker daemon host, and we want these applications to communicate. Naturally, it is better for different namespaces to direct traffic into or out of different physical networks, or different subnets or different VLANs on the physical network.  For example, the physical  interfaces in the “global” namespace in the host may be in the range 172.16.1.0/24, while the virtual interfaces within the container may be in the range 10.1.1.0/24.





























In other words, *microflows* allow you to easily add complex business logic to the processes in your application without having to write code.

In the Mendix platform you create a model of your application using the  Mendix Business Modeler. We do not generate code but interpret this  model when starting the application in our server runtime. This approach has all kinds of advantages, such as being able to [debug visually](https://www.mendix.com/blog/the-ultimate-debugger/), even on remote environments.



Event handlers define microflows that handle certain events related  to the entity. Depending on the chosen moment and type, a microflow is  executed before or after creating, committing, deleting, or rolling back an object.

Event handlers should be used moderately, as they will be triggered  every time the corresponding event occurs, so they must be for things  you want always to happen. If you only want something to happen on a  certain page, you can use a microflow there (for example, on a  customized **Save** button).

Event handlers are not triggered in a  particular order. So, make sure events do not depend on each other in  any way (also with regard to events in generalizations and  specializations).

When events are triggered from microflows you can choose to bypass the event handlers in the microflow action.	



Phase is the state at a given time period. 

Event: a notification that makes Timon initiate a Microflow  

Microflow is a actions required to transition from phase another

Is a unit that helps with root cause analysis. Microflow helps to implement phase shifting



To avoid confusion, we must clarify that Microflows are not . It is rather a way of . For instance, in the first phase 

. A Microflow is essentially a time-framed phase

expressing the evolution of ahow an experiment evolves. 

Notably, Microflows are not independent bunch 

such as change the number of clients, number of servers, or inject failures. 



  On production environments, scheduled events are enabled/disabled via the appropriate tools (Developer Portal, Windows Service Console, etc.).



 or "phase". When an event is fired, TIMON marks the beginning of a new phase, and yield statistics for metrics (e.g, tail latency) as a function of time. 



distributed coordination abstractions that are required to instruct start and end of the various phases containers go through. In particular, these abstraction include 

The act of simulating something first requires that a model be developed. The model represents the key characteristics or behaviors of the selected environment, whereas the simulation represents the evolution of the internal state of the environment over time. 


CloudWatch Events does not provide second-level precision in schedule expressions. The finest resolution using a cron expression is a minute. Due to the distributed nature of the CloudWatch Events and the target services, the delay between the time the scheduled rule is triggered and the time the target service honors the execution of the target resource might be several seconds. Your scheduled rule is triggered within that minute, but not on the precise 0th second.

A rate expression starts when you create the scheduled event rule, and then runs on its defined schedule.

- [Cron Expressions](https://docs.aws.amazon.com/AmazonCloudWatch/latest/events/ScheduledEvents.html#CronExpressions)
- [Rate Expressions](https://docs.aws.amazon.com/AmazonCloudWatch/latest/events/ScheduledEvents.html#RateExpressions)

## Understanding Event Schedule Types[#](https://www.netiq.com/documentation/directory-and-resource-administrator-92/authoringguide/data/understandingscheduledevents.html#understandingeventscheduletypes)

Workflow Automation provides the following types of event schedules:

| One Time                | The event schedule generates an event once at the specified date and time. |
| ----------------------- | ------------------------------------------------------------ |
| Recurring               | The event schedule generates an event on a regular basis, such as the last Friday of every month. You can also configure the event schedule to generate an event multiple times on the specified day, such as every hour from 10:00 AM to 2:00 PM. |
| Start/End of Time Range | The event schedule generates an event at the beginning or end of one or more specified time ranges. The selected time ranges determine whether the event schedule is recurrent. You can also configure the event schedule to generate an event at both the beginning and the end of the specified time ranges. |

% operators can create templates for network devices (define network traffic policies), templates for IoT components (define CPU, MEMORY, IOPS, network devices), combine IoT components and application into services, and define phases and phase-dependencies for the experiment. 
























































\subsubsection{Orchestrators}

We, therefore, ground our approach in managing the experiment's lifecycle through machine-readable definition files, rather than physical configuration or interactive configuration tools. 





given workload for a fixed system configuration

high availability, rapid response, and local processing

Complex use cases and real-time responsiveness
    Performance requirements for 




anomalous 






Firstly, based on the real-time monitoring mechanism of CGroups file system, Virtual File System (VFS) of Linux kernel was used as a medium to pass the network control parameters set when Docker container was created to the Linux kernel controller TC. Then, the Intermediate Functional Block device (IFB) module was introduced to archive uplink and downlink bandwidth control, and the parameters (rate, ceil and prio) were used to achieve idle bandwidth sharing and container priority control. Finally, the specific network limitations were conducted by controlling the TC, and flexible network resource control between containers was realized.









On their own, custom resources simply let you store and retrieve structured data. When you combine a custom resource with a custom controller, custom resources provide a true declarative API.


​    



IoTTaaS  of remote distributed interoperability testing, scalable automated conformance testing, and semantics validation testing components adequate for testing IoT devices. 





autonomously control Things based on data input by sensors (e.g, telemetry, remote commanding). 



configure the Linux kernel packet scheduler, and enforce network traffic rules





Using a container technology like Docker, it is easy to deploy new containers programmatically using projects/services such as [Kubernetes](https://www.datadoghq.com/blog/monitoring-kubernetes-era/) or [ECS](https://www.datadoghq.com/blog/monitor-docker-on-aws-ecs/). 



. If you also design your systems to have a [microservice architecture](http://martinfowler.com/articles/microservices.html) so that different pieces of your system may be swapped out or scaled up without affecting the rest, you’ve got a great pattern for scale. 



%A host agent is run on system hosts to create the other failure scenarios like resource contention.

%two common frameworks are used; an injection framework and a host agent. The injection framework allows code to be instrumented with these different types of failures based on configuration which can be read quickly at runtime during the experiment. 





One of the places CPU shares breaks down is when you *don’t want* a container to be able to burst above its share when there is no  contention on the host. There are a number of valid use cases such as:



The end-to-end traceability of data flows through n-tier systems is a challenging task which becomes more important when systems increase in complexity. The Application Response Measurement defines concepts and APIs for measuring performance and correlating transactions between tiers. 

Used in IoT performance testing, they can assure their customers that their applications will be able to handle the scales of connections, topics and varieties of messages to work properly when deployed across heterogeneous environments. They can also create variety of benchmarks to show the scalability for sensors, volume of messages and topics. 

% single ycsb hi




 Custom controllers can work with any kind of resource, but they are especially effective when combined with custom resources. The Operator pattern combines custom resources and custom controllers. 

Separate logical tiers may run on separate physical servers, and each logical tier may itself run on a cluster.

In our emulator, we model the former behavior by means of intermittent connectivity, and the later by forcibly killing the Thing. 



Improved visibility: See what your simulation is doing with integrated IoT Hub charts showing device counts, connected devices, and message counts. You can also view message throughput, total connected devices, and error counts along with simulation configuration details.
    

    JSON or Protobuf messages: Send telemetry from your devices using your JSON schema or send telemetry using the binary Protobuf format from your simulated devices.

Integration with monitoring tool
    We customized an existing cluster monitoring tool Otus to gather the internal statistics of YCSB++, table stores, system services like HDFS, and operating systems, and to offer easy post-test correlation and reporting of performance behaviors. 







In IoT, however, the networking characteristics of a service depend on the tier the service is located to. This is challenging for the implementation for \ac{IOTIER} since network traffic rules cannot be statically defined within the container, but rather they have to managed externally. 

\subsection{Deploy Testbed}

But as the stack of the experiment grows, we start finding common configuration details that span multiple services. Changes have to be duplicated many times, while mistakes or omissions can happen by accident. To avoid repeating ourselves and make bulk updates easier, we split the testbed definition into three YAML files: resources.yml;, tier.yml, experiment.yml.

Resources are templates for various hardware and networks. Tiers, define templates for the virtual topology in which  Resources are placed, and how these topology is realized on a cluster of physical machines.  Templates are  for Docker objects. As shown in Listing~\ref{lst:yaml}, only Networks and Services are actual Docker objects that are instantiated. A Service is a group of one or more containers with the same configuration running under Docker's Orchestrators. Docker integrates two different Orchestrators for automated container deployment, scaling, and management across a cluster of machines: Docker-Compose and Docker-Stack. 

\todo[inline]{Write the overview}





Given a model with an initial environment state and a well-defined model, TIMON can trigger those events at a particular instant in time, It is also possible to define different evaluation 

operators to declare or specify the desired state of the testbed and 

for controlling the testbed's lifecycle through configuration and coordination of 



You can deploy and update a custom controller on a running cluster, independently of the cluster's lifecycle.

For example,   Similarly, it can change dynamically the network traffic rules enforced by  TC  within the containers.



through dynamic registration, , and inject failures either randomly or in deterministic patterns.  



you can let the runtime execute a microflow at a specific moment in time. The event can also be repeated with a given interval, for example every day.

on an automated schedule in Timon Events using cron or rate expressions. 

You can create rules that All scheduled events use UTC time zone and the minimum precision for schedules is 1 minute.

CloudWatch Events supports cron expressions and rate expressions. Rate expressions are simpler to define but don't offer the fine-grained schedule control that cron expressions support. For example, with a cron expression, you can define a rule that triggers at a specified time on a certain day of each week or month. In contrast, rate expressions trigger a rule at a regular rate, such as once every hour or once every day.



Scheduled events allow you to initiate a work item at a specific date and time. For example, if your company sets up, manages, and maintains servers for multiple customers, you can create a workflow that:

1. Starts at the beginning of a maintenance period for a particular set of servers.
2. Places the servers in maintenance mode.
3. Performs routine maintenance, such as performing a backup or rebooting a server.
4. Waits until the maintenance period ends.
5. Puts the servers back into production mode.







This means that every link is assigned to a separate subnet, and is accessible by the container as a different virtual network interface. This convention also makes the emulation of network properties more natural. It is easier to understand that the "i5G interface emulates a 5G device" rather than "172.50.25.0 subnet emulates a 5G device".








    Reusable device models: Device models can be saved, edited, and re-used across multiple simulations.
    
    Reusable simulations: Save your simulations and re-run them at any time from the simulation dashboard.






\subsubsection{Compose links} 

With TC configuration going through TIMON, we also gain automation on creating composite links to interconnect IoT components that are otherwise connected through intermediate nodes. This is a three step process. 

Whenever end-to-end communication is required, the traffic goes through  whose network distance is a vector of all the intermediate links along the path.

%At a high-level, TIMON provides (1) calculation of network traffic rules (2) execution of parallel commands to containers (3) 

If the variable becomes equal to the coordination group, it means that all containers have joined the current phase, and TIMON notifies its beginning.   If the variable becomes zero, it means that all containers have exited the current phase, and TIMON notifies clients to start joining the next phase. 



 You want per-interface metrics (because traffic happening on the local lo interface doesn’t really count). But since processes in a single cgroup can belong to multiple network namespaces, those metrics would be harder to interpret: multiple network namespaces means multiple lo interfaces, potentially multiple eth0 interfaces, etc.; so this is why there is no easy way to gather network metrics with control groups.



Ticks, and phases thereof, are time-based. Phases may be overlapping, but their duration and the period after which they `tick' the next phase are strictly guided by time. It is possible, however, for Timon to start new containers upon an event. For example, to kickstart a new server if the clients are experiencing a low performance. In this case, the event belongs to the phase in which it took place. Whereas containers provisioned to a phase are hot-started, event-based containers triggered at runtime, are inevitably cold-started. 

Besides, all the containers of a tier must be registered to a phase. Listing~\ref{lst:yaml} shows two phases: Load and Run, with the latter depending on the former. This dependency means that Run will start only after Load has sent a tick to Timon. 



When a tier is spin-up, the containers are pre-allocated but remain idle for as long as their phase is not `ticked'. This convention allows us to minimize interfering Memory and CPU spikes caused by a container's cold start, and ensure that containers run only on hosts with adequate resources to serve the provisioned load.



To better understand the impact of inter-tier and intra-tier connectivity, Figure~\ref{fig:network_profiles} depicts the performance profiles of some network interfaces that are common in IoT environments. 



Due to the large design space, it is not difficult to become lost in a sea of configuration noise.  We use *noise* as a colloquial to the phenomenon where the user is overwhelmed by exposed variables and blindly tries values, until the resulting values of the experiment makes sense. In an effort to facilitate valuable experiments with small learning curve, IOTIer is shipped with a set of of predefined resources. 





The Docker daemon listens on unix:///var/run/docker.sock, which only allows local connections by the root user. When you launch Docker, however, you can bind it to a different port or socket.

Like docker stats, the REST API continuously reports a live stream of CPU, memory, and I/O data. However, the API provides longer, live-streaming chunks of JSON, with metrics about the container.

While all these options are useful if you're planning to build your own tooling around Docker monitoring, there are several pre-built solutions, including Prometheus, cAdvisor, Scout, DataDog. We'll take a closer look at Docker health monitoring tools in the future.










thus system developers have little information to 

\ac{IOTIEr} sets the foundations for . 

. 











.The virtual network may reproduce long-distance WANsin the lab environment. These scenarios facilitate the test and evaluation of protocols and devices from the application layer to the  under a variety of conditions. NETEMallows the user to modify parameters such as delay, jitter, packet loss, duplication and re-ordering of packets






The testbed is based on three primary objects: Things, Networks, Tiers, and Data. All four are first-class objects that can be dynamically created, modified, or destroyed. 

 


The plethora of IoT devices, interconnection, and placement options limit traditional end-to-end testing due to the number of variables. 

%-- Solution




Virtual testbed describes the concept of 

Additionally, the amount of IoT devices and their collaborative behavior limits the scalability 

the *testing* rate


and use the new knowledge as a seed to the design of comprehensive data management architectures for IoT environments. 

We finally propose a data management framework for IoT that takes into consideration the discussed design elements and acts 




In addition, real-time or context-aware queries are handled through the federation layer via a sources layer that 





adaptive synchronization 

The framework we propose adapts a federated, data-centric and source-centric approach to link the diverse Things with their abundance of data to the potential applications and services that are envisioned for IoT.


\todo[inline]{Characterize the lifecycles as storage,process,communication intensive, in order to know what parameters to change}


exploration of large design spaces, and Chaos engineering.  The former is a practice for generating new knowledge, while fault injection is a specific approach to testing one condition.


Applying Chaos Engineering improves the resilience of a system.  You can then address those weaknesses proactively, going beyond the reactive processs

 yield statistics for metrics (e.g, tail latency) as a function of time.
    verifiable performance, price-performance, and availability metrics. 
       

Sensors produce a large amount of data for edge gateway devices so that these can make decisions by analysing the data. 





Hence, businesses can face a major issue of decreasing storage space in IoT data management. Also, business leaders have to explore how they can share and optimize the gathered data. For this purpose, business leaders can ask themselves the following questions:

    Can the existing infrastructure handle large volumes of data?
    Which platform can be used to manage the obtained data?
    Who can access the collected data?
    What will be the expected rate of data growth over the next five years?




We highlight the distinctive design primitives that we believe should be addressed in an IoT data management solution, and discuss how they are approached by the proposed solutions. 




In this paper, we highlight the data management lifecycle from the perspective of IoT architecture and show why it should be different from traditional data management systems. 






The integration of cloud environments with "edges” resources that combine both processing and storage elements











Devices generate and consume data, gateways provides low-latency low-performance storage and processing capabilities, and clouds provide high-latency high-performance storage and processing capabilities.









Devices: communication-intensive

Gateways: communication-intensive, process-intensive, storage-intensive

Cloud: process-intensive, storage-intensive.

![IoTA_gateway_model_figA_desktop](https://www.cloudtp.com/wp-content/uploads/2016/06/IoTA_gateway_model_figA_desktop.png)



Both offline and real-time data cycles need to be supported in an IoT Gateways, to accommodate the various storage and processing needs of potential IoT scenarios. 





An FMEA can be a qualitative analysis,[1] but may be put on a quantitative basis when mathematical failure rate models[2] are combined with a statistical failure mode ratio database. 



As IoT networks proliferate and use cases expand, the demands on IoT gateways for these capabilities will only intensify.







It takes less time for a device to send data to a nearby server (outer tier), but the storage and processing capabilities are limited. Also, servers located away from central data-centers are prone severed connectivity to data networks and power sources. On the other hand, the closer a server is located to the Cloud (inner tier), the greater the capabilities and stability it offers, but the data transfer time increases as well.  

Outermost to Outer tiers -> lower inter-tier latency, lower intra-tier bandwidth
Outermost to Innermost tiers -> high inter-tier latency, high intra-tier bandwidth






Tail latency volatility, for example, is fueled by packet delay, jitter, packet loss, and other problems 

 either at the concentration points or at the autonomous virtual units within the IoT

Wired or wireless broadband communications may be used there to transfer data to permanent data stores.







![IoTA_gateway_model_figA_desktop](https://www.cloudtp.com/wp-content/uploads/2016/06/IoTA_gateway_model_figA_desktop.png)








Additionally, they have the ability to discover and engage  "Things" in their vicinity.

An access network is a type of telecommunications network which connects subscribers to their immediate service provider. It is contrasted with the core network, which connects local providers to one another

fectively offers a trade off between increased storage and processing resources, at the expense of high-latency access to the data, and vice-versa. 



Having many different devices connected directly to cloud services presents a huge attack surface, which can be mitigated by channelling data through a secure gateway device.

Due to the multi-faceted operation of Gateways it is difficult to classify their lifecycle as communication-intensive or storage-intensive. When acting as a frontend that forwards data over Things and Clouds, it is apparently communication-intensive. it is storage-intensive. However, under circumstances, query processing can be considered more communication-intensive than storage-intensive, as they provide real-time data to certain queries. 













%Some experts classified the three-tiers in the IIoT system as edge, platform, and enterprise and these are connected by proximity network, access network, and service network, respectively.

LAN



An access network is a user network that connects subscribers to a particular service provider and, through the carrier network, to other networks such as the Internet. Some types of access networks: Ethernet is the most commonly installed wired LAN (local area network) technology.

A service network is a structure that brings together several entities to deliver a particular service

Networks where the physical proximity of a user to a network makes immediately available a local service environment






  On the surface, these streams are completely incompatible as they may be presented in many forms from electrical signals to IP-data. 






Automated tiered storage (also automated storage tiering) is the automated progression or demotion of data across different tiers (types) of storage devices and media. The movement of data takes place in an automated way with the help of a software or embedded firmware and is assigned to the related media according to performance and capacity requirements. More advanced implementations include the ability to define rules and policies that dictate if and when data can be moved between the tiers, and in many cases provides the ability to pin data to tiers permanently or for specific periods of time. 

 

 Network characteristics are possible the worse thing to overlook when considering tiered architectures. 



is all about handling a buffer with a finite number of packets waiting for an action.






Preprocessing: IoT data will come from different sources with varying formats and structures. Data may need to be preprocessed to handle missing data, remove redundancies and integrate data from different sources into a unified schema before being committed to storage.

Processing/Analysis: This phase involves the ongoing retrieval and analysis operations performed and stored and archived data in order to gain insights into historical data and predict future trends, or to detect abnormalities in the data that may trigger further investigation or action. Task-specific preprocessing may be needed to filter and clean data before meaningful operations take place. 



He wrote the bible on using mathematics to set up communication systems, thereby laying the foundation for the digital age. 





  in an adaptable, flexible, and seamless data network.









Additionally, space has to be optimised for 



Storage operations aim at making data available on the long term for constant access/updates, while archival is concerned with read-only data.







to reduce time for storage










sophisticated application needs of an IoT network that needs to  





As such, no competing solution can offer the same performance on 



Current solutions for IoT data management address partial aspects of the IoT environment with special focus on sensor networks. 

resources available through the individual and any subsystems designed to manage the aforementioned “Things”. 

A data management framework for IoT is presented that incorporates a layered, data-centric, and federated paradigm to  

pushing it up the network to aggregation points and subsequently to database servers, or sending it as a response triggered by queries that request the data from sensors and smart objects. 







Any  relevant design should originate from these field tests,  point and discuss how the  emerging "techno-natural" monopolies should be treated today in general. Otherwise, the critique will fall very short and be any easy target to  the kind of arguments that you are referring to. I think you have been  aware of this point but somehow this movement missed it.

Data from the field tests helps improve the design and create a higher-quality solutions.



Edge devices run a Web-based dashboard that end-users can access to monitor the flow of data, so they can decide how various systems in demonstration and devices are running, and get notified by alarms



field dictates



Functions such as adaptive maintenance, predictive repair, 

IoT device data also need to be checked for quality. 



Much of the IoT initiatives are geared towards manufacturing low-cost and energy-efficient hardware for these objects, as well as the communication technologies that provide objects interconnectivity.






However, as we describe later in this post, containers exist in a  twilight zone somewhere between hosts and applications where neither  application performance monitoring nor traditional infrastructure  monitoring are effective. This creates a blind spot in your monitoring,  which is a big problem for containers and for the companies that adopt  them.



Easily create full-stack installers for your project across a variety of platforms.    



Typically, the container infrastructure is not as dynamic as containers. Stretching the compute capacity of the container infrastructure can  happen quite quickly. 



To manage this, you’ll likely want to use [Kubernetes](http://kubernetes.io/) or [AWS ECS](https://aws.amazon.com/ecs/) to move from manual, imperative provisioning to autonomic, declarative  provisioning. This allows you to say, for example, “I need one container of type X per instance per zone, at all times,” and your scheduler will make sure this is always the case. This kind of automation is necessary for modern container architectures, but opens the door to fresh new  kinds of chaos.



Where to start:

- Start with small workloads which you can easily measure
- Monitor your changes and adjust accordingly
- Rinse and Repeat for other containers/services













But one thing you might not have much experience with is understanding how Docker containers behave under different loads.

Because Docker containers, from the outside, can look a lot like  black boxes, it's not obvious to a lot of people how to go about getting runtime metrics and doing analysis.

In this post, we will set up a small CrateDB cluster with Docker and  then go through some useful Docker commands that let us take a look at  performance.



 has distinctive characteristics that make traditional data management systems an obsolete solution. 








 For one example, consider an apartment complex equipped with a network  of ZigBee-based fire-detection and entry sensors: Data is compiled and  stored in a local ADSL intelligent gateway that periodically reports to a security company. The gateway would be programmed to immediately raise  an alarm when the system detects an abnormal sensor response. 



While cellular and WiFi are quite common wireless standards, emerging  low-power wide-area networks (LPWAN), such as Sigfox, LoRa and PLANet,  are relatively new standards optimized for IoT/M2M communication. Unlike traditional cellular networks, LPWANs are optimized for low data rates, long battery life, low duty cycle, and the ability to coexist in a  shared spectrum using unlicensed ISM bands. An example is in city street lamp lighting systems, which tend to be in place for decades, far  longer than typical cellular standards are in force.



To facilitate future development, standards are quickly forming and evolving as new devices become connected. 



Gateways will increasingly use standard interfaces to devices and to  the cloud, but the amount of intelligence they’ll need will depend on  specific applications. One key to rapid deployment of custom gateways is the availability of test gear flexible enough to meet the needs of  engineers across R&D, manufacturing and deployment.



 To understand  this flexibility in this context, consider an example: Early in product  development, engineers can run 
 
 
Once prototypes are available, engineers can make use of lab-grade  test equipment, which generally has built-in measurement applications  that can show whether the prototype performs to standards. For custom  gateway products, engineers can do pre-qualification testing for each  supported format to verify the product will meet the relevant  specifications, including interoperability with other communication  standards.










“Things” are expected to communicate among themselves and interact with the environment by exchanging data generated by sensing (sensors), while reacting to events and triggering actions to control the physical world (actuators). 


For one example, consider an apartment complex equipped with a network of ZigBee-based fire-detection and entry sensors: Data is compiled and  stored in a local ADSL intelligent gateway that periodically reports to a security company.


 




Today, an IoT “thing”  is any entity can be any natural or man-made entity, fixed or mobile, able to transfer data over a network. It’s likely that a majority of IoT things will rely on some kind of  wireless communication technology. 



Gateways traditionally have been used as a communication frontend responsible for  translating protocols and handling data flow seamlessly and securely from individual devices the cloud. 



In many  instances, there is no direct connection between the thing and the  cloud, or the remote application that needs to communicate with it.







For example, Gateways can ingest, store, filter, index, process, and possibly 



Weave Net creates a virtual network that connects Docker containers  across multiple hosts and enables their automatic discovery. With Weave  Net, portable microservices-based applications consisting of multiple  containers can run anywhere: on one host, multiple hosts or even across  cloud providers and data centers. Applications use the network just as  if the containers were all plugged into the same network switch, without having to configure port mappings, ambassadors or links.

Services provided by application containers on the Weave network can  be exposed to the outside world, regardless of where they are running.  Similarly, existing internal systems can be opened to accept connections from application containers irrespective of their location.









provision of a standard platform for developing  cooperative services and applications.

available devices and networking options, 

efficient usage of multiple-tier offerings

heterogeneity of IoT devices,  adaptation to non-standard communication layers, and 

, networking, and  configuration—in fact [there](http://kubernetes.io/) [are](https://mesos.apache.org/) [many](https://github.com/coreos/fleet) [active](https://github.com/zettio/weave) [software](https://coreos.com/blog/introducing-rudder/) [projects](https://opsbot.com/advanced-docker-networking-pipework/) [addressing](https://coreos.com/using-coreos/etcd/) [these](https://www.digitalocean.com/community/tutorials/an-introduction-to-using-consul-a-service-discovery-system-on-ubuntu-14-04) [issues](https://zookeeper.apache.org/).






In this architecture, IoT data will roam the network until it reaches concentration storage points (Clouds or Gateways) where it will finally statically reside in fixed- or flexible-schema databases. 




 ingest the massive volume of IoT data and make . The reasons are fundamental and have to do with their "flat" (single tier) architecture, and the design assumption that such systems will operate in 





# Bonus Topic: Flaky Tests

 The reasons can be  several:

- State from the previous tests that are passed on to the next tests
- Infrastructure issues such as low memory of the machine running the test, especially when using emulators
- Animations that are not very well managed by the test tools
- Thread Concurrency Issues
- And others…

The big problem with intermittent testing is that they take away the  reliability of your suite and greatly disorder the continuous delivery  process. So I will mention some tips that can help mitigate this issue  on Android:





End-to-end testing is a technique  that tests the entire software product from beginning to end to It defines the product’s  system dependencies and ensures all integrated pieces work together as  expected.

The main purpose of End-to-end (E2E)  testing is to test from the end user’s experience by simulating the real user scenario and validating the system under test and its components  for integration and data integrity.

Software systems nowadays are complex and interconnected with numerous subsystems. If any of the subsystems  fails, the whole software system could crash. This is a major risk and  can be avoided by end-to-end testing.

The reasons are fundamental since 

## **Benefits of End-to-End Testing**

End-to-end testing has been more reliable and widely adopted because of these following benefits:

- Expand test coverage
- Ensure the correctness of the application
- Reduce time to market
- Reduce cost
- Detect bugs 



 Deploying into the wild Internet a data management system that is designed for data-centers, can cause intriguing failures that may jeopardize key aspects of a system's operation. This can consist of an overload of concurrent requests, unintended traffic storms due to write/read amplification, degraded performance due to impertinent networks, or cascading timeouts due to tight coupling of software. 
 
 
 
 Traditional gateways have mostly performed device management functions, protocol translation, and propagation of query requests and results to and from Things. 
 
 
 
 
 
 http://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.492.8359&rep=rep1&type=pdf
 
 
 

create virtual testing environment in order to evaluate its behavior under controllable conditions.


evaluate their systems in software-defined environments that replicate the infrastructure layer of complex IoT systems, at real-time.


s. IOTier is a distributed emulator used to replicate the conditions of the uncontrolled IoT environment into a containerized environment, where developers can objectively measure the impact of hardware, network, data storage and data management systems, to the application-perceived performance. 


an IoT system to be immersed and tested in a 




Open modeling language to create custom domain models of any connected environment using Digital Twins Definition Language

Live execution environment to bring your digital twins to life in a live graph representation

Input from IoT and business systems to connect assets, including IoT devices, using Azure IoT Hub, Logic Apps, and REST APIs

Output to Time Series Insights, storage, and analytics using event routes to downstream services including Azure Synapse Analytics






multi-phase experiments, IOTier makes a grounded framework that automates the testing and evaluation of complex IoT systems. It also serves  and applications (e.g, haptics, video, voice). 




It also provides minimum flexibility on experimenting with 

which connectsa diverse set of devices over different transport layers, usinga variety of protocols. Provisioning a virtual testbed of IoT devices can accelerate IoT application development by enabling automated testing without requiring a continuous connection tothe physical devices

This, however, increases the complexity of IoT systems and calls for a flexible testing environment to simplify the development process. 

testing of lower-level layers of the IoT system. For instance, testing system scalability is not limited to processing data on the application level, but also 


create tests with custom stacks,

ntroduces a framework for benchmarking organisations ± ``evolutionary benchmarking’’.
As the complexity of a distributed system increases, it eventually reaches a point where no single individual can reasonably understand the entirety. At this point, when the interactions between components are unpredictable, the system becomes chaotic. 

It generates new knowledge and often suggests new avenues of exploration. 

thus leading to stronger and more resilient systems.



Use Experimentation to answer "given a system, what infrastructure is required to attain desired properties". Use testing to answer "given an infrastructure, what system better attains the desired properties ?"



    
    In this framework, operators can systematically define the different phases of an experiment, and control how the testbed topology changes in each phase. This framework represents a significant new vision for event-based experiments as it (1) helps to keep pace with the rapidly multiplying testing scale of networked systems (2) automates exploration of large design spaces, and (3) facilitates root-cause analysis as well.



 %To emulate the passing of control from access point (AP) to a client station (STA) and vice-versa, control has to be passed between queues within the emulator. Passing of control within NetEm is difficult because the emulator needs to be fast enough to keep up with real data transmission speeds and robust enough to forestalllock up. 







designed to implement end-to-end IoT Testing by covering all protocols required by IoT Applications, Middleware, Brokers, Load Balancers, MQTT gateways and clients.




Provisioning a virtual testbed of IoT devices can accelerate IoT application development by enabling automated testing without requiring a continuous connection to the physical devices.



Running benchmarks and stressing the applications is in the essence of a performance engineer. In its current form, however, it remains a manual process whose instrumentation consumes valuables resources and time. While there exist several workload generators, monitoring tools, and virtualization platforms, there are no realistic and proven testbeds to automate the evaluation of distributed applications. 


 Benchmarking is about measuring the performance of a specific system's configuration, IOTier is the missing link for experimenting with several different configurations, in a manageable way. 




Using IOTier, we effectively replicated variable IoT conditions and measured their impact to both common and uncommon path operations. 

A testbed is a platform for conducting rigorous, transparent, and replicable testing of scientific theories, computational tools, and new technologies




Foundry enables users with varying technical ability and deep subject matter expertise to work meaningfully with data.

With the testing scale rapidly multiplying, software-defined Virtual 


for testing complex IoT systems inside flexible, software-defined environments Our framework, called \ac{IOTIER}, is designed to bring the best of emulators and simulators into an integrated tool. 



In effect, flexible ingestion, indexing, and aggregation of large streams of real-time data from numerous devices require next-generation IoT systems to be designed with tiering in mind. 

. Factors such as hardware in IoT components, inter-tier and intra-tier communication, as well as the software's tight coupling, create challenges that are like to hinder the functionality of IoT systems. 

The Internet of things (IoT) describes the network of physical objects—“things”—that are embedded with sensors, software, and other technologies to connect and exchange data 
, over different transport layers, using a variety of protocols. 


  This is why we built TiPocket, a fully-automated testing framework based on Kubernetes and Chaos Mesh. Currently, we mainly use it to test TiDB clusters. However, because of TiPocket’s Kubernetes-friendly design and extensible interface, you can use Kubernetes’ create and delete logic to easily support other applications.


 
 
 %Network emulators, e.g., a Linux traffic controller known as NetEm, can model a wired network performance in real time or nearly so. However, to model WiFi over a wired network emulator such as NetEm, queues at nodes have to be coordinated such that when one queue transmits, the other queues pause

 
 Discusses the concept and operation of th e framework, alon g with its proposed advantages in aidin  gbenchmarking. The benchmarking approach proposed utilises an evolutionary classification methodcalle  d cladistics. Use  s an example classification of automotive assembly plant   s to sho  w ho w theproposed framework help  s benchmarking in term  s of: providing a framework for representingbenchmarking information; enhancing the quality and validity of the information according to theclassification rule  s of parsimony, congruence an d homology; and providing a comparison tha tindicates ho w the practices shoul  d be adopted. Thi  s framework is considered to  be usefu  l toresearchers wh o stud y benchmarking methodologies an d thos e tha t categorise the findings ofbenchmarking studies.
 
 Fierce competition, globalisation and th e development of  new information andcommunication technologies have forced organisations to continuously search fo rand adopt new configurations (processes an d structures) by which to exi
 
 To   catalogue such diversity and to facilitate learningbetween  different  configurations  requires  a  classification  of  som  e  s
 
 Helios also serves as a reference blueprint for other large-scale systems within Microsoft.


Engineers can therefore emulate IoT components, structure IoT components into dynamic IoT testbeds that can be dynamically altered, specify how the experiments evolves over time, 

While the testing scale is rapidly multiplying, systems evaluation remains a painfully manual process. 


Hence, if we want to to recreate the actual conditions of a network protocol, such as 4G, 80211, or Fiber, 

and providing a comparison that indicates how the practices should be adopted. This framework is considered to be useful to researchers who study benchmarking methodologies and those that categorise the findings of benchmarking studies


%In other words, to encode domain knowledge for specific production environment behaviors, and validate a system against that environment. 


6.1. Linux-Based Devices. The Linux operating system pro- vides a hardware abstraction layer to user applications. 




Having a key/value database as a reference, we 

evaluate the impact of 

We use the above building blocks to create a proof-of-concept testbed and evaluate s of , including impact of 



such as 


Using these building blocks, IoT and storage engineers can easily replicate IoT tiered infrastructures, with every tiers consist of different devices, network protocols, and operating conditions. 


IoT data management systemthe product






pose significant challenges in testing new ones. Performing tests in real-world IoT platforms is expensive, require the maintenance of hundreds of different devices, and provide few means to assess the baselines a system presents. 


The trade-off and the collaborative behavior of tiers  creates a web of complexity to connect the different tiers and their data streams. 




simulations that include virtual  measurement tools. These can attach to nodes in the simulation,  As the design moves from simulation to reality, physical device modules can be  substituted into the simulation, and real measurements replace their  virtual simulations.




The trade-off and the collaborative behavior of tiers  creates a web of complexity to connect the different tiers and their data streams. 


Sitting at the intersection of containerization, chaos engineering, and simulation, 




Using a combination of IFB and TC, we can track opened connections on the server, and (1) balance the traffic between them (2) put traffic into classes, and define the minimum and maximum bandwidth settings for those classes.  









Docker-Compose and Docker-Stack are based on the same configuration file. Depending on the experiment, we distilled two different methods for using the cluster. 


 a tool for running multi-container applications on Docker defined using the Compose file format. 
 
 
 
 
 
 
 
* **Assymetry:** Observing both the download and upload speeds, it is clear that fiber  service tiers are generally symmetric in their actual upload and  download speeds. This results from the fact that fiber technology has  significantly more capacity than other technologies and it can be  engineered to have symmetric upload and download speeds. For other  technologies with more limited capacity, higher capacity is usually  allocated to download speeds than to upload speeds, typically in ratios  ranging from 5:1 to 10:1. This resulting asymmetry in download/upload  speeds is reflective of actual usage because consumers typically  download significantly more data than they upload. 

  It should be noted that while upload and downloads speeds are measured  independently and shown separately, they are typically offered by an ISP in a paired configuration. Together, these plans serve the majority of Internet users of the participating ISPs.




\paragraph{Geographical distance}

Leaving aside contributing processes and devices, the end-to-end latency between a sender node and a destination node is dominated by the propagation delay, which depends on the geographical distance between the nodes. 

\todo[inline]{Use distance labels to emulate geographica locality}










    

















\subsection{Calibration}


    
    \item Does the namespace partition improve or worsen the per client performance ?
    
    
    
    how long does it take the performance of a database to recover after resharding

help to improve 


# Evaluation

What is the impact of transient clients on long-running clients when deployed on the same database node ?

    


With percentile value we can intuitively characterize this system:

1. Around 900 DNS resolution will happen below `0.59s`
2. Around 90 DNS resolution will take between `0.59s` to `0.66s`
3. Around 10 DNS resolution will go beyond the `0.66s` .



## Calibration

The first step in validating our virtual TestBed is to stress emulated building blocks and  ensure that the defined limits are respected.  We measure building block in isolation, using standardized tools in their categories. In particular we use iperf for network emulation, fio for block device emulation, and XXX for CPU emulation.  For memory no particular stressing as it is statically allocated.

## Baseline

In the next step, 

* CPU
* IOPS
* Memory
* Network

## Contention

* Server load 
* Multiple clients

## Partition

* Evaluate the effect of a client sending traffic to multiple servers

* Static number of servers
* Same tier

* Different tiers

## Load Balance

* Like partition, but with dynamic servers

## Replication

* Evaluate the impact of replication to the tail latency
* Intra-tier replication
* Inter-tier replication





| Experiment     | Path     | Topology | Description                                    |
| -------------- | -------- | -------- | ---------------------------------------------- |
| Link type      | Common   | Fixed    | Link changes between client-server             |
| Partition Size | Uncommon | Fixed    | Client link to number of (unthrottled) servers |
| Migration      | Uncommon | Phases   | Servers added in phases                        |
| Replication    | Common   | Fixed    | (Unthrottled) clients to (throttled) servers   |
| Contention     | Common   | Phases   | 1 Server, Clients added in phases              |
| Tiering        | Common   | Fixed    | Clients send to various links                  |





##### Network Policy Enforcement

* For multi-client experiments we use iperf2 since iperf3 supports single-client. 



<img src="https://lh6.googleusercontent.com/HSwkcEI54RssIc_Wvt02xyqsVzBOHkE2OkVWEn2Y5g_zRfC1P4nJjSE2fQmOnNnepSdnXfKAfE5nniDSNCpisSgHsKE1504heOmGf_YACzRG30bTjZurghBS098hG1ZyqTVON5IRAVY" alt="Chart" style="zoom:50%;" /> <img src="https://lh4.googleusercontent.com/XuyTQBr4OnkOHJfmwtAp1bPGlk6hNVe9qIEk8_eib1lFeX1KEJPA-wzy39CUcBtf02s8VsJj-_PCUOl0bvvSfidEqtX6DyPKdhpoALdTuW0cO7J2DCCNKOr6ReFGUc88ZROW52zSBxA" alt="Chart" style="zoom:50%;" />


 

* **Units:** Network data rates are typically measured in bits per second (bps),  whereas data rates for non-network equipment are typically shown in  bytes per second (Bps). This is a common source of confusion, pay close  attention to the units. For example, to put a 10 megabyte (MB) file "on the wire" over a  1Mbps link, we will need 80 seconds. 10MB is equal to 80Mb because  there are 8 bits for every byte!    





  

* Throughput 
  * Iperf



* nping
  * To go all the way to the stack

Gns3's VPCS clients can ping using UPD or TCP. Why can't Ping on Windows,  Cisco or Linux do that? Sometimes it's necessary to see if UPD packets  can reach the destination.

 

Or sometimes even when we can ping with ICMP to make sure a destination  host is online, the really needed communication protocol between the  applications is UDP ehich might have been blocked on a firewall in  between.





###  Benchmark Workload



YCSB stages are split into different containers categories

Load: run on the "cloud" tier so to populare the database as fast as possible

Run: runs on the "edge" as it would normally happen

**recordcount**: the number of records in the dataset at the start of the workload. used when loading for all workloads. (default: 1000)

**operationcount**: the number of operations to perform in the workload (default: 1000)





TPC Express Benchmark IoT (TPCx-IoT) Specification Version 1.0.513 IoT workloads consists of data ingestion and concurrent queries simulating workloads on typical IoT Gateway systems. The dataset represents data from sensors from electric power station(s).The data ingestion and query workloads are detailed in the following section.



* **Record: **Each *record* generated consists of driver system id, sensor name, time stamp,sensor reading and padding to a 1 Kbyte size. The driver systemid represents a power station. 
* **Dataset**: The dataset represents data from 200 different types of sensors
* **Replication**: TheSUT must run a data management platform that is commercially available and data must be persisted in a non-volatile durable mediawith a minimum of two-way replication.  



The TPC Benchmark IoT (TPCx-IoT) benchmark workload is designed based on Yahoo Cloud Serving Benchmark (YCSB).



* Depth-first (number of tiers) and Broadth-first (tier capacity)



YCSB values are taken from TPCx-IOT benchmark



## Latency



## Distributed YCSB

**Measuring tail latency for multiple clients**

* Phase 1: Run for M minutes and notify  Phase 2
* ...
* Phase N-1: Run for M minutes and notify  Phase N
* Phase N: Run for M minutes and complete
* 







## Databases



### TIKV

* TIKV depends on Two-phase commit (Percolator)
* Storage nodes use Placement Drivers (PD) as the timestamp  oracle 
  * Because timestamps server as transaction ID, nodes must contact PD for every new transaction
  * **THIS WILL BE GREATLY IMPACTED BY DELAY**



# 

Generally, all communication takes a few milliseconds, but every once in a while, some packets take a few seconds. The packets that take a  few milliseconds generally belong to the 90th percentile or higher of latencies. Long tail latencies occur when these high percentiles begin to have values that go well beyond the average and can be magnitudes  greater than the average. Thus average latencies only give half the  story. 


Longtail latencies affect members every day and improving the response  times of systems even at the 99th percentile is critical to the member's experience. There can be many causes such as slow applications, slow  disk accesses, errors in the network, and many more.



- **Bandwidth:** Maximum throughput of a logical or physical communication path

- **Delay:** the amount of time it takes for the first bit to travel over a link between the source sending a packet to the destination

- **Latency:**  the total amount of time it takes to send an entire message.
  - Because latency depends on the receiver's processing capabilities, for the links we are mostly interested in the delay.


\subsection{Plan-Interconnection}

\subsection{Plan-Partitioning}

\subsection{Plan-Availability}
A cloud database must be highly available despite failures,and the Availability tier measures the impact of failures on the system. The simplest way to measure availability is to start a workload, kill a server while the workload is running,and observe any resulting errors and performance impact. However, in a real deployed system, a variety of failures can occur at various other levels, including the disk, the network, and the whole datacenter.


\subsection{Plan-Contention}
Single experiment, multiple phases, at each phase change number of clients 

\subsection{Plan-Replication}
multiple experiments, Single phase,  at each experiment change number of replicas 

\subsection{Plan-Migration}

Add new server, remove server

\subsection{Plan-Tiering}

% Device performance (fixed)
Constrained Memory
Constrained Memory + CPU
Constrained Memory + CPU + IOPS 

% Network effects (fixed)
Constrained Bandwidth
Constrained Delay
Global namespace in tiering

% System performance (Dynamic)
99th on Rebalancing
99th on contention



\subsection{Memory equal to 20\% of the dataset for Zipfian}




In our testing framework, we:
    Observe the normal metrics and develop our testing hypothesis.
    Inject a list of failures into TiDB.
    Run various test cases to verify TiDB in fault scenarios.
    Monitor and collect test results for analysis and diagnosis.
    
    
quantify the  consequences of work deferment and the benefits of anticipatory configu-ration optimization such as B-tree pre-splitting or bulk load-ing, and abstract APIs for explicit incorporation of advanced features in benchmark tests.







But the sheer number of communication, storage and processing options, creates a web of complexity to the creation of systems that 



 and applications that . Opting for a tier entails a tradeoff between increased storage and processing resources, at the expense of high-latency access to the data, and vice-versa. 

 
Hence, in order to distribute optimally the computation and storage tasks across IoT tiers,  it is not only necessary to know how the system behaves in various circumstances, but also to understand a tier's trade-offs, at both the coarse-grained service level and fine-grained device level. There is the need to 


Yet, with the increasing demands for real-time processing and analysis, the logical solution  would seemingly be upgrade the role of Gateways from communication-frontend to functionality frontend.



But with the sheer number of IoT device increasing disproportional to the available bandwidth, it becomes prohibitively expensive to transfer raw to centralized Clouds. 

However, the processing and storage capabilities of Gateways remain limited in comparison to the Cloud servers, for reasons related to manufacturing cost and energy-saving.









IoT data will roam the network until it reaches concentration storage points, where it will finally statically reside in fixed- or flexible-schema databases. The in-network processing may be performed in response to real-time events, localized queries, or for data whose value degrade by time and  there is no need to propagate this data further up to concentration points in the system.   "Things" and Gateways may store the data for a certain time interval, so when there is no connection, they will still gain insights, make decisions and prepare for data distribution. However, due to the limited capabilities of such objects, storage capacity remains limited in comparison to the centralized storage model. 




Opting for a tier entails a tradeoff between increased storage and processing resources, at the expense of high-latency access to the data, and vice-versa. Communication, storage and processing capabilities will thus be defining factors in the design of data management solutions for IoT. 











You have a hot tier, that’s probably made of NVMe flash or something expensive. You have a cold tier that’s made out of hard drives and lower cost technologies. Then you have the storage management software layer that’s moving data back and forth. What do you get out of that? You get unpredictable performance. If you have guessed right, or your data has been recently used, then it’s in the hot tier [and] performance is not bad. If you guessed wrong or the workloads have changed or the compute cluster is overloaded, the data is still in the cold tier, and your nodes are idle while you’re pulling data up to the hot tier,” said Anderson.
 






%By processing and storing data closer to the data source, we can minimize the large volume of message exchanges that translate into communication overhead and latency, and therefore reduce energy footprint and maintenance of inoperative data stored in data centers. 




interacts directly with the

via a communication layer, while Cloud is  an offline backend that handles the  of IoT data.

While tiering is in constant decline within data centers, it is a rising start for the 





Traditionally, 

 As the IoT has both real-time and historical data stored, it can provide effective decision-making instructions to devices, and control certain actions and aspects of when and how they function.
 
 Lately, it seems like every application or device is somehow connected to the cloud, whether it’s storing data, processing, or working in the cloud. 
 
 
 
 
 
as happens with any architectural shift, this means new data management challenges come to surface. 


All the above create a web of complexity that makes


However, siloed data across these experiences makes it challenging to build digital twin solutions that bring those models to life, and doing so in a scalable, secure way is often time-consuming.




--and incorporate the new knowledge into the design of new architectures--

Snell pointed out in shaping the discussion, “The implementation of solid state or flash storage has continued to grow among HPC users, and in most cases it exists together with, not separate from, conventional spinning disk hard drives. Having data on the right tier at the right time has become a compelling conversation point in determining what constitutes high performance storage, together with the potential latency and moving data between tiers. Meanwhile, the need for long term data stewardship is no less important. 

 
 

 
 “This is an example of temperature based data placement, how recently something has been accessed, determines where it lives, unless you’re reaching in and manually managing where data lives which has its own set of costs and issues,” he said.



Using what he called a single tier approach, where data placement is based on size using a mix of technologies, is the key. “Comparing HPC storage products is difficult, because there’s such wildly different hardware.


the network parameters of real devices, such as bandwidth, transmission delay, addressing, and many more.


where different sensors may produce high amounts of data or where critical system functionalities must be ensured during access network problems. 


The heterogeneity within the IoT domain necessitates a highly flexible, secure, dependable, and energy-efficient IoT processor architecture. In this paper, we propose a novel processor architecture for IoT that renders energy efficiency, 
With the increasing streaming rates and the limited bandwidth, it becomes prohibitively expensive to transfer raw data generated by millions of devices to centralized Clouds. Yet, the geographical distance between them is an unsurpassed obstacle to real-time processing and analysis. 





not only necessary to learn how a system behaves in various circumstances but also to experiment


design and testing a challenging endeavor.  Through experimentation researchers can answer complex question such as 

To answer questions like the above, we have created a Virtual Testbed that can emulate tiered IoT infrastructures through the 



%There is no such thing as an IoT communication standard, so networks  will need to cope with numerous devices having different communication  requirements. At one end will be simple wireless devices such as battery-powered sensors and actuators that will transmit little data  while operating unattended for several years. At the other end will be high-bandwidth, mission-critical services and devices such as autonomous cars demanding constant, reliable and super-secure connections.

in which engineers can model and execute 



that provides the following building blocks: 


Our testbed replicates fundamental offerings that cover many of the outlined tiers, they should provide the following building blocks:
\begin{itemize}

\item real-time emulation of numerous IoT devices ;

\item emulation of dozens of network protocols  ; 

\item orchestration of distributed testing environments with hundreds of IoT devices and networking options, intermixed in arbitrarily complex network topologies (e.g, star, bus, tier).

\item an event-based engine in which operators can script scenarios that express the environment's evolution over time, and continually maintains the current state of the testbed in sync with the desired state.

\end{itemize}
\ac{IOTIER} can be used for both experimentation and benchmark testing. 


how many clients is it better to replicate state across gateways 



 engineers to optimize their database operations through data analysis and gather feedback to develop and test advances in wind turbine development.


Azure Digital Twins Preview is an Azure IoT service that creates comprehensive models of the physical environment. 



 

Databases, or in general storage systems, that , fall short in handling 

In turn, this requires storage engineers to validate their solutions against diversified infrastructures characterized by 

be able to change the hardware, 


Concerning experimentation, \ac{IOTIER} can stimulate events in recorded order, change the state of the runtime environment, and provide the means to analyze the effect of these changes on the applications. 





This way, 

 are fundamentally inadequate for operation

As extant systems  

designed for operation within data-centers

are . They typically depends . As such, they 

Well known challenges include 






%-- Solution
 
search for applicable solutions from the best in class. 


% Programmable testbeds 


%
% To perform complex processing on IoT data Gateways need to be more powerful than Things.


%can answer complex question that frequently occur in real-world production environments, such as "how much is the tail latency of long-running clients affected by transient clients", "what is the latency variance (jitter) during load balancing ?"

 



% The Gateway tier is a real-time frontend that interacts directly with the interconnected IoT devices. 
%The core of Cloud storage is the deployment of storage structures that handle the efficient organization and persistence of large amounts of data as well as the integration of continuous updates of data as it becomes available. Data is usually time-stamped or geo-stamped and can be in the form of simple key-value pairs, or it may contain rich audio/image/video content, with varying degrees of complexity in-between. Furthermore, there is metadata that describes “Things” or Gateways themselves (e.g, object identification, location, running services).


%But to create testbeds with more than one container operators have to handle manually several Dockerfiles, Networks, TC rules, Resource assignment, and so on. All these configurations can add on the load of maintaining them, is time-consuming, and forfeit 

%By default, all containers have networking enabled and they can make any outgoing connections. 


% It is an

%Originally, this mechanism was designed to uniformly throttle disk I/O throughput across all containers without actually imposing any kind of stress on other resources (i.e. CPU) on the machine.

%By design, FIFO does not shape anything, and if there is a connection that eats up all of the bandwidth, FIFO will not stop it from doing so. Other common disciplines to shape, classify, and prioritize traffic, include PFIFO, which works more or less as FIFO enhanced to prioritize certain packets, or Token Bucket Filter (TBF), which shapes traffic to conform to a configured output rate and burstiness. 


%The random behavior of a real-time WiFi network is effectively shaped by burst patterns, e.g., by the probability distribution of slot intervals under various noise conditions. In this manner, WiFi models can be studied for their effect on latency in live application sessions, e.g., gameplay sessions, conferencing sessions, etc. Such studies can also include components that request participants to rate their perception of performance. The results of such a study can be used towards better network design, improving user experience, etc.

% Among the advantages of  benchmarking is


% t establishes pragmatic goal   s base  d on  a concerted vie w of externalconditions 

%It provides significant leaps in performance no t always attained by other management techniques


%Benchmark Testing is used to validate the product value of the system software application or the web-based software application, against the regulations set by the development team or the system architecture, in order to maintain or enhance the reputation of the application. This product value determination process involves various testing flow, depending on the regulations fixed for the application. In most cases, it is achieved by exposing the application for a round of performance testing.


%The wisdom behind this process is to observe and identify systematic weaknesses, and once one area of concern is resolved, reset the testing criteria or parameters and run the experiment again with a new hypothesis. Developers can also expand the blast radius by incremental testing, introducing new or more powerful stressors into the testing environment in order to gauge the limits of the system. The more difficult it is to disrupt the steady state of the challenge group, the greater the confidence developers can have in the strength and integrity of their applications.


% One approach is to allow each database request to carry aspecial fault flag that causes the system to simulate a fault.This approach is particularly amenable to benchmarking be-cause the workload generator can add the appropriate flagfor different tests to measure the impact of different faults.A “fault-injection” header can be inserted into PNUTS re-quests, but to our knowledge, a similar mechanism is notcurrently available in the other systems we benchmarked.An alternate approach to fault injection that works well atthe network layer is to use a system like ModelNet [34] orEmulab [33] to simulate the network layer, and insert theappropriate faults.The second difficulty is that different systems have dif-ferent components, and therefore different, unique failuremodes. Thus, it is difficult to design failure scenarios thatcover all systems.Despite these difficulties, evaluating the availability of sys-tems is important and we are continuing to work on devel-oping benchmarking approaches.




% Create custom test stacks A broad-stack test is a test that exercises most of the parts of a large application. It's often referred to as an end-to-end test or full-stack test. It lies in contrast to a ComponentTest, which only exercises a well-defined part of a system

%Broad-stack tests have the advantage of exercising the application with all its parts connected together and thus can find bugs in the interaction between components in the way that component tests cannot.

 %Test Double (think stunt double). Test Double is a generic term for any case where you replace a production object for testing purposes. 
 
 
 


%The workload is representative of activities typical in IoT gateway systems, running on commercially available hardware and software platforms. The TPCx-IoT can be used to assess a broad range of system topologies and implementation methodologies in a technically rigorous and directly comparable, in a vendor-neutral manner. 



% -- Problem Statement
%With no solution being really mature yet, a fundamental question raises: 

%Also, Yet, to create an IoT-based system, it is not necessary 


Data can be classified into periodic observations about certain monitored phenomena and reports of abnormal events of interest. Periodic observations are most demanding in terms of communication overhead and storage due to their streaming and continuous nature, while events present time-strain with end-to-end response times depending on the urgency of the response required for the event.






In this paper, we study the feasibility of bringing some  as virtualized, dynamically deployable components utilizing local hardware capacity.
 
 
 
 
 Unfortunately, extant Cloud databases cannot be easily extended to federate databases running on Gateways. The reasons are fundamental and have to do with the fact that existing databases typically depend their operation on high-performance servers interconnected via high-bandwidth network links. 
 
 
 
 Devices across different tiers may differ substantially, communication between devices take place over the Internet with high network latencies, and IoT is underpinned by variable operational conditions with highly diversified application requirements. 
 
 
 
makes data federation in IoT a particularly challenging topic. 

There are multiple parameters . 



can help storage engineers to 



This paper examines the structural differences betweenvarious IoT protocols and enterprise protocols and identifies keytechnical challenges that need to be addressed to implementservice virtualization in IoT environments.




experiment with multiple parameters including 


create tiers with different parameters for devices, networks, and failure rates. 

various emulated devices, communicating over multiple networks with different 

different device resources, 



metrics, such as service time, bandwidth, dropped packets, resource consumption, and so on. 

emulate devices with various , emulate networks with various 

experiment with various 


With respect to the previous example, storage engineers can experiment with IOPS, 

examine various device and inter


approaches to distribution of computational and storage services across tiers,  with regard to processing, storage, and network capabilities, and federation of localized services that communicate over the Internet. 






applying a discipline of empirical exploration on large design spaces. 

application, utilization of a tier's offerings with respect to 

In this paper, we introduce IoT Testing as a Service- IoT-TaaS, a novel service-based approach for an automated IoT testing framework aims to resolve constraints regarding coordination, costs and scalability issues of traditional software testing in the context of standards-based development of IoT devices, and explore its design and implementation. 

Using \ac{IOTIER} storage engineers can 





 Having a real-world production environment as a reference, enables researchers to 
 
 For instance, they can validate approaches for 

 

 
 
 
 
Solutions stemming from the aforementioned challenges can be addressed in a piecemeal fashion, but any solution targeted at a single challenge may prove unsuitable for another. 
 
 
 
 
The control plane is the part of a network that carries signaling traffic and is responsible for routing. Control packets originate from or are destined for a router. 




To do that, containers include a set of agents to enforce network traffic rules on their local network interfaces, and to interact with other subsystems of \ac{IOTIER}. Figure~\ref{fig:network_profiles} shows a collection of performance profiles for various network protocols.





traffic control, log collection and forwarding, and inter

This, however, is not achievable at the level of the container.






%virtual runtime that can be regarded as easily—configured, lightweight VMs that start-up fast, often in under one second.


\ac{IOTIER} is composed of three autonomous subsystems: Hardware emulation, Network emulation, Event simulation.



%One of the places CPU shares breaks down is when you *don’t want* a container to be able to burst above its share when there is no contention on the host. There are several valid use cases such as:


Docker, however, does throttle network resources. To circumvent this limitation, we use Traffic Control (TC) agents running within the containers.  




The interplay of Docker and TC ground the foundations to create testbeds with hundreds of emulated IoT components, clustered in various network topologies. 





Additionally, since Orchestrators are agnostic to the services running within containers, TIMON provides REST endpoints for distributed service coordination.



If some containers don’t need all of their allotted resources, then it will be made proportionally available to other containers. 



A container with a period of  100,000-microsecond and a 50,000-microsecond quota would be throttled if it attempted to use more than half of the CPU time during its 0.1s periods. \todo[inline]{Explain that in Ghz terms}





Events related to intriguing system behaviors can be later integrated into various levels of testing in order to to 

The exact specification of how containers will transit from one phase to another depends on the Microflows defined in TIMON.







As shown in , there are at least two different Microflows to control the transition between phases: Disjoint and Evolutionary.

e.g, progressively joining clients, pseudo-random termination of server instances, or any other failure injection that may affect system's stability.

For example, we can go from a phase with 10 containers to a phase with 30 containers, either by killing the 10 clients and starting 30 new ones, or by adding 20 new ones.  



Docker-Compose is used to run multi-container environments over multiple physical nodes. If scalability is required, containers are spread across all the available nodes. If minimal interference is required, as happens in tiering scenarios, we use orchestrator's placement constraints to place a tier's containers into an exclusively allocated group of physical nodes (e.g, tagged by the tier's name)



%A Microflow is not a bunch of independent tasks, but rather a way of consistently changing and tracking its progress the state of the testbed. 

%TIMON can execute commands synchronously or asynchronously or schedule them for execution in the future and deals with all the threading and distributed complexity.



represent the 

the performance perceived by the application would be the same as if was running on a real IoT device. 



 is the same as if communication was taking place over real-world

IoT software into containers, and then 

CPU, Memory, IOPS, and network bandwidth of physical machines in a lab environment exceed by far the perf

Instead, we create virtual entities whose performance characteristics, in terms of CPU, Memory, IOPS, and storage capacity, 


Equally, we do not attempt to simulate  Running an interference model before sending a request over the network is not likely to yield any valuable insights for the application performance. 



Network emulation strikes the balance between using real machines on full-fledged networks and running software models of applications and networks in simulation environments. Advanced Linux features make it possible to emulate entire networks on a single machine, enabling experiments that are much easier to run and repeat. However, some of these features were not designed with the primary purpose of supporting emulation frameworks: if not carefully configured, they can lead to erroneous results. In this paper we note a few properties of Linux-based network emulation that researchers should consider while planning their experiments. 


This way, we make sure that a service performs as expected when interacting with other services over unreliable networks.



In a static, or single-phase experiment,

There are no changes at the level of the testbed. 

. This stasis can manifest in many ways in experimental research. For example, when researchers want to evaluate the effect of a different number of clients on a system, they have to repeat the experiment using a different number of clients. To answer more intriguing questions, such as "how long does it take for a system to recover to its previous 99th latency after N clients leave", there is the need for more dynamism. 

 
 batching autonomous tests 

in order to explore large design spaces without continuous intervention from the user.

, IOTier allows operators to 



in a way that was not previously possible. 

Situations invariably arise in which you have thousands of metrics at your disposal but none are quite what you need to understand what’s really happening. Either because metrics are not relevant, or their granularity isn't good enough. For instance, a common methodology to measure 99th percentile is to run numerous experiments with an increasing number of clients, and observe the system's performance in its run. The metrics are relevant, but they are so coarse-grained that are not realistic. It cannot diagnose (1) how many clients the system can accommodate before performance starts degrading (2) if degradation is gradual or cliff-like (3) the time it takes to recover to its previous after clients leave (4) the difference between short-lived and long-lived clients. 

And there are still other scenarios where you have all the metrics you need, but the signal-to-noise ratio is so high that the problem is virtually impossible to diagnose the problem. For example, waiting for a background task (e.g, rebalance) to occur will produce such a large log that it will be difficult to relate an observed behavior back to task. Or, a specific behavior that happens when the task runs, may be falsely attributed to another task started in the meantime (e.g, replication). 


\begin{figure*}[ht]
    \includegraphics[width=\linewidth]{images/phases.pdf}
    \caption{Phases overview}
    \label{fig:phases}
\end{figure*}




\ac{IOTIER} is implemented over Docker Engine, and its native Orchestrator Docker-Compose. With Docker-Compose, we can specify the testing environment, in terms of hardware, software, network, and placement policies, in one YAML file, and then create, update, or destroy the entire environment, in a single command. 

If TC was used at the host level, we would be able to perform throttling transparently to the containers, but it would require all host machines to have TC installed and to have access to those machines - which is not always possible.




To import applications \ac{IOTIER} provides automates pipelines in bash to create Docker images with all the necessary agents installed. TIMON is implemented is about 1,000 lines of Golang code. 






Note that for the above to work, TC and IFB modules must be loaded to the kernel of the host. 




Another reason for choosing the particular profiles is to demonstrate compatibility issues. At first glance, there is no common network interface between these two devices, and therefore they are not compatible.  The factor 2x2 denotes two MIMO antennas that establish up to two data streams within the receiving device, thus doubling the maximum supported bandwidth.










network namespace of container (REF: NAMESPACES). Each network namespace is a virtualized network stack with isolated network interfaces, IP addresses, routing tables, tunnels, firewalls.


When a container joins the network, Docker Engine creates a new virtual network interface device (NIC) under the container's namespace (REF: NAMESPACE) and a veth pair. The "veth pair" is basically a virtual network cable which have a virtual network interface device (NIC) on each end; packets transmitted on one end are immediately received by the other end.

new virtual network interface (veth) under the container's namespace (REF: NAMESPACE). 

(veth)


 By attaching one side of the veth pair to a bridge running on the host, and the other side to a container, we effectively enable the communication between all containers and the physical network of the host.
 
 The basic component of TC is the queueing discipline (qdisc). Lying between the IP protocol output and the network device, a qdisc contains two interfaces: one interface queues packets to be sent, and the other interface releases packets to the network device. 





emulat

that exactly mirrors 

another , intermediate solution. It consists of

, failure injection

 In such environments, 



a single configuration; it is usually not possible to modify the platform to test the system under different conditions (for example, different net-work conditions), leading to results that lack generalization.


Although platforms like IoT-LAB yield high-accurately insights, the high cost make it a prohibitive choice. Yet, existing testbeds provide few means 










The Internet-of-Things (IoT) is an emerging field that connects a diverse set of geographically spaced devices exchanging data with other devices and systems over the Internet. In its simplistic view, an IoT architecture consists of at least three tiers: Tier 1: Things, Tier 2: Edge Gateways, and Tier 3: Clouds. 

Traditionally, Gateways were used as a communication-intensive frontend responsible for the propagation of query requests and results to and from Things, and Cloud was used as a storage-intensive backend responsible for the mass storage and in-depth analysis of IoT data. The The in-Gateway functions can be: (1) collection and preliminary processing (2) localized querying in response to real-time events, or (3) local storage of files that are very large or need very low latency access or their value degrades with time and there is no need to propagate this data further up to the Cloud. 



In an IoT solution, the back-end service provides functionality such as:

    Receiving telemetry at scale from your devices, and determining how to process and store that data.
    Analyzing the telemetry to provide insights, either in real time or after the fact.
    Sending commands from the cloud to a specific device.
    Provisioning devices and controlling which devices can connect to your infrastructure.
    Controlling the state of your devices and monitoring their activities.
    Managing the firmware installed on your devices.





facilitate complex topologies with IoT specific workloads. 

IoT service run in containers in order to .

IoT service developers can   of  containerized  IoT  services [22]. 



IoT provided a way to address the scarcity of resources available on hardware devices, augmenting them with the capabilities of cloud environments

The proposed testbed is meant for testing high-level application protocols and interaction with cloud services rather than analyzing low-level nuances of, e.g., medium access control in wireless communications. 

We therefore ground our approach in simulating real-world environments, devices, and sensors [7]

We therefore ground our approach in simulating real-world environments, devices, and sensors [7] which, on the one hand, does not require custom hardware for application development, while on the other hand permits integration with existing IoT hardware devices depending on the maturity of the tested IoT system. 




However, such tools are mostly i

Examples of such emulators are MicroGrid [2], Modelnet [3], Emulab [4],EMPOWER [5], IMUNES [6], V-em [7] and eWAN [8].

However, those approaches are generally quite complex, and their deployment outside of the laboratory which developed them is often very limited, because they involve a non-trivial setup phase. 



Emulated networks enable educators, researchers, and operators to conduct realistic network scenarios on commodity hardwar



Virtual testbed 




is a well-adopted technology 

The main domain of our work presented in this paper is IoT testing, a topic already well researched and described in multiple publications


Virtual testbed is a well-adopted technology 


Batch  processing  systems  like  MapReduce  [13,  22,24] are well suited for efficiently transforming or analyz-ing an entire corpus: these systems can simultaneouslyuse a large number of machines to process huge amountsof  data  quickly.  Despite  this  scalability,  re-running  aMapReduce pipeline on each small batch of updates re-sults  in  unacceptable  latency  and  wasted  work

The main domain of our work presented in this paper is IoT testing, a topic already well researched and described in multiple publications, several of which we discuss in Section 2.3. However, our proposed methodology involves adoption of the software-defined concept in this domain in order to provide a novel solution answering common IoT testing issues which stem from integration with cloud services. To the best of our knowledge, a similar concept has not previously been described; therefore, we divide related work into three parts corresponding to the areas mentioned. In Section 2.1 we describe the role of Mobile Cloud Computing in the context of IoT, in Section 2.2 we try to place our work in the context of other software-defined IoT solutions, and in Section 2.3 we describe other IoT testing approaches.


\ac{IOTIER} 

Virtualization is a technology than span 



Most  distributed  storage  systems,  such  as  Ceph  [15]  orHDFS [16] include tools to balance the amount of data hostedby each node. Some works such as that of Liao et al. [17] placethe data uniformly from the beginning to avoid rebalancing




In order to ensure flexibility of virtual testbed components creation, we introduce software-defined management of the testbed itself. The process of connecting virtual sensors to virtual devices, i.e., virtual wiring, and the creation of a virtual environment, along with a scenario which expresses its behavior, is defined by the software.

To replicate normal and abnormal operating conditions, 

For example, engineers 

Apart from Mininet there exist other tools to simulateor  emulate  computer  networks.  Simulators  try  to  mimicthe  behavior  of  a  system  model  in  a  more  abstract  waywhereas with emulators the same code can be executed asin  the  real  system.  A  disadvantage  of  emulators  may  bethat they run slower than the actual hardware and thereforeare  not  always  able  to  reproduce  a  realistic  timing.  Insimulators the execution is more flexible and can even befaster then in the real system [11]. On the side of the sim-ulation tools, there is ns-3, an open source discrete-eventsimulator that was mainly created to support education andresearch [12]. Others are fs-sdn [13], which as Mininet istargeted at SDN prototyping and the commercial EstiNetX  Simulator  [14].  An  example  for  network  emulationis  Mahimahi,  a  record-and-replay  tool  that  can  be  usedfor recording traffic from HTTP-based applications. LaterMahimahi  can  replay  the  traffic  emulating  the  networkstructure that produced it. Linux network spaces are usedhere as well [15].Although  hundreds  of  nodes  can  be  emulated  on  asingle machine with Mininet at some point the resourcescome  to  an  end  where  it  is  not  possible  to  make  thenetwork  larger.  To  handle  this  problem  Blankstein  et  al.developed  a  distributed  version  of  Mininet  where  thetopology  of  a  virtual  network  is  split  between  multiplecomputers automatically [16]. This approach has now alsobeen  followed  by  the  Mininet  community  and  there  is  acluster edition prototype available in the repositiory.




In this paper we propose a testbed aimed at end-to-end testing of IoT systems from the application point of view. 

  Challenges stemming from the aforementioned characteristics can be addressed in a piecemeal fashion [4], but any solution targeted at a single subsystem may prove inadequate for other subsystems. The problem of design and implementation of IoT systems is therefore challenging, but may be ameliorated by suitable development tools, such as sensor network simulators [5, 6].
  
  
  
  
But platforms like IoT-LAB provide few means of evaluating the system under different conditions (device characteristics, variety of networks and topologies), thus leading to results that lack generalization.







The experimental results show that the proposed mechanism can effectively limit the actual container bandwidth within 2% fluctuation range in the container exclusive bandwidth scenario, and can precisely limit the network bandwidth of the container with average 0.5% error range in the shared idle bandwidth scenario. Meanwhile, the mechanism can flexibly manage resources based on priorities. With the advantage of providing a more native interface for Docker and requiring no additional tools, this mechanism can provide a convenient and effective solution for fine-grained elastic network resource






In particular, we devise a series of experiments to answer the following questions:


\subsection{Baseline}


\begin{itemize}
    \item Defining a measurable steady state that represents normal circumstances to use as a baseline.
    \item Developing a hypothesis that this state will continue in both control and challenge groups.
    \item Introducing realistic network stressors into a challenge group, 
    \item Attempting to invalidate the hypothesis by noting differences in behavior between control and challenge groups after chaos is introduced.
\end{itemize}









we use the platform to evaluate a key/value database in ways that had not been possible before. 


strategies for a rescaling operation and try tominimize various subsets of the objectives.



 





    establish baselines for the following experiments. From the outcome of distill the corner cases and we use them as basis to configure the next experiments. 
    
    
    In contrast to the first experiment, there is no intuition here about the performance recovery since databases are stateful and 
    
    
    With C for client and S for server, the phases are: 


\item is it CPU, Memory, IOPS, or Network that accelerate saturation on a server, and at which rate
    \item how long does it 
    
    (1) identify how ; (2) identify if, and after how long, the database performance recover after bursty traffic is over.

The approach is same as before, with the exception that the server runs a key/value database and the client a YCSB benchmark. The goals for that experiment are     
    
    
There are two main differences compared to previous examples. Firstly, is that now we use replication. 

 For the implementation we use Grid topologies. 

Although the previous experiments were stressing client-to-server communication, this experiment stresses server-to-server communication. In particular, we use Tier topology to decide whether 

difference is that now we use replication

In this experiment we emulate the impact of networking to replication strategies. In the context of IoT, that would mean the impact of making replicas across gateway or across cloud servers. 
    
    

    


The experiment consists of 4 phases, with phase tick every 180 seconds, and Evolutionary Microflow handling the phase transition. With C denoting the client and S the server, the phases are: (1C,1S) $\rightarrow$ (1C,2S) $\rightarrow$ (1C,3S) $\rightarrow$ (1C,4S).

    
    here since new entries are likely to increasing 
    
    a database is a stateful process 
    
    This is a much harder question to answer
    
    a throttled database responds to an increasing load, and how long it takes for the tail-latency on the
    
    then see how long it takes for the database to recover to its previous.
    
    it takes for the database to recover after a saturation point has been reached 
    
    limitations are more likely to saturate the system (2) 
    
    Same as before, the goal is to see how a throttled database r The 
    
    The goal here is to 
    
    
    
    
    
    
    
\item is the size of the namespace related to network characteristics ?
    \item can a slow server influence the overall database performance  ?
        \item how is resharding frequency related to network characteristics ?     
    
    


In this IoT scenario we emulate bursty traffic on a cell tower that serves transient IoT devices (e.g, moving cars). The experiment is multi-phased (dynamic) and consists of 1 server and up to 32 clients that appear gradually and disappear after a few minutes.  In total, the experiment goes through 5 phases in the following order: (1C,1S) $\rightarrow$ (8C,1S) $\rightarrow$ (16C,1S) $\rightarrow$ (32C,1S) $\rightarrow$ (1C,1S). For the implementation, we use a Cluster topology with servers running a key/value database instance and clients running YCSB benchmark. For the evaluation, we use this configuration and perform tests with different network profiles.





\subsection{Goals}
We evaluate \ac{IOTIER} using synthetic and production workloads on key/value databases. 



 
    
    The goals for that experiment are (1) to determine if its better to have more to have less servers when the network is fast, or slow (2) to identify the rate at which a slow server can affect the whole system. 
    
        Some of the question we want to answer include "when there is a fast network, is it better to have more or less servers 
    
    
    
    virtual devices (CPU, Memory, IOPS) and virtual networks (Bandwidth, latency) works are expeceted. To do so we use standard benchmarks. Stress-ng for the devices and iperf for the networks.
    
    In the second experiment, we repeat the setup of the first experiment, with the difference that 

We use scheduled events to dynamically add or remove clients and servers. When a scheduled event is fired, it marks the transition from one phase to another. The transition is handled by an Evolutionary Microflow.


thus system developers have little information to assess the baselines their systems present.



that exactly mirrors a selected production environment, from a hardware, software, and operations perspective.






\subsubsection{Metrics}
Although mean and median latency can reveal baseline performance characteristics, systems often exhibit artifacts such as garbage collection, negotiation overheads, and other "hiccups" that average values tend to hide. Without tail latency granularity, engineers lack the insights to understand what is actually happening. Plotting latency by percentile distribution is an excellent way to see  what the performance behavior actually looks like because latency is not going to be uniform.





 **But what this single most representative value has done is, it has hidden the outliers** (outlier is a data point that differs significantly from other observations), which may seem insignificant in this small dataset.



By identifying the 


take mitigating actions upon 

A virtual testbed for 

  In this view, Virtual Testbeds will play an important role in 

evaluation of database systems, 

algorithms, applications, and policies before actual development of cloud products.

The interplay of containers and agents ground the foundations for building arbitrarily complex distributed testbeds. 

under different conditions (for example, different net-work conditions), leading to results that lack generalization.



It must be clarified that although IOTier provides the mechanism for data collection, monitoring, and correlation between system model and observed performance, it does not provide root cause diagnosis of performance problems. It merely points developers to where they should look. 





Notably, \ac{IOTIER} takes a cloud-native approach to create, manage and monitor experiments. It does not require any host-level knowledge or access. As such, it may be adopted for use over Docker-As-A-Service or Kubernetes-As-A-Service platforms.


tool will be able to detect architectural issues automatically and recommend changes according to policies published in the \textit{hub}. 


Although not strictly scientific, this contribution is something that is greatly missing in the literature.





Scale out your IoT solution by packaging your business logic into standard containers, then you can deploy those containers to any of your devices and monitor it all from the cloud.




By systematically mastering (or editing) events in a definition file, and confining their ramification into framed phases, we facilitate root-cause analysis since any observed phenomena within a phase can be explicitly attributed to a triggering event. 






Configuring models to run in real time enables you to use hardware-in-the-loop simulation to test controllers. You can make design changes earlier in the development process, reducing costs and shortening the design cycle. 


As we do, both simulators are based on discrete-events that 


Modeling concerns may range from the instruction set of specific hardware architecture (e.g, ARM, x86), to environmental factors such as distance between the sender and the receiver, electromagnetic interference, multipath effects, and so on.



distribute computation and storage tasks across the tiers optimally
devices, improving responsiveness in Edge computing paradigms.


In particular, we evaluate their impact in contention, namespace partitioning, tiered load-balancing, and replication strategies. 

demonstration of platform capabilities to estimate how a key/value database designed data centers would behave if deployed over a tiered IoT environment. 




%In Sections~\ref{sec:evaluation} we use the platform to evaluate a key/value database in ways that had not been possible before. 

We also explicate particular properties that improve the fidelity of emulation results

By harnessing the power of distributed edge resources, 
In that view, it is difficult to design competitive solutions without first understanding a tier's trade-offs at both the coarse-grained service level and fine-grained device level. 



We use limit for the emulation of IoT devices. This thin provision enables us to create scalable testbeds with numerous containers. 






Like CPU, throttling I/O require more advanced techniques than simple resource allocation. The reasons are fundamental and have to do with the sampling period of quantized allocation units, and the fact that utilization metrics are governed by workloads that may be bursty.

However, hard limits are not always feasible to achieve.  such as CPU, IOPS, and Network, are challenging. . Whenever hard limits are not feasible we use soft limits. A soft limit is a value that is used more as a baseline and does not strictly guarantee that the container will not exceed the limit. 

Throttling real-time resources like the CPU, block I/O, and Network, 




tries to continually , by 


x
internal simulation engine 

The FSM can change from one state to another in response to some inputs; the change from one state to another is called a transition.

controller 
finite state machines (FSM)


into Timon internal simulation engine. When an event is fired, Timon's controller 

 to 

that can 



Through this tool, operators can express 
The given scenarios are interpreted by Timon's controller




are expresses as sequences of events that change the internal simulation engine from one state to another. 

which change the internal 

are then . 

write testing scenarios that express 

 as a series of events that change the state of the testbed from one state to another. Whenever an event is fired, Timon alters the structure of the testbed dynamically 
 
 


alters the structure of the testbed to reflect that change. 









 \begin{listing}[htbp]
  \begin{minted}[linenos=false,escapeinside=||]{yaml}
# Resource specification
&link-80211n:
labels: 
- com.timon.tc=rate 150mbit delay 50ms

networks:
 dev_gw:
 <<: *link-80211n
 ipam.config.subnet: 172.16.238.0/24

&storage-SSD_M2:
labels:
- com.timon.io.read_bps_device=259:0 2gbps

 
# Specify Device
&Dell_Edge_5100:
<<: *Storage_SSD_M2
networks: [dev_gw, gw_gw, gw_cloud, ...]
resources.limits: [cpu:1, memory:8G]


# Test with gradually joining clients
Services: 
 store-gateway:
 <<: *tikv-store
 <<: *Dell_Edge_5100
    
...
clients-phase-two:
<<: *ycsb
<<: *Microsoft_Hololens_v2
Env: [PREV=.., CUR=.., TOTAL=540,TICK=180]
 
\end{minted}
\caption{Example of an IOTier full-stack experiment. The anchor '\&' defines a chunk of configuration, and the alias '*' is used to refer to that chunk elsewhere. Labels in the "com.timon.*" namespace are used as a medium to pass parameters to Timon. ENV is abusively used to implement native YAML functions, in order to define phases and dependencies between them.}
\label{lst:yaml}
\end{listing}





Now bear in mind, a crashed pod is just one example of fault injection that Chaos Mesh is capable of. There are six chaos types: PodChaos, NetworkChaos, TimeChaos, StressChaos, IOChaos, and KernelChaos. Concerning networking errors, in particular, you have a lot more options than the other chaos types. There’s network-delay, network-corrupt, network-loss, network-duplication, and network-partition, all of which affect the network as their names suggest. For filesystem chaos, you have just two, I/O delay and I/O error that simulate file system I/O delays and errors, respectively.


Other major chaos experiments include container-kill, an important one because it lets you kill a specific container in a pod, CPU-burn that stresses the CPU of a selected pod, and Memory-burn that stresses its memory. TimeChaos is also an important one, especially in a distributed environment where it’s critical to maintain a synchronized clock across all nodes to remain compliant and maintain security. TimeChaos introduces a fault called “clock skew” that basically introduces a time difference between the clocks on different nodes to see how your systems respond.





\subsubsection{Consistency models}
\begin{itemize}
    \item Global ordering
    \item Eventual consistency
\end{itemize}





Traditionally, transactional and analytical data are managed in separate systems. To derive business insights to support important business decisions, enterprises have to use extract, transform, load (ETL) tools and processes to migrate data from an online transaction processing (OLTP) database to an online analytical processing (OLAP) database. This approach involves complex software, and leads to issues like stale or inconsistent data. Any insights gained from this stale data are of limited value











 Therefore, the testbed should be able to accommodate hundreds of parallel workload generators, and control their execution through distributed synchronization;
 
 
 
 
 
Kube-monkey: breaks the Kubernetes itself. It randomly deletes Kubernetes (k8s) pods in the cluster encouraging and validating the development of failure-resilient services.


Number of clients (without degraded tail-lantecy)
\item Per client tail-latency to number of nodes
number of nodes


Cloud systems must provide high levels of availability. In particular, they are often multi-tenant systems, which means that an outage affects many different applications. Moreover, the use of commodity hardware means that failures are relatively common, and automated recovery must be a first-class operation of the system. 


Blockade features:

    A flexible YAML format to describe the containers in your application
    Support for dependencies between containers, using named links
    A CLI tool for managing and querying the status of your blockade
    When run as a daemon, a simple REST API can be used to configure your blockade
    Creation of arbitrary partitions between containers
    Giving a container a flaky network connection to others (drop packets)
    Giving a container a slow network connection to others (latency)
    While under partition or network failure control, containers can freely communicate with the host system – so you can still grab logs and monitor the application.



    
    To build an HTAP database system like TiDB, we had to conquer several engineering problems. Building an HTAP system is a tough task due to the following reasons:

    OLTP and OLAP systems have different design philosophies:
        In OLTP scenarios, we focus on transaction correctness. Their performance metrics are queries per second (QPS) and latency. OLTP systems often deal with point writes or point selects.
        In OLAP scenarios, we're more concerned with the query throughput, the processing capability, and the costs for large batches of data. In many cases, to do an analytics query, the system must scan millions of rows of data, and join more than 10 tables.

    OLTP systems usually use row-oriented storage (or row stores), like InnoDB and RocksDB, while OLAP systems usually use column-oriented storage (or column stores). To implement these two in the same system, it's difficult for the architect to make tradeoffs between row stores and column stores.

    OLAP queries are resource-consuming. If they are not isolated well from OLTP queries, OLTP performance will be affected.
    
    
    
 We’ll talk more in depth about these topics in later series, for now I think it’s worth mentioning before we dive into refactoring that it’s first on this list for a good reason.







 Designed to be extensible, the protocol offers a multitude of applications beyond traditional IM in the broader realm of message-oriented middleware, including signalling for VoIP, video, file transfer, gaming and other uses. 





way it operates under the presence of failures, either partial or total. 
The need to characterize cost and availability and operating is nothing new. 


and quantify self-healing properties 

Without , such as  it is difficult to estimate the overall cost of running a system.  The second impact is that it cannot . \comment{More ?}







a variety of operating conditions and business scenarios. \comment{examples: minimum operating cost, maximum availability, maximum clients, minimum blast radius}



Without redundancy and automation in place, these disappearing servers could cause service problems. 
 

The problem is 

Generated workload can be 



YCSB has been the undisputed winner for the comparing databases in an  apples-to-apples manner. YCSB is effectively a nice abstraction for hammering  By calculating the difference between request submission and acknowledgment, YCSB can yield performance statistics such as .








This allows users to have a centralized subsystem that can collect, analyze and store logs from across the Kubernetes cluster and all applications running in it. 


that provides extensive information about the operating environment of a running container, and several metrics for CPU utilization, IOPS, or network traffic. 

At the same time, emerging databases are natively integrated with Prometeheus monitoring tool. 








Kubernetes continuously collects information about the cluster state, and upon deviations from the desired state trigger an automatic action to ensure that system operates within its desired configuration

that you then get to find out what happens when the app’s connection to the storage is interrupted. Since you have control over all of the infrastructure just by changing Kubernetes, you can use tools like Litmus, which work within Kubernetes, to simulate an outage.





Also, some of the more database-specific administrative tasks—backups, scaling, tuning, etc.—are different due to the added abstractions that come with containerization.

Since pods are mortal, the likelihood of failover events is higher than a traditionally hosted or fully managed database. It will be easier to run a database on Kubernetes if it includes concepts like sharding, failover elections and replication built into its DNA (for example, ElasticSearch, Cassandra, or MongoDB). Some open source projects provide custom resources and operators to help with managing the database..


Databases that are storing more transient and caching layers are better fits for Kubernetes. Data layers of that type typically have more resilience built into the applications, making for a better overall experience.  


They may include additional features like sharding, leader election, and failover functionality needed to successfully deploy MySQL or PostgreSQL in Kubernetes.






 
  Outages happen. What’s important is how your application responds to the outage. Does it come back up on its own? After how long? With Litmus, you know exactly when you’ve injected the chaos, and you can observe the results in a controlled environment. 
 
 


actual situations met in specific 
To compare available solutions, we need tools 




and goes beyond measuring the rate of simple workloads. \comment{Availability ? Reliability ? cost-efficiency ?}



Notably, systems observability was an emerging field at that time, exposing only coarse-grain information \comment{such as ?}.







that cover interesting parts of the performance space 


Thus it eliminates under-provisioning bottlenecks, and over-provisioning costs. 

it provides capabilities for monitoring, alerting, 


 for


Such vertical scaling of existing systems also enables them to use virtualization technology more effectively, as it provides more resources for the hosted set of the operating system and application modules to share.

 At this point, when the interactions between components are unpredictable, the system becomes chaotic. 



that provides a realistic view of 

Finding out how components intermix and work together is often a process of seeing what problems arise when a service fails in production.

Assessing the performance of a database and the environment where it runs 


Janus particles, named after the double-faced Roman god, are compartmentalized colloids
with two sides of different chemistry or polarity. 














Before we can put a distributed system like TiDB into production, we have to ensure that it is robust enough for day-to-day use. For this reason, several years ago we introduced Chaos Engineering into our testing framework. In our testing framework, we:

    Observe the normal metrics and develop our testing hypothesis.
    Inject a list of failures into TiDB.
    Run various test cases to verify TiDB in fault scenarios.
    Monitor and collect test results for analysis and diagnosis.


a full chaos engineering application consists of hypothesizing around defined steady states, running experiments in production, validating the system via test cases, and automating the testing.







%LitmusChaos  is a toolset to do cloud-native chaos engineering. Litmus provides tools to orchestrate chaos on Kubernetes to help SREs find weaknesses in their deployments. SREs use Litmus to run chaos experiments initially in the staging environment and eventually in production to find bugs, vulnerabilities. Fixing the weaknesses leads to increased resilience of the system


they created an automated process called a Chaos Monkey aimed at  and services using. Over the years Netflix developed a series of additional agents in their chaos tooling family, known as The Simian Army, to inject more complex types of failures and induce abnormal system conditions


To accomplish this, 






Chaos Testing is about running a test in production
Scrutiny is about re-creating the condition for this test to run on another system
Like benchmarks, that goes beyond measuring simple workloads

The process for fixing issues identified through this process was the following,

    Discover the issue, identify the impacts if any and determine the root cause.
    Mitigate the issue to prevent data loss or service impact in any customer facing environments
    Reproduce the error through automation
    Fix the error and verify through the previous step it will not reoccur

The Kubernetes ecosystem contains dozens of components dedicated to testing your Kubernetes cluster. Tests are usually run in a dedicated environment so they don’t break production deployments. 

However, one of these components does just the opposite: it runs on the production environment and breaks things on purpose.



Chaos engineering (sometimes also called chaos testing) involves artificially injecting failure into our live, production systems, as a way to proactively validate that those systems handle a degraded environment.


an API call which responds at a rate of 1 byte a second will usually cause much more mayhem than an API call which doesn’t respond at all.


Based on the above requirements, we need an automatic workflow that:
\begin{itemize}
    \item \textbf{Injects chaos}: Fault injection is the core chaos testing. In a distributed database, faults can happen anytime, anywhere—from node crashes, network partitions, and file system failures, to kernel panics. 
    \item \textbf{Verifies the impact of that chaos}: To validate how TiDB withstands chaos, we implemented dozens of test cases in TiPocket, combined with a variety of inspection tools. To give you an overview of how TiPocket verifies TiDB in the event of failures, consider the following test cases. 
    \item \textbf{Automates the chaos pipeline}: To make \ac{Scrutiny} more dedicated to the testing part of our workflow, we chose the open-source tools approach. This, plus our all-in-K8s design, lead us directly to Argo.
\end{itemize}


    
    
    
    Visualizes the results
    
    
    
    
Netflix Chaos for Production -> Chaos Mesh for Kubernetes -> TiDB over Chaos Mesh + Argo for database failrues


Some people thought this was crazy, but we couldn’t depend on the infrequent occurrence to impact behavior. Knowing that this would happen on a frequent basis created strong alignment among our engineers to build in the redundancy and automation to survive this type of incident without any impact to the millions of Netflix members around the world. 


Automation

Any change to the production environment changes the resilience of the system. At Netflix, our production environment might see many hundreds of deploys every day. As a result, our confidence in an experimental result quickly diminishes with time.

In order to have experiments run unsupervised, we had to make them safe. We designed a circuit breaker for the experiment that would automatically end the experiment if we exceeded a predefined error budget. An automated, ongoing analysis hooks into the same system we use to do canary analysis.

Before ChAP, a vulnerability could be identified and fixed, but then regress and cause an incident.



Litmus


Chaos testing helps you find out how your application responds to infrastructure events. This isn’t that big a deal for a monolithic app where all the state is probably on one server. If your app is a suite of microservices that are all spread out across a bunch of servers, and if those microservices need to use the network to talk to other related services, then you’ll want to make sure the app comes back after a network interruption, right?

 
 
 The ability to execute experiments that represent real life events in a controlled manner in production systems seems scary at a first glance but it can certainly increase the quality not only of the business applications but of the infrastructure systems as well.
 
 When you use code to control network infrastructure, you need tools to evaluate the potential impact of a change before you apply it in production, because even a simple error can cause an outage. But when you operate a hyper-scale cloud platform, the expression “test network” has a meaning of its own. You just can’t replicate your entire network for testing. The next best option, Microsoft figured, is simulating the network, which is what it’s done with CrystalNet, a virtual copy of the entire Azure network infrastructure, named after the crystal ball a fortune teller might use.
 
 CrystalNet is an accurate copy of the network with the same interfaces and workflow because it runs real device firmware in Docker containers and virtual machines. “Each device's network namespace has the same Ethernet interfaces as in the real hardware; the interfaces are connected to remote ends via virtual links, which transfer Ethernet packets just like real physical links; and the topology of the overlay network is identical with the real network it emulates.” It loads real configurations into emulated devices and injects real routing states into the emulated network, while management tools run in VMs and connect to devices the same way they do in the production network.
 
 
 CrystalNet isn't the only tool Azure network engineers use. It won’t find memory leaks or timing bugs, and while what-if analysis and verification tools like Batfish and MineSweeper don’t reflect the live network as precisely, they are more efficient at answering questions like, “Is there a scenario where one or more links fail and send excessive traffic through this particular switch?”

Formal verification tools aren’t as useful as you might expect, because they assume that devices work correctly. “In reality, device behavior is far from ideal.” But they’re a good thing to run first as a low-fidelity check, because they don’t need as many resources as CrystalNet.

A Chaos Proxy is a service that your microservices can connect to.

It routes traffic to real destination microservices and returns responses back to the microservices through the proxy — but does so in a very unreliable way.

Through the proxy, requests are randomly delayed and/or randomly fail in unexpected ways — all for the sole purpose of helping you understand how the microservice responds to these various failure conditions.





On the other hand,  Cloudproviders  want  to  provide  the  best-matching  hardware  configurations  for  different  use-cases. 

Despite the common belief that hardware unreliability shapes the software fault tolerance design, years of improvement in 
machines

 This technology builds a data analysis platform with many relatively inexpensive x86 machines, and uses parallel capabilities to solve computing problems of big data sets.







, and the diversity of infrastructures to support these applications.  

Although benchmarks provide rich capabilities for measuring the rate of simple workloads, they cannot simulate arbitrary topologies of inject failures. On the other hand, 

impact of hardware, network, data storage and data management systems, to the application-perceived performance. 




Therefore, CloudSim a popular  event-based  framework by Calheiros et al.,  was developed  to model  and simulate theusage of IaaS (Infrastructure-as-a-Service) Clouds.  




  simple performance evaluation becomes irrelevant. Resiliency, Burst 


are only effective on comparing one setup over another. 




the demand for ergonomic tools that can replicate production environments increases as well. 


not to mention the challenge of automating the pipeline to make the testing scalable and efficient.




new workloads, in addition to making it easy to benchmark new systems.

exploring databases under dynamically changing conditions. 








The number of emerging cloud serving systems and the wide range of proposed applications, coupled with a lack of apples-to-apples performance comparisons, makes it difficult to understand the tradeoffs between systems and the workloads for which they are suited.  

real-world situations and automate the exploration of large design spaces.


Replicating a production IoT  means developing and executing 


create arbitrarily complex topologies, and configure the desired network impairments in software (e.g, bandwidth constraints, packet delays, transmission windows)

lack automation for altering the setup at runtime, as it happens in real-world deployments. 

performance alone cannot help build confidence in the system's capability to withstand unexpected conditions.





 

for experiment 


 Further, they are being ap-plied to a diverse range of applications that differ consider-ably from traditional (e.g., TPC-C like) serving workloads.




One one hand simulators provide the means for evaluation of 

Simulators, however, only evaluate mathematical models rather than actual systems. One the other hand, Chaos testing suites can inject failures on production systems to 
They cannot however represent the problem domain for the future systems leading to a gap between system design and problem domain.


Metrics like usage costs, resource utilization and energy consumption can be also investigated using CloudSim.  

 We have multiple fault scenarios, against which dozens of test cases run in the Kubernetes testing cluster. Even with Chaos Mesh helping to inject failures, the remaining work can still be demanding—not to mention the challenge of automating the pipeline to make the testing scalable and efficient.




They lack, however, automation pipelines for exploring large design spaces. 


to evaluate algorithms, systems, and policies before the actual deployment.

test their services in repeatable and controllable environment free of cost, and to tune the performance bottlenecks 

for timely, repeatable, and controllable methodologies for evaluation of algorithms, systems, and policies before the actual deployment.






have event logs for  that we can correlate  to find out how the system behaves in that particular infrastructure event.

Additionally, with the contemporary monitoring tools,  was an arduous task. 




The demand of usable, ergonomic, Graphic User Interfaces (GUI) from end users is growing rapidly today. On one hand, User Interface Management Systems (UIMS) are used to construct the user interface components. On the other hand, there is a need for 








As a proof-of-concept, we use our to estimate how a key/value database designed data centers would behave if deployed over a tiered IoT environment. In particular, we experiment with constrained CPU cycles, Memory allocation, block device IOPS, and Network protocols, and analyze their effects on common and uncommon path operation of the key/value database. 



\ac{IOTIER} provides the building blocks to emulate the various IoT tiers into software stacks with configurable device capabilities (e.g, CPU, Memory, IOPS), network capabilities (e.g, banwidth, delay), and operating condition (e.g, disk failure rates, network outage). 

 delivering reliable, secure, fault-tolerant, sustainable, and scalable computational services, which are presented as Software, Infrastructure, or Platform as services (SaaS, IaaS, PaaS). Moreover, these services may be offered in private data centers (private clouds), may be commercially offered for clients (public clouds), or yet it is possible that both public and private clouds are combined in hybrid clouds. 




Each MongoDB cluster can output its logs into this pipeline making it available for your favorite log aggregators. You can also push events into MongoDB Ops Manager for viewing, alerting and making performance tuning recommendations.


The cloud computing paradigm is continually evolv-ing, and with it,  

 
 
 For event-based, we have created a new that can dynamically alter the structure of the testbed based on given scenarios. 
 
 
 Traditionally we use unit tests and integration tests that guarantee a system is production-ready. 



At PingCAP, we faced the same issues with our product, TiDB, an open-source, distributed NewSQL database. Fault tolerance and resilience are top priorities because the most important asset for any database user — the data itself — is at stake. 

they provide no insights on how a database will perform in a different environment. A slight change can make the results irrelevant. Yet, 



Further, they are being applied to a diverse range of applications that differ consider-ably from traditional (e.g., TPC-C like) serving workloads.The number of emerging cloud serving systems and the widerange of proposed applications, coupled with a lack of apples-to-apples performance comparisons, makes it difficult to un-derstand the tradeoffs between systems and the workloadsfor which they are suited.

Many of these“cloud” systems are also referred to as “key-value stores” or“NoSQL systems,” but regardless of the moniker, they sharethe goals of massive scaling “on demand” (elasticity) andsimplified application development and deployment

The large variety has made it difficult for developers tochoose the appropriate system.  The most obvious differ-ences are between the various data models, such as thecolumn-group oriented BigTable model used in Cassandraand HBase versus the simple hashtable model of Voldemortor the document model of CouchDB. However, the datamodels can be documented and compared qualitatively. Com-paring the performance of various systems is a harder prob-lem. Some systems have made the decision to optimize forwrites by using on-disk structures that can be maintained us-ing sequential I/O (as in the case of Cassandra and HBase),while others have optimized for random reads by using amore traditional buffer-pool architecture (as in the case ofPNUTS). Furthermore, decisions about data partitioningand placement, replication, transactional consistency, andso on all have an impact on performance






The same trend is reflected on Cloud providers, where uptime and durability are apparently deemed of greater importance than performance in some Service Level Agreements (SLA). 

Splitkernel disseminatestraditional OS functionalities into loosely-coupledmon-itors,  each  of  which  runs  on  and  manages  a  hardwarecomponent.   A  splitkernel also  performs  resource allo-cation and failure handling of a distributed set of hard-ware components.

Notably, similar claims were stated in earlier studies, but the technological barrier of that time forfeited the implementation of relevant benchmark. 





The main motivation for developing new cloud serving systems is the difficulty in providing all of these features (es-pecially scale-out and elasticity) using traditional database systems. As a tradeoff, cloud systems typically sacrifice th ecomplex query capabilities and strong, sophisticated trans-action models found in traditional systems.  Without theneed for complex planning and processing of joins and aggre-gates, scale-out and elasticity become significantly easier toachieve. Similarly, scale-out (especially to multiple datacen-ters) is easier to achieve without strong transaction protocolslike two-phase commit or Paxo



Blockade is a utility for testing network failures and partitions in distributed applications. Blockade uses Docker containers to run application processes and manages the network from the host system to create various failure scenarios.





At least two difficulties arise when benchmarking avail-ability. First, injecting faults is not straightforward. Whileit is easy to ssh to a server and kill the database process,it is more difficult to cause a network fault for example.



In this paper, we study data center network reliability by ana-lyzing network error logs collected for over a year from thousandsof network devices across tens ofgeographically distributed datacenters.Our goals for this analysis are two-fold. First, we seek to characterize network failure patterns in data centers and under-stand overall reliability of thenetwork. Second, we want to leverage lessons learned from this study to guide the design of future datacenter networks.Motivated by issues encountered by network operators, westudy network reliability along three dimensions:



All links in our data centers use Ethernet as the link layerprotocol and physical connections are a mix of copper and fibercables. The servers are partitioned into virtual LANs (VLANs) tolimit overheads (e.g., ARP broadcasts, packet flooding) and to iso-late different applications hosted in the network. At each layer ofthe data center network topology, with the exception of a subset ofToRs,1:1 redundancyis built into the network topology to miti-gate failures



 





intensive inter-node communication, or lack of elasticity.

qualities on the server side. Properties like , 


no single individual can reasonably understand the tradeoffs between systems. 



With the increasing number of emerging cloud serving systems and the widerange of proposed applications, 

As the number of emerging cloud service systems increasing

, coupled with a lack of apples-to-apples performance comparisons,  and the workloads for which they are suited


When you configure a zonal or regional persistent disk, you must select one of the following disk types:

    Standard persistent disks (pd-standard) are suited for large data processing workloads that primarily use sequential I/Os.
    Balanced persistent disks (pd-balanced) are an alternative to SSD persistent disks that balance performance and cost. With the same maximum IOPS as SSD persistent disks and lower IOPS per GB, balanced PD offers performance levels suitable for most general purpose applications at a price point between that of standard and SSD persistent disks.
    SSD persistent disks (pd-ssd) are suited for enterprise applications and high-performance database needs that require lower latency and more IOPS than standard persistent disks provide. SSD persistent disks are designed for single-digit millisecond latencies; the observed latency is app specific.






Land models, which have been developed by the modeling community in the past two decades to predict future states of ecosystems and climate, have to be critically evaluated for their performance skills of simulating ecosystem responses and feedback to climate change. Benchmarking is an emerging procedure to measure and evaluate performance of models against a set of defined standards. This paper proposes a benchmarking framework for evaluation of land models. The framework includes (1) targeted aspects of model performance to be evaluated; (2) a set of benchmarks as defined references to test model performance; (3) metrics to measure and compare performance skills among models so as to identify model strengths and deficiencies; and (4) model improvement. Component 4 may or may not be involved in a benchmark analysis but is an ultimate goal of general modeling research. Land models are required to simulate exchange of water, energy, carbon and sometimes other trace gases between the atmosphere and the land-surface, and should be evaluated for their simulations of biophysical processes, biogeochemical cycles, and vegetation dynamics across timescales in response to both weather and climate change. Benchmarks that are used to evaluate models generally consist of direct observations, data-model products, and data-derived patterns and relationships. Metrics of measuring mismatches between models and benchmarks may include (1) a priori thresholds of acceptable model performance and (2) a scoring system to combine data-model mismatches for various processes at different temporal and spatial scales. The benchmark analyses should identify clues of weak model performance for future improvement. Iterations between model evaluation and improvement via benchmarking shall demonstrate progress of land modeling and help establish confidence in land models for their predictions of future states of ecosystems and climate.





Hence, it is now feasible to create 

This trend opens new avenues for benchmarking, 



unique failure modes

The second difficulty is that different systems have different components, and therefore different, unique failure modes. Thus, it is difficult to 


Hence, they remained largely unexplored 


Hence, they remained  due to limited access and lack of repeatability. 




 In this paper, we discuss the evaluation of fourdifferent Infrastructure as a Service (IaaS) Cloud systems–from Amazon, Rackspace,and IBM–alongside a private Cloud installation of OpenStack, using a set of fiveso-called micro-benchmarks to address key aspects of such systems. The results fromour evaluation are offered on a web portal with dynamic data visualization.  On this basis, we can suggest that performance-basedpricing schemes would seem to be more appropriate than fixed-price schemes, andthis would offer much greater potential for the Cloud Economy. 
 
 





%73% of the organizations have a service availability goal of over 99.91% (less than 8 hours of unplanned downtime a year) for mission critical systems. That’s compared to 68% that had this goal in 2013





the diversity of emerging paradigms warrant the use of additional metrics that cover the full lifecycle of a system.  

Kubernetes can upgrade assigned resources to an instance or add more capacity to a running system by deploying new instances of each component and shifting load to them. 


By using Kubernetes API, users can dynamically , in order to the meet the desired system capacity. 


With  all  the  changes,  we believe it is now  necessary to  conduct  a  new  study  on  failures  in  modern  large-scale Internet data centers.

In view of this technological shift, we wonder if it possible to use Kubernetes API to realize the infrastructure insights missing from modern benchmarks, and investigate new metrics for understanding the tradeoffs between systems and the business models for which they are suited.  


This means Litmus triggers infrastructure events randomly and reports back on how Kubernetes handles it. 

Since, however, different infrastructures have different components, and therefore different, operating modes, it was difficult .


A key feature of the \textit{frisbee} framework/tool is that it is extensible — it supports easy definition of (1) device capabilities (2) network protocols and topologies (3) and events that modify the Testbed's behavior at runtime, simulating normal and abnormal conditions that dominate production environments. 

The impact of such failures may range from service downtime, to potential data losses. Yet, a failure may initiate a cascade of other failures to other service than can eventually bring down the whole system. Therefore, besides performance, it is also important to consider the scalability, availability, elasticity offered by a system. 


 However, the increasing number of emerging systems and the diverse range of applications makes it difficult for developers to choose the best-suited system for their business model. 










 
 that take humans out of the failure-recovery loop,
 In particular, MTTR is
 
 
 

The large variety of has made it difficult for developers to choose the appropriate system.
The most obvious differences are between the various data redundancy models, such as the replication-oriented used in [EXAMPLES] versus erasure coding used in [EXAMPLES].


 

However, the redundancy models can be documented and compared qualitatively. Comparing the recovery of various systems is harder problem. Some systems have made the decision to optimize for replication [...], while other have optimized for erasure coding [...].







enable recovery to happen 

and . 

detecting failures, and making the necessary adjustments to 







Hence,  To do so, they depend on data redundancy (e.g, replication or erasure coding) and employ models, whether external or internal, to monitor system behavior and use obtained inputs to adapt themselves to the run-time environment. 







open new avenues of exploring 


The number of emerging cloud serving systems and the wide range of proposed applications, coupled with a lack of apples-to-apples performance comparisons, makes it difficult to understand the tradeoffs between systems and the workloads for which they are suited.  


different systems have different components, and therefore different, unique failure modes.
 
 However, 








system that 




Self-healing systems 

These factors have actuated research dealing with the concept of self-healing systems. 


 and indulged operators to care less about hardware dependability.




Possible mitigation techniques include hardware redundancy (e.g, RAID, network links) and data redundancy (e.g, replication, erasure coding), or enhanced features such as detection systems making failures easier to notice and repair, predictive failure analysis, or systems partitioning.






For database benchmarking, inherit availability is the most appropriate availability metric, and represents only the corrective maintenance (CM) downtime of the system. 




Corrective maintenance is a maintenance task performed to identify, isolate, and rectify a fault so that the failed equipment, machine, or system can be restored to an operational condition within the tolerances or limits established for in-service operations

Inherent availability is the steady state availability when considering only the corrective maintenance (CM) downtime of the system. This classification is what is sometimes referred to as the availability as seen by maintenance personnel. This classification excludes preventive maintenance downtime, logistic delays, supply delays and administrative delays. Since these other causes of delay can be minimized or eliminated, an availability value that considers only the corrective downtime is the inherent or intrinsic property of the system. Many times, this is the type of availability that companies use to report the availability of their products (e.g., computer servers) because they see downtime other than actual repair time as out of their control and too unpredictable.






Availability, or more precisely, steady state availability, is the  Availability is typically measured either as uptime or downtime ratio. Banking and telecommunications systems are typical examples of high availability environments.



In general, availability describes uptime/downtime of a system in relation to time, accounting for both the reliability and maintainability properties of a system. Depending on the system, there are multiple definitions 












The classification of availability is somewhat flexible and is largely based on 

As a result, there are a number of different classifications of availability, including:














For Internet companies, however, an occasional loss of a localized service may be tolerable, a system-wide outage is unacceptable. 



There are mu

Availability is often measured by the uptime ratio—which is aclose approximation of the steady state availability value and represents the percentage of time a computer system is available throughout its useful life

Availability is an important metric used to assess the performance of repairable systems, accounting for both the reliability and maintainability properties of a component or system. However, there 







,  The lack of such a benchmark continues to leave a gap in the evaluation process, and it is generally agreed throughout the industry that a method for benchmarking availability is needed. 

elsayed2021reliability

Steady State Availability is the most commonly quoted availability metric, 

. Another frequently used availability metric isdowntime per yearwhich is calculated using thefollowing formula:










Each technique, however, comes with advantages and disadvantages. 


Example: 1 fault in SW RAID•  Compares Linux and Solaris reconstruction–Linux:Small impact but longer vulnerability to 2nd fault–Solaris:large perf. impact but restores redundancy fast–Windows: did not auto-reconstruct





System ArchitectureTo what extent can the system recover from a processing node failure:-Single node-Cluster-Active/active-Remote data mirroring-Demonstrated failover or recovery timeNo Single Point of Failurewithin a Single NodeEvery critical  component  should  have  a  backup  which  is  put  into  service  automaticallyupon the failure of its mate. These components include:-Processors-Memory-Controllers-Controller paths-Disks (mirrored gets a higher score than RAID 5)-Networks-Power supplies-FansHot Repair of System ComponentsFailed componentscan be removed and replaced with operational components withouttakingdownthe system:-Allof the components listed aboveDisaster Backup and Recovery-Availability of the backup site-Currency of backup data at the backup site:oBackup tapesoVirtual tapeoAsynchronous replicationoSynchronous replication-Demonstrated time to put the backup site into service

Compared to performance benchmarking, availability  is  still  in  its  infancy.  A  widely adopted  benchmarking framework  has  yet  to  be  designed.  This  is  partly  due  to  the complexity  of  such  a  task  and  the  problems  associated  with  it. Numerous  factors  have  to  be  taken  into  account,  and  there  is  adebate as to how to include these factors in the benchmark



General purpose computer systems, such as UNIX based systems, tend to execute the same sequence or series of steps during system startup and outage recovery. Our experience has shown that these 


Additionally, the factors that create variability in restart/recovery can be bound and represented in a meaningful way. A defined set of measurements, coupled with a specification for representing the results and system variables, provide the foundation for system recovery benchmarking.






The term fault-tolerant means a system can operate in the presence of hardware component failures. A single component failure in a fault-tolerant system will not cause a system interruption because the alternate component will take over the task transparently






The creation of staging environments for software testing was always an important topic. In this section, we analyze some of the approaches. We discuss the respective order: testbeds with real devices and networks, simulations based on mathematical models, and emulators based on virtual machines and containers. From the container-based solutions, we analyze works that are based on Docker Swarm, and Kubernetes-native solutions. \frisbee{} falls in the category of container-based emulators for Kubernetes.


In this paper, 

With new technological trends, however, 

describes the failure rate of hardware , and latter the the time it takes for maintenance team to repair a failure. However, the emergence of self-healing systems open new avenues for benchmarking availability.


 By taking humans out of the failure-recovery loop, such systems not only , but they also render MTTR measurable. 

 
 a benchmark specification designed 

key/value databases and introduces a Kubernetes-native prototype. 




We have spent a decade perfecting performance measuring via formal benchmarks. There was not much attention given to systems availability since (a) cluster scales were rather small (b) systems did not have to run 24x7. 



Understanding the performance implications of the decisions for a given type of application is challenging. 


This article introduces different system categories to help find a server type best
suited to specific business availability needs. This information will assist administrators in making decisions when attempting to balance cost against availability






and .


Repairs are intended to remove faulty components and restore a system to a functional Upgrades are implemented to replace the current hardware or software withnewer (or enhanced) versions.


 Unfortunately, both metrics are business-specific and . MTBF depends on the , and MTTR is dominated by 


the removal of human factors renders availability a factor of 







 







There  are many problems to solve in order to achieve meaningful availability benchmarks, primarily due to the infrequency of failures in the field.



This article also covers basic
fundamental concepts—basic mathematics is emphasized for the sake of simplicity—
of Reliability, Availability, and Serviceability (RAS) relating to the hardware, operating
systems, and application elements. 

\todo[inline]{State}. 

\todo[inline]{Description about systems replication, raid, erasure coding}






The speed with
which a system can return to service following an outage
is a critical factor in overall system availability

-- Start discussing about mean-time to repair ?






Unlike hardware MTBF, system MTBF, and MTBI are measurements of events visibleto end users. System failures can result in extended periods of application servicelevel outage, while most system interruptions result in short outages that in manycases are restored without human intervention

Hardware MTBF is probably the most frequently cited MTBF metric even though itdoes not reflect the typical end-user view of a reliable service level becausehardware component failures do not necessarily result in a system interruption






 often go hand-in-hand with availability, and sometimes the differences are subtle.  gives a good explanation of reliability versus availability. 


Although this need has been longed discussed, 




For Internet companies, availability/uptime 





Although an occasional lossof a localized service may be tolerable, a system-wide outage is unacceptable.Banking and telecommunications systems are typical examples of highavailability environments

Sun cluster systems assist in the recovery from both hardware and softwarefailures, whereas a fault-tolerant system has the operating system and application asa single point of failure.


 However, a careful analysis of availability attributes can lead to a good start toward obtaining useful availability metrics

\item Rate (rate of fault and maintenance events), 
    \item Robustness (a system's ability to handle fault, maintenance, and
system-external events and the resulting degree to which it remains available in the face of these events), 
    \item Recovery (the speed with which a system can return to
operation following an outage). 

. Previous research
in availability benchmarking has been focused on
benchmarking system robustness attribute [1, 2, 3, 6]. There has been a lack of research in benchmarking recovery aspect of system availability


Alternatively, benchmarks can be defined that focus on
some subset of the framework attributes and their submetrics. This is very similar to the performance benchmarking space, where there are benchmarks that
measure the system as a whole, as well as benchmarks
that measure a specific subsystem.


Under application-level availability, a system is deemed available as long as the Queries per second and Tail latency is acceptable to the end-user.

 When an availability fault is corrected, it is essential that access to uncorrupted data is restored

Open sourcing is just a starting point. In addition to the infrastructure-level chaos experiments introduced in previous sections, we are in the process of supporting a wider range of fault types of finer granularity, such as:

    Injecting errors at the system call and kernel levels with the assistance of eBPF and other tools
    Injecting specific error types into the application function and statement levels by integrating failpoint, which will cover scenarios that are otherwise impossible with conventional injection methods



In [7], a hierarchical framework, named R3
, is
established to benchmark availability. R3 represents the
three system attributes that are key to availability
identified in the framework. These attributes are Rate
(rate of fault and maintenance events), Robustness (a
system's ability to handle fault, maintenance, and
system-external events, and the resulting degree to which
it remains available in the face of these events), and
Recovery (the speed with which a system can return to
operation following an outage). The R3 framework
provides for a benchmark that incorporates all defined
attributes, thus yielding a downtime-per-year metric.




In this paper, we discuss our rationale 
Our objective is to convey two basic assertions: recovery
time can be benchmarked; and a recovery time
benchmark is useful and meaningful. 
of using recovery time for measuring availability, and introduces a framework which can be used to implement availability benchmarks that are applicable across a wide range of systems.





Failures in a syste 

in the chain—cables, power supplies, cooling, drives, software (and even the sys admins).

may occur at all 




This includes all elements 


Our perspective: Dependability and Cost of Ownership are the upcoming challenges –  Past challenges: Performance and Cost of Purchase



disrupt access to users’ data. 




 adopted scalable key/value databases to accommodate larger loads. At the same time, 


systems , just by adding resources either making hardware stronger (scale up) or adding additional nodes (scale out). At the same time, 







However, the heterogeneity in both hardware components and workload, result in even more complex failures. 


Developers of various database systems frequently state replication, erasure-coding, and many other self-healing approaches. However,  they seldom report measured numbers. There is good reason for that. 
\comment{backup, Systems offering replication, systems offering erasure-coding}





, making sure that data remains accessible and intact whenever are needed. 




Critical to microservices organizations is the need to understand large amounts of computer-generated data and instantly pinpoint availability concerns and identify threats in any complex, distributed systems. 


The scope of our reproduced experiments is extended with a performance evaluation of Cassandra on different Amazon EC2 infrastructure configurations, and an evaluation of Cassandra and HBase elasticity by measuring scaling speed and performance impact while scaling.



scenarios that needs to be handled by the system, including the disk, the network, the power source, or the system itself. 



performance it yields . To quantify user satisfaction, we rely on application-level performance metrics that capture .




discuss a core set of scenarios and compare key aspects of four widely used systems: MongoDB, TiDB, TIKV, Cockroach. We specifically examine resource utilization, hotspots, time to recover, , and data loss. 

This paper 

 We conduct a detailed fault susceptibility study that measures how much more fault resilient programs are when defining correctness at the application level compared to the architecture level. 




system recovery benchmark for Kubernetes. 

Our goal in this effort is to define 



besides performance, engineers have to face four major challenges: scalability, elasticity, availability and durability. 

Benchmarks have historically guided research and development in computer systems performance. 

conditions.

This paper proposes a framework for benchmarking the availability of computer systems.  The proposed framework is a hierarchical approach which goes beyond direct benchmarking of availability in terms of number of outage minutes per year. This paper identifies the three key attributes impacting system availability (fault and maintenance rate, robustness, and recovery), and methods to benchmark these key attributes of availability


Traditionally, fault tolerance researchers have required architectural state to be numerically perfect for program execution to be correct. However, in many programs, even if execution is not 100% numerically correct, the program can still appear to execute correctly from the user's perspective. Hence, whether a fault is unacceptable or benign may depend on the level of abstraction at which correctness is evaluated, with more faults being benign at higher levels of abstraction, i.e. at the user or application level, compared to lower levels of abstraction, i.e. at the architecture level. The extent to which programs are more fault resilient at higher levels of abstraction is application dependent. Programs that produce inexact and/or approximate outputs can be very resilient at the application level. We call such programs soft computations, and we find they are common in multimedia workloads, as well as artificial intelligence (AI) workloads. Programs that compute exact numerical outputs offer less error resilience at the application level. However, we find all programs studied in this paper exhibit some enhanced fault resilience at the application level, including those that are traditionally considered exact computations - e.g., SPECInt CPU2000. 



At scale, new conditions arise that warrant new benchmarks for resource utilization, elasticity, heterogeneity, and failure handling.





Today, more DevOps teams leverage the power of containerization and technologies like Kubernetes to automate and manage database clusters. Reasons to do so include rapid spin-up of isolated clusters, repeatability across environments, and dynamic changes at the level of infrastructure. Another advantage is that Kubernetes provides a centralized logging infrastructure for all applications and services to funnel logs into a single pipeline. The net effect is that we correlate an infrastructure event with application logs, and find out how systems and operating environments intermix and work together.



%Other researchers [26] are doing work to benchmark analytical systems such as these. Similarly,there are existing benchmarks for a variety of data storagesystems (such as SQL databases [22] and filesystems [12,10]).  However, the novel interfaces (usually neither SQLnor POSIX), elasticity, and new use cases of cloud serving systems motivate a new benchmark.








-- conducive to the replication of real-world environments. 


unable 
to assess elasticity, availability, and durability of databases.






scaling capabilities, and database availability under a variety of different faults. 








In this context, it seems a bit ironic that these qualities are provided by dozens of systems, but there is no competent benchmark suite for their evaluation. 




 

The performance of Cloud systems is a key concern, 


A  modern  Web  benchmark  should  have  realism  along  three  key  dimensions:  (i)  a  realistic  server-side  application,  (ii)  a  realistic  Web  workload  generator  that  faithfully  emu-lates  user  behavior,  and  (iii)  a  realistic  workload  injec-tor  that  emulates  the  actual  “browser  experience.” 


\begin{itemize}
    \item \textbf{scale-up:} help developers to study a set of performance points that show how an application's performance changes when additional resources (e.g., CPU cores, memory, faster disks) are added.
    
\end{itemize}

\begin{itemize}
    \item a framework and its API for scalability, elasticity, availability and durability experiments.
    \item a series of scenarios for comparing the baselines different systems present
    \item a series of metrics for quantifying the impact of the above scenarios to the running system. 
\end{itemize}







Automation doesn’t remove human influence– shifts the burden from operator to designer» designers are human too, and make mistakes» unless designer is perfect, human operator still needed

Automation can make operator’s job harder– reduces operator’s understanding of the system» automation increases complexity, decreases visibility» no opportunity to learn without day-to-day interaction– uninformed operator still has to solve exceptional scenarios missed by (imperfect) designers» exceptional situations are already the most error-prone


Improving recovery/repair improves availability– UnAvailability =  MTTRMTTF– 1/10th MTTR just as valuable as 10X MTBF


“Macro” benchmarks for competition, must be fair, hard to game, representative; use ~ 10 operators in routine maintenance and observe errors; insert realistic HW, SW errors stochastically– “Micro” benchmarks for development, must be cheap;inject typical human, HW, SW errors •
– initial recovery benchmarks find peculiarities– Lots of low hanging fruit (~ early RAID days)






Traditional performance benchmarks rely on workload generators that send requests from clients to servers. In this context, performance benchmarks are unable for the measurement of elasticity, availability, or durability of databases, since these qualities require to change the infrastructure while the system is running.



 



This documentmay not be distributed in any way by electronic means.©2007Sombers Associates, Inc., and W. H. Highleymanwww.availabilitydigest.com1Availability DigesttheLet’s Get an Availability BenchmarkJune 2007Benchmarks have been around almost as long as computers, Benchmarks are immenselyvaluable to buyers of data processing systems forcomparingcost and performance of thesystemswhich they are considering. They are of equal value to system vendors to comparethe competiveness of their products with others.In  the  early  days  of  computing,  there  were  no  formal  benchmarking  specifications;andvendors were free to define their ownbenchmarks. This,of course,led to a great disparity inresults  and  benchmark  claims. 


Virtually all of today’s accepted benchmarks focus on performanceand cost. 



Think aboutit.  Consider  a  critical  application  in  which  the  cost  of  downtime  is  $100,000  per  hour.  Thecompany running the application chooses a system which costs $1 million dollars and which hasan availability of three 9s (considered today to be a “high availability” system). An availability ofthree 9s means that the system will be expected to be down an average of only eight hours peryear. However, over the five-year life of this milliondollar system, it will be down about 40 hoursat a cost of $4 million dollars.$1 million  dollars for the system  and $4 million  dollars for downtime. There has to be a  betterway.One  solution  to  this  problemisto  provide  purchasers  of  systems  not  only  performance/costmetrics  but  also  availability  measures.  A  company  could  then  make  a  much  more  informeddecision as to the system which would be best for its purposes.


Οιπαράγοντες  που  πρέπει  να  εξεταστούν  για  να  μπορέσουν  επιτυχημένα  να επιτευχθούν  οι υπηρεσίεςτης Ηλεκτρονικής Διακυβέρνησης, είναι η ορθότητα (efficacy),η αποδοτικότητα (efficiency)και η αποτελεσματικότητα (effectiveness). Το κριτήριο της  ορθότητας  εξετάζει  αν  τα  αποτελέσματα  είναι  σωστά,αν  δηλαδή  ο  πολίτης  θα εξυπηρετηθεί για αυτό που αιτείτε. Το κριτήριο της αποδοτικότητας εξετάζει τη χρήση πόρων που απαιτούνται για την ορθή λειτουργία,όπου εδώ ελέγχεται ο χρόνος αναμονήςκαι  η  σπατάλη  πόρων  στην  εξυπηρέτηση. Και  το  κριτήριο  της  αποτελεσματικότηταςεξετάζει το συνολικό όφελος, αν είναι ικανοποιημένος ο πολίτης από τις υπηρεσίεςπου τουπαρήχθησα






The main idea is that you capture a workload from production, you extract some performance information, then you replay the same workload to one or more environments that you want to put to test, while capturing the same performance information. At the end of the process, you can compare performance under different conditions, identify regressions, avoid unwanted situations and rate your tuning efforts.


f you want to replay a workload from production to test, you need to be able to capture the workload first. Even before you start, you’re already confronted with a myriad of questions:

What do you use for this? A server-side trace? Extended events? Profiler maybe?
Which events do you capture? Which fields?
How long do you need to run the capture? How much is enough? One hour? One day? One week? One month?
Can you apply some filters?
Will you have enough disk space to store the captured data?

Fault instrumentation can be used in systems with limited redundancy to achieve high availability. Maintenance actions occur during brief periods of down-time only after a fault indicator activates. Failure is only significant if this occurs during a mission critical period.




there is not only variability in performance by provider, but also variability,which can be substantial, in the performance of virtual resources that are apparently 





We  examine  the  dataset  statistically  to  discover  failurecharacteristics   along   the   temporal,   spatial,   product   line   andcomponent  dimensions.  We  specifically  focus  on  the  correlationsamong different failures, including batch and repeating failures,.  Wereconfirm or extend findings from previous studies. We also findmany new failure and recovery patterns that are the undesirableby-product   of   the   state-of-the-art   data   center   hardware   andsoftware  design.







\section{Abstractions}

\subsection{Infrastructure}

\subsection{Databases}

\subsection{Chaos}

\subsection{Event notifier}

\subsection{Metrics}

\subsection{Object Modelling}

\subsubsection{Nodes}
\begin{itemize}
    \item Memory
    \item CPU
    \item Storage (capacity, throughput, IOPS)
\end{itemize}


\subsubsection{Networks}
\begin{itemize}
    \item TCP-based
    \item RDMA
\end{itemize}












\subsection{Overview}

Now Let’s see what are the components of Chaos Mesh:

    Chaos Operator: the core component for chaos orchestration. Fully open-sourced.
    Chaos Dashboard: a Web UI for managing, designing, monitoring Chaos Experiments; under development.

\subsection{Automate Chaos Pipeline}



UI to visualize and manage Workflows
Loops
Parameterization
Conditionals
Timeouts (step & workflow level)
Retry (step & workflow level)
Prometheus metrics

    
\subsection{Chaos Sceduling}
Service owners can now express a schedule in terms of the mean time between terminations, rather than a probability over an arbitrary period of time. We also added grouping by app, stack, or cluster, so that applications that have different redundancy architectures can schedule Chaos Monkey appropriate to their configuration. Chaos Monkey now also supports specifying exceptions so users can opt out specific clusters. 


\subsection{Event Tracking}
Chaos Monkey can now be configured for specifying trackers. These external services will receive a notification when Chaos Monkey terminates an instance. Internally, we use this feature to report metrics into Atlas, our telemetry platform, and Chronos, our event tracking system.
The graph below, taken from Atlas UI, shows the number of Chaos Monkey terminations for a segment of our service. We can see chaos in action. Chaos Monkey even periodically terminates itself.


















Now CustomResourceDefinition or CRD is a powerful Kubernetes feature that basically extends the Kubernetes API to allow you to define custom resources. Chaos Mesh uses this ability of Kubernetes to define custom chaos objects like the 6 chaos types we mentioned earlier. Chaos Mesh also leverages existing CRD implementations wherever applicable and allows you to use existing CRDs to build new objects to start chaos experiments with. New objects can be created or existing CRDs updated with a YAML file or a Kubernetes API.

The YAML method is the preferred method here, especially since it can conduct chaos experiments post-deployment. To create your own custom chaos experiment, you need to create your own YAML config file though it’s pretty easy to find examples online. Alternatively, CRDs can be manipulated directly through the Kubernetes API. The fact that Chaos Mesh defines chaos objects with CRDs makes it a natural fit for Kubernetes for Kubernetes-based applications. This also makes installation a lot easier since it’s as simple as applying a set of CRDs to a cluster.


With Chaos Mesh 1.0, Chaos Dashboard is available to everyone. Chaos Dashboard greatly simplifies the complexity of chaos experiments. With only a few mouse clicks, you can define the scope of the chaos experiment, specify the type of chaos injection, define scheduling rules, and observe the results of the chaos experiment—all in the same web interface.

% operators can create templates for network devices (define network traffic policies), templates for IoT components (define CPU, MEMORY, IOPS, network devices), combine IoT components and application into services, and define phases and phase-dependencies for the experiment. 






CustomResourceDefinitions design

Chaos Mesh uses CustomResourceDefinitions (CRD) to define chaos objects. In the Kubernetes realm, CRD is a mature solution for implementing custom resources, with abundant implementation cases and toolsets available. Using CRD makes Chaos Mesh naturally integrate with the Kubernetes ecosystem.

Instead of defining all types of fault injections in a unified CRD object, we allow flexible and separate CRD objects for different types of fault injection. If we add a fault injection method that conforms to an existing CRD object, we scale directly based on this object; if it is a completely new method, we create a new CRD object for it. With this design, chaos object definitions and logic implementation are extracted from the top level, which makes the code structure clearer. This approach also reduces the degree of coupling and the probability of errors. In addition, Kubernetes’ controller-runtime is a great wrapper for implementing controllers. This saves us a lot of time because we don’t have to repeatedly implement the same set of controllers for each CRD project.

Chaos Mesh implements the PodChaos, NetworkChaos, and IOChaos objects. The names clearly identify the corresponding fault injection types.





spec:
 action: pod-kill
 mode: one
 selector:
   namespaces:
     - tidb-cluster-demo
   labelSelectors:
     "app.kubernetes.io/component": "tikv"
  scheduler:
   cron: "@every 2m"

This code does the following:

    The action attribute defines the specific error type to be injected. In this case, pod-kill kills Pods randomly.
    The selector attribute limits the scope of chaos experiment to a specific scope. In this case, the scope is TiKV Pods for the TiDB cluster with the tidb-cluster-demo namespace.
    The scheduler attribute defines the interval for each chaos fault action.
    
    
    \subsection{Running chaos using a YAML file}
    
    \subsection{Running chaos using Kubernetes API}
    
    
    
    
    Chaos Mesh is designed for Kubernetes. Chaos Mesh:

    Requires no special dependencies, so that it can be deployed directly on Kubernetes clusters, including Minikube.
    Requires no modification to the deployment logic of the system under test (SUT), so that chaos experiments can be performed in a production environment.
    Leverages existing implementations so that fault injection methods can be easily scaled.
    Integrates with other testing frameworks.



CustomResourceDefinitions Design

Chaos Mesh uses CustomResourceDefinitions (CRD) to define chaos objects. In the Kubernetes realm, CRD is a mature solution for implementing custom resources, with abundant implementation cases and toolsets available. Using CRD makes Chaos Mesh naturally integrate with the Kubernetes ecosystem.

Instead of defining all types of fault injections in a unified CRD object, we allow flexible and separate CRD objects for different types of fault injection. If we add a fault injection method that conforms to an existing CRD object, we scale directly based on this object; if it is a completely new method, we create a new CRD object for it. 

With this design, chaos object definitions and logic implementation are extracted from the top-level, which makes the code structure clearer. This approach also reduces the degree of coupling and the probability of errors. In addition, Kubernetes’ controller-runtime is a great wrapper for implementing controllers. This saves us a lot of time because we don't have to repeatedly implement the same set of controllers for each CRD project.



For true operators you want to keep the responsibility isolated to managing a single CRD. But you might need to interact with other CRDs that the operator doesn’t manage. For example, maybe you’re providing a way to provision instances of a content management system and the content management system itself uses mongodb as a dependency. Then you might want your content management operator to submit mongobdb instances to the kubernetes API.




Since there is no such thing as Linux containers in the kernelspace, containers are various kernel features tied together, when you are building a large platform or distributed system you want an abstraction layer between your management code and the syscalls and duct tape of features to run a container.  That is where containerd lives.  It provides a client layer of types that platforms can build on top of without ever having to drop down to the kernel level.  It’s so much nicer towork with Container, Task, and Snapshot types than it is to manage calls to clone() or mount().

Containerd was designed to be used by Docker and Kubernetes as well as any other container platform that wants to abstract away syscalls or OS specific functionality to run containers on linux, windows, solaris, or other OSes.  With these users in mind, we wanted to make sure that containerd has only what they need and nothing that they don’t.  Realistically this is impossible but at least that is what we try for.  Things like networking are out of scope for containerd.  The reason for this is, when you are building a distributed system, networking is a very central aspect.  With SDN and service discovery today, networking is way more platform specific than abstracting away netlink calls on linux.  Most of the new overlay networks are route based and require routing tables to be updated each time a new container is created or deleted.  Service discovery, DNS, etc all have to be notified of these changes as well.  It would be a large chunk of code to be able to support all the different network interfaces, hooks, and integration points to support this if we added networking to containerd.  What we did instead is opted for a robust events system inside containerd so that multiple consumers can subscribe to the events that they care about.  We also expose a task API that lets users create a running task, have the ability to add interfaces to the network namespace of the container, and then start the container’s process without the need for complex hooks in various points of a container’s lifecycle.

Another area that has been added to containerd over the past few months is a complete storage and distribution system that supports both OCI and Docker image formats.  You have a complete content addressed storage system across the containerd API that works not only for images but also metadata, checkpoints, and arbitrary data attached to containers.

We also took the time to rethink how “graphdrivers” work.  These are the overlay or block level filesystems that allow images to have layers and you to perform efficient builds.  Graphdrivers were initially written by Solomon and I when we added support for devicemapper.  Docker only supported AUFS at the time so we modeled the graphdrivers after the overlay filesystem.  However, making a block level filesystem such as devicemapper/lvm act like an overlay fillesystem proved to be much harder to do in the long run.  The interfaces had to expand over time to support different features than what we originally thought would be needed.  With containerd, we took a different approach, make overlay filesystems act like a snapshotter instead of vice versa.  This was much easier to do as overlay filesystems provide much more flexibility than snapshotting filesystems like BTRFS, ZFS, and devicemapper as they don’t have a strict parent/child relationship.  This helped us build out a smaller interface for the snapshotters while still fulfilling the requirements needed from things like a builder as well as reduce the amount of code needed, making it much easier to maintain in the long run.







with an autonomous behavior


This automation not only reduces , but it also makes the recovery time consistent, reproducible, and measurable, and can thus be benchmarked.




thus making the recovery process both consistent and measurable.

These auto reboot/quick recovery
mechanisms tend to execute the same sequence of
steps, 

allows to measure the time it takes for a system to regain normative performance levels after a failure. 

to benchmark recovery time. 


By , these design not only reduce recovery time from slow , but they are guarantee that 

self-healing properties that 

, and 

self-healing databases today implement recovery designs that 

at fast  rather than . Other than minimizing recovery time, these designs tend  

 and

Some systems achieve 





Reliability provides a metric of how often a component fails, while availability includes the effects of downtime any failures produce.  Serviceability  is  synonymous  with  recoverability  -the  characteristic  of  a  system’s  reaction  to  faults,  errors,  and maintenance



 Some have taken a metric such as MTBF and misconstrued it to mean something quite different. 
There are many ways to classify a system, which can change the benchmark dramatically. 

Each typeof  system  has  different  availability  requirements,  contingenton  their  usages.  For  example,  on-board  avionic  computersystems have entirely different standards than an engineeringsimulation  system,  or  even  a  network  storage  system.  Therequirements are drawn up from users, customers, and some-times  developers.  To  fulfill  the  requirements,  a  benchmarkcould define a system based on its availability, from which asystem could be selected. In another application, a benchmarkcould  determine  what  effect  a  change  in  the  system  wouldmanifest.




In this paper, we discuss how Chaos testing and Observability tools can be used for measuring the recovery attribute of self-healing databases, and present a prototype benchmark based on Kubernetes. 


Nevertheless, there is one common underlying idea: introducing an autonomousbehavior to handle an otherwise complex and unmaintainable system. This autono-mous behavior must independently take decisions at runtime and manage the assignedsystem. Management actions (e.g., configure, adapt, recover) are goal dependent, how-ever, must result in a consistent system. The success of an adequate autonomousbehavior depends on an accurate system knowledge. Both, autonomic computing andself-adaptive system research [72,75] agree, only the knowledge of internal state (selfaware) and external situation (context aware) allows for proper adaptation. This com-bined awareness is gained by filtered data from sensing and feedback from effect-ing interfaces aligned to the context resulting in an accurate system overview. Tokeep a current view and meet contingent time constraints a closed loop system isassumed.


evaluation of individual  of select system components and their combined effects on the system.

he  benchmark  can  also  test  









Portability is an especially challenging topic for benchmarks 

. A properavailability benchmark would 

This is especially true for availability 

In performance benchmarking, the variances in results are usually masked by considering only the relative performance amongst evaluated systems. For availability benchmarks, however, this is especially problematic since 


authors typically state their experimentation platforms, until now 

However, the number and types of failures a system can tolerate . Comparing the actual recovery time of various systems is a harder problem. 




JANUS introduces a model using Object Oriented Analysis (OOA) from which a virtual testbed can be almost automatically generated. Operators 






the state of the system at the time of failure is important. A temporary network delay between servers may go unnoticed during an idle period, but it can set off a cascade of events if it happens during a replication process. While arbitrary (randomly) injected faults may seems appropriate for testing a system's robustness, 




 

In contrast to performance and scalability of cluster-based services that have been studied extensively in the literature, recoverability has received much less attention.



, e.g., [3], [6], [8]. In contrast, understandingdesigns for availability, behavior during component faults,and the relationship between performance and availabilityof these services 



In this paper we develop a methodology that combines fault-injection with modeling to quantify the 



that .


Regardless of the technology, these systems share the goal of automating the recovery process and 




The performance and scalability of cluster-based services have been studied extensively in the literature. In contrast, understanding designs for availability, behavior during component faults,and the relationship between performance and availability of these services has received much less attention.



 

%f  the  faultload  designer  is  not  careful,  he  or  shemay  inject  the  fault  at  a  level  where  a  check  would  havealready  been  made,  such  as  after  checking  the  parity  bitsbut  before  retrieving  and  using  the  memory. 




\CHECKnote{[MM] Summary of challenges ? (matching Section 3) Summary of approach and main contribution ?}


 
 
 %In this paper, we propose a two-phase methodology for systematically evaluating the performability (performance andavailability) of cluster-based Internet services. In the first phase, evaluators use a fault-injection infrastructure to characterize theservice’s behavior in the presence of faults. In the second phase, evaluators use an analytical model to combine an expected fault loadwith measurements from the first phase to assess the service’s performability. Using this model, evaluators can study the service’ssensitivity to different design decisions, fault rates, and other environmental factors. To demonstrate our methodology, we study theperformability of a multitier Internet service. In particular, we evaluate the performance and availability of three soft state maintenancestrategies for an online bookstore service in the presence of seven classes of faults. Among other interesting results, we clearly isolatethe effect of different faults, showing that the tier of Web servers is responsible for an often dominant fraction of the serviceunavailability. 
 

Prelude to self-healing is data redundancy; some system employ erasure coding models[EXAMPLE, whereas others rely on simpler replication models, which can be either synchronous [EXAMPLE] or asynchronous [EXAMPLE]. 


It will also benefit developers and researchers to have a metric to determine the best course of action for system design.







However, every solution is based on a different set of design choices, contingent on their usages. 

These services must therefore exhibit several characteristics, including high performance, scalability, and availability. 

To study 


The performance and scalability of these services have been studied extensively in the literature[EXAMPLES]. In contrast, understanding designs for availability, behavior during component faults, and the relationship between performance and availability of these services have received much less attention. 


To meet the ever-growing demand for Internet services, 

people build large clusters of commodity computers as their supporting infrastructure. 

 

 







[ EXAMPLES ]


The large variety has made it difficult for developers to choose the appropriate system. 





In an always-on world where systems are expected to operate continually, 

   
Although today's service designers 



Over time, there has been a plethora benchmarks for apples-to-apples comparison between systems. 


To enable companies choose the right system for their needs, there have been several benchmarks for an 

Over time there have been  amongst there. 



While today there has been an explosion of high-available services [EXAMPLE], the design and evaluation of service availability is still an art based on the practitioner’s experience and intuition, rather than a scientific methodology.



Understanding how well each system achieves those goals is important for companies 

However, the large variety has made it difficult for developers to choose the appropriate system. Some aspects can be documented and compared qualitatively, such as the number and types of tolerated failures, but  quantifying the effectiveness of recovery mechanisms is harder problem. 

Firstly, the metrics must be relevant across  two architecturally different systems. Secondly, a performance benchmark is as good as its workloads. Similarly, an availability benchmark is as good as its faultloads. Thirdly, while arbitrary fault injection may seem appropriate for testing a system's robustness, as happens in Chaos testing, randomness impedes the repeatability of a benchmark. And last, a benchmark should be portable across experimentation platforms. 



Choosing appropriate system for their needs is important for Internet Companies as it helps to strike the right balance among software complexities, hardware reliability, and operation cost, thus reducing the total cost of ownership (TCO) in data centers.










 Furthermore, the state of the system at the time of failure is important. A temporary network delay between servers may go unnoticed during an idle period, but it can set off a cascade of events if it happens during a replication process. 
\CHECKnote{[MM] missing citations: why mention only "databases" ?}


\CHECKnote{[MM] benchmark vs. benchmarking framework ? Is it about extensibility ?}


\CHECKnote{[MM] Summary of challenges ? (matching Section 3) Summary of approach and main contribution ?}


%Understanding the performance implications of these de-cisions for a given type of application is challenging.  De-velopers of various systems report performance numbers forthe “sweet spot” workloads for their system, which may notmatch the workload of a target application. Moreover, anapples-to-apples comparison is hard, given numbers for dif-ferent systems based on different workloads. Thus, devel-opers often have to download and manually evaluate mul-tiple systems.  Engineers at Digg [20] reported evaluatingeight different data stores in order to implement one feature(the Green Badge, or “what have my friends dugg” feature).There have been multiple similar examples at Yahoo!. Thisprocess is time-consuming and expensive


%Furthermore, the state of the system at the time of failure is important. A temporary network delay between servers may go unnoticed during an idle period, but it can set off a cascade of events if it happens during a replication process. 

 










\CHECKnote{[MM] Summary of challenges ? (matching Section 3) Summary of approach and main contribution ?}
%The  remainder  of  the  paper  is  organized  as  follows:  Section  2  lists  a  few  of  the  metrics  commonly  associated  with availability. Section 3 details some of the factors pertinent to the  topic  such  as  typical  hardware  failures.  Section  4  briefly discusses different modeling techniques for testing. Section 5explains issues related to workloads in fault-injection testing.Section  6  covers  a  few  of  the  known  problems  that  present roadblocks  and  misrepresentation.  Lastly,  section  7  presents what other research is being done and section 8 concludes thepaper




%As such, we do not expect papers to necessarily include a rigorous evaluation, although we do prefer papers that provide a crisp problem statement, a compelling motivation for the work, and some contextualization with respect to related academic work and the current state-of-the-art in industry.


%








 


Reliability  and  serviceability  often  go  hand-in-hand  withavailability,  and  sometimes  the  differences  are  not  apparent.[1] gives a good explanation of reliability versus availability.Reliability provides a metric of how often a component fails,while availability includes the effects of downtime any failures produce.  Serviceability  is  synonymous  with  recoverability  -the  characteristic  of  a  system’s  reaction  to  faults,  errors,  and maintenance evenets





the impact of changes from one version to another on availability, and therefore, performability, producing a more complete picture than just the previous data on performance.








In various embodiments, a node manager configures a “new” node as a replacement for an “unavailable” node that was previously included in a distributed data store. First, the node manager identifies a source node that stores client data that was also stored in the unavailable node. Subsequently, the node manager configures the new node to operate as a slave of the source node and streams the client data from the source node to the new node. Finally, the node manager configures the new node to operate as one of multiple masters nodes in the distributed data store. Advantageously, by configuring the node to implement a hybrid of a master-slave replication scheme and a master-master replication scheme, the node manager enables the distributed data store to process client requests without interruption while automatically restoring the previous level of redundancy provided by the distributed data store.

Software vendors often report performance numbers for the sweet spot or running on specialized hardware with specific workload parameters and without realistic failures. Accurate benchmarks at the persistence layer are crucial, as failures may cause unrecoverable errors such as data loss, inconsistency or corruption. To accurately evaluate data stores and other microservices at Netflix, we developed Netflix Data Benchmark (NDBench), a Cloud benchmark tool. It can be deployed in a loosely-coupled fashion with the ability to dynamically change the benchmark parameters at runtime so we can rapidly iterate on different tests and failure modes. NDBench offers pluggable patterns and loads, support for pluggable client APIs, and was designed to run continually. This design enabled us to test long-running maintenance jobs that may affect the performance, test numerous different systems under adverse conditions, and uncover long-term issues like memory leaks or heap pressure.






% Replicas may affect recovery (send raw data, vs sending the index)


%With failure pattern characterization remaining an open challenge, the next best thing in  comparing systems from different vendors is to have micro-benchmarks that measure how fast a system can detect a failure, the blast radius of the failure, and the time it takes for a system to recover from it. 


Such systems employ models, whether external or internal, to monitor system behavior and use inputs obtaining therefore to adapt themselves to the runtime environment.



   some  of  the  benchmarks  wereperformed in an ad-hoc manner using a combination of APIs,making direct REST calls in each microservice, or using toolsthat  directly  send  traffic  to  the  data  stores.  However,  mostbenchmark  tools  are  not  integrated  as  microservices  and  donot  have  out  of  the  box  cluster  management  capabilities  anddeployment strategies


 Being a cloud-native enterprise, we want to make sure that oursystems  can  provide  high  availability  under  multiple  failures cenarios,  and  that  we  are  utilizing  our  resources  optimally.There  are  many  other  factors  that  affect  the  performance  ofa  database  such  as  the  hardware,  virtualized  environment,workload  patterns,  number  of  replicas  etc.
 
 
 %hile some tools covereda subset of our requirements, we were inte%ested in a tool thatcould achieve the following:•Single  benchmark  framework  for  all  data  stores  andservices•Dynamically  change  the  benchmark  configuration  and workload while the test is running.
 
 %est a platform along with production microservices•Integrate  with  fundamental  platform  cloud  services  likemetrics, discovery, configurations etc.•Run  for  an  unlimited  duration  in  order  to  test  perfor-mance under induced failure scenarios and long runningmaintenance jobs such as database anti-entropy repairs.•Deploy,  manage  and  monitor  multiple  instances  from  asingle entry point.
 
 %etflix Data Benchmark (NDBench) is a pluggable cloud-enabled benchmarking tool that can be used across any data store system. NDBench provides plugin support for several data stores and can be extended to other client APIs..
 
 
 %e  incorporated  NDBench  into  the  Netflix  Open  SourceSoftware (OSS) ecosystem by integrating it with componentssuch as Archaius for configuration management [14], Spectatorfor metrics [19], and Eureka for service registration [18]. How-ever, we designed NDBench so that these libraries are injected,allowing the tool to be ported to other cloud environments, runlocally, and at the same time satisfy our Netflix OSS ecosystemusers. We have been running NDBench for almost three years,having validated multiple database versions, tested numerousNoSQL  systems  running  on  the  Cloud,  identified  bugs,  andtested new functionalities
 
 
 
 %Modern architectures and infrastructure are ephemeral and dynamic, with unpredictable user behavior intersecting with unforeseeable events. Our systems have begun to function less like predictable metal machines, and more like biological machines with emergent behaviors.
 
 
%Faults may be injected at various levels including the operating system (CPU, memory), the network level, or the application itself. Using a clustered database as an example, Chaos Engineering works by simulating a network partition between two database servers and lets the operator analyzes how this failure affects the QPS (queries per second).


%For clustered systems, recovery (and the notion of
%returning to service) takes on a somewhat different
%meaning, since clusters provide levels of
%redundancy on services, and a fatal condition on a
%cluster node may not result in a service disrup









% Problem statement
These services must therefore exhibit several characteristics, including high performance, scalability, and availability. Over time, there have been numerous benchmarks for comparing the performance and scalability of those services. In contrast, as of today, there is no industry-wide benchmark for availability. 


% Challenge



% Approach







 measures a repeatable set of quantifiable results that serves as a point of reference against which products/services can be compared. The purpose of benchmark testing results is to compare the present and future software releases with their respective benchmarks.

We choose to focus our effort on availability within the
dependability space because availability can be measured by well-defined metrics, and also because
availability is what customers care about most today.

recovery), and methods to benchmark these key attributes of availability
%Assessing
%availability today involves examining the features
%of the hardware and software designed to keep the
%system running, since an agreed-upon industry
%benchmark for measuring availability does not
%exist. The lack of such a benchmark continues to
%leave a gap in the evaluation process, and it is
%generally agreed throughout the industry that a
%method for benchmarking availability is needed.

%In this paper, we first describe System Recovery
%Benchmarks (SRBs), a generic framework for
%developing benchmarks that measure automated
%recovery, and the first implementation of an SRB,
%the SRB-A benchmark. T

Many server architectures degrade dramatically at high (near 100%) levels of usage — "fall off a cliff" — and benchmarks should (but often do not) take that factor into account. Vendors, in particular, tend to publish server benchmarks at continuous at about 80% usage — an unrealistic situation — and do not document what happens to the overall system when demand spikes beyond that level.


Many benchmarks focus on one application, or even one application tier, to the exclusion of other applications. Most data centers are now implementing virtualization extensively for a variety of reasons, and benchmarking is still catching up to that reality where multiple applications and application tiers are concurrently running on consolidated servers.

Relevance: Benchmarks should measure relatively vital features.
Representativeness: Benchmark performance metrics should be broadly accepted by industry and academia.
Equity: All systems should be fairly compared.
Repeatability: Benchmark results can be verified.
Cost-effectiveness: Benchmark tests are economical.
Scalability: Benchmark tests should work across systems possessing a range of resources from low to high.
Transparency: Benchmark metrics should be easy to understan

normally by running a number of standard tests and trials against it.
Benchmarks provide a method of comparing the performance of various subsystems across different chip/system architectures. 

This raises the question: What is the smallest experiment we can run that still gives us confidence in the result?



Our goal in this paper is to create a standard benchmark and benchmarking framework to assist in the comparative analysis of remediation mechanisms between self-healing key/value databases. We focus on the 

To show the practicality of our benchmark, we use it to study 

Using our benchmark, we can quantify the system's responsiveness in the presence of degraded resources, and the time it takes for a system to regain its nominal performance levels after catastrophic failures. 




%  Section  2  lists  a  few  of  the  metrics  commonly  associated  with availability. Section 3 details some of the factors pertinent to the  topic  such  as  typical  hardware  failures.  Section  4  briefly discusses different modeling techniques for testing. Section 5explains issues related to workloads in fault-injection testing.Section  6  covers  a  few  of  the  known  problems  that  present roadblocks  and  misrepresentation.  Lastly,  section  7  presents what other research is being done and section 8 concludes thepaper



























%Mangle enables you to run chaos engineering experiments seamlessly against applications and infrastructure components to assess resiliency and fault tolerance. It is designed to introduce faults with very little pre-configuration and can support any infrastructure that you might have including K8S, Docker, vCenter or any Remote Machine with ssh enabled. With its powerful plugin model, you can define a custom fault of your choice based on a template and run it without building your code from scratch








 For  this  reason,  werun  regular  exercises  on  a  weekly  basis  that  test  AvailabilityZone  outages,  split  brain  situations  (data  replication  gettingqueued  up)  or  regional  outage  simulations.  

o do so, the principle 
We also must be mindfu

You start by .

Then, you .

It can also be used to discover new, unknown failure modes. While these artificial failures are typically injected into production systems, they’re done so in a controlled, relatively safe way.

By designing and executing Chaos Engineering experiments, you will learn about weaknesses in your system that could potentially lead to outages that cause customer harm.

Chaos Engineering lets you validate what you think will happen with what is actually happening in your systems.

The advantage of chaos engineering is that you can quickly smoke out issues that other testing layers cannot easily capture. This can save you a lot of downtime in the future and help design and build fault tolerant systems




In contrast, understanding designs for availability, behavior during component faults, and the relationship between performance and availability of these servers have received much less attention. 
%defines a hierarchical approach to benchmarking system
availability, either as a whole, or as a subset based on the key aspects of availability defined therein. The
framework defines methods for representing each attribute as a standalone entity, such that Rate,
Robustness, or Recovery can be broken down for the purpose of further analysis and comparison

Benchmarks also provide researchers with a technique to measure progress andmake trade-off analyses among designs.

Measures of robustness may include the magnitude of deviation from the nominative performance levels, whereas measures of recovery may include time to return to nominative performance levels and completeness of the recovery in a finite amount of time.




In  order  for  a  benchmark  to  be  credible,  thebenchmark must accurately represent a system's behavior in real world environments, and the benchmarkresult must  be reproducible.

In this context, R-Cubed proposed an hierarchical approach to benchmarking system availability, with metrics that are well understood and accepted: 




The second difficulty is that different systems have different components, and therefore different, unique failure
modes. Thus, it is difficult to design 

as of today an  for measuring availability does not
exist

Although vendors can use production traces to model the failure rate of their infrastructure, these traces do not necessarily depict the way a different infrastructure may behave 

Ironically, R-Cubed was proposed in 2002. It is no coincidence that 20 years later a widely adopted availability benchmark has yet to be designed. This is mostly due to the complexity of modeling a failure pattern that is both accurate and infrastructure-independent. 




there are several differences: test duration, 

arise since our goal is to achieve short-running 

and despite its name, NDBench is a testing tool rather than benchmarking. 

However, 

between the two approaches. 


Yet, we are not aware of any studies that focused on benchmarking control operations in cloud nativestorage systems—this position paper’s focus

will enable engineers and researchers to effortlessly compare systems. Yet


this setup is fairly similar to  design in the sense that it provides a benchmarking layer (on the client side) and a failure injection layer (on the server side). 

YCSB  isfairly  similar  to  our  design  in  the  sense  that  it  provides  anabstraction layer for adapting client APIs to specific data storesand it is probably the closest tool to compare with NDBench.


We    NDBench  into  the  Netflix  Open  SourceSoftware (OSS) ecosystem by integrating it with componentssuch as Archaius for configuration management 

- API
- Model

-- Chaos

These models can be tailored 

.Traeger et al. [36] conducted an extensive study of file systemsand storage benchmarks. 

Benchmarks have been developed to facilitate developers from writing specific test applications to simulate a given workload. In on hand, framework-based benchmarks, like fio or stress-ng, are tunable engines that permit users to create customized workloads. Although these benchmarks useful for getting performance insights for a system, different systems have different components, and therefore different, unique testing requirements. On the other hand, Model-based benchmarks, like YCSB, have a predefined set of coarse-grained workloads used to compare systems in an apples-to-apples manner.




To quantify performance, most benchmarks are based on workload generating clients that hammer system's servers with requests. By measuring the difference between request submission and acknowledge received by the system, benchmarks report performance statistics for throughput, Queries per second (QPS) or tail-latency. 


The concept of chaos engineering originated at Netflix in 2011. They were migrating Microservices from data centers to less reliable cloud infrastructure and wanted to ensure that their systems could cope with this less stable environment. To test resiliency, Netflix created the Simian Army, which consists of a series of agents known as “monkeys” (AKA Chaos Monkey’s) that deliberately inject failure into their services and systems. Wrapping several Linux utilities to change the behaviour of production instances (e.g, TC, Stress-ng), Monkeys where able to terminate services, induce network delays,  burn up CPU, or take disks offline, etc. 



%However, in order to separate the impact of chaos testing from the noise of the system, making it verifiable by humans and machines, engineers ended up running larger and longer chaos experiments, risking unnecessary disruptions for their customers. To limit the blast radius, Netflix developed ChAP; a tool that takes a small subset of traffic and distribute it evenly between a control and an experimental cluster. This way, engineers identified mistuned retry policies, CPU-intensive fallbacks, and unexpected interactions between circuit breakers and load balancers.

With the adoption of Kubernetes, new Chaos injector paradigms emerged that supplant agents and can be deployed directly on clusters. Chaos Mesh and Pumba use Kubernetes API to simulate abnormal system conditions, including Pod failures, container failures, network failures, file system failures, system time failures, and kernel failures. 

However, Chaos Mesh lacks automation pipelines that make the testing scalable and efficient. In this respect, PingCAP extended Chaos Mesh to TiPocket, an automated testing to build a full Chaos Engineering testing loop for distributed databases. Powered by Argo workflow engine, TiPocket automates the chaos pipelines to:
\begin{enumerate*}
    \item Injects chaos
    \item Verifies the impact of that chaos using a variety of benchmarks
    \item Visualizes the results through metrics, logging, and tracing.
\end{enumerate*}


The ability to execute experiments that represent real life events in a controlled manner in production systems seems scary at a first glance but it can certainly increase the quality not only of the business applications but of the infrastructure systems as well.

Featuring extensible interface, it allows integration with other testing frameworks and can perform chaos experiments in production environments. 

Microsoft adopted a similar approach by creating their own monkey’s which were able to inject faults into their test environments.



Pumba does not really cover the concepts of tests or experiments, at least not as procedures that can succeed or fail based on how target applications respond. Instead, it works specifically as a chaos injector, wrapping several Linux utilities to change the behaviour of resources used by containers, such as network and CPU usage.





%DeathStarBench provides a set of interactive macro-benchmarks for microservice implementing social networks, media services, and e-commerce sites. Both NDBench and DeathStarBench target cloud applications and are not explicitly storage benchmarks




Arguably without establish failure patterns we cannot claim that obtained results from the benchmark represent realistic behavior.





Many opportunities to compare commercial products and claims, measure value of research ideas, ... with recovery benchmarks





This paper discusses a Java based testing environment that  facilitates  the  testing  of  distributed  applications  with  easy   publication,   monitoring   and   control   of   prototype   systems  on  a  peer-to-peer  test-bed.   Such  tests  may  require  the  creation    of    specialist    control    and    monitoring    tools.    Furthermore,   monitoring   code   must   often   be   inserted   throughout   such   prototype   systems.  



This work deals with general difficulties and aims when  especially when heterogeneous interfaces are used. As a solution RemoteTest is proposed, a framework for the test of distributed systems and their interfaces. This is done by integrating individual system components into a virtual environment that emulates the adjacent modules of the system. The interface details are thereby abstracted by the framework and there is no special interface knowledge necessary by the tester. In addition to the decoupling of components and interface abstraction, RemoteTest facilitates the testing of distributed systems with flexible mechanisms to write test scripts and an architecture that can be easily adapted to different systems.

A coordinated test method has subsequently been proposed to solve these two problems. In the present article: 1) we show that controllability and observability are indeed resolved if and only if the test system respects timing constraints, even when the system under test is non-real-time; 2) we determine these timing constraints; 3) we determine other timing constraints which optimize the duration of test execution; 4) we show that the communication medium used by the test system does not necessarily have to be FIFO; and 5) we show that the centralized test method can be considered just as a particular case of the proposed coordinated test method.







% Systems increasing in scale

% Manual methods can no longer server the puThe traditional methods can l



Therefore, a scalable MBT technique should be flexible regarding the size of the generated test suites and should be easily accommodated to fit resource and time constraints.


A   semi-centralised   peer-to-peer   network,   using   a   single index server is used as the communications substrate for  the  framework.  This  is  similar  to  Napster  [3].  Nodes  Proceedings of the Fourth International Conference on Peer-to-Peer Computing (P2P’04) 0-7695-2156-8/04 20.00 © 2004 IEEE
participating  in  the  test-bed  network  are  typically  standard  general-purpose  workstations.  Each  runs  a  small  client  application which allows it to host distributed applications.       The  client  registers  with  the  index  server  that  it  is available  to  host  a  test  process.    When  the  developer  publishes  a  process  to  the  test-bed,  they  are  informed  by  the server of the current number of nodes willing to host a new test. From this pool of nodes, the developer selects an appropriate  test  size,  and  ‘publishes’  the  modified  system  to the network. The modified software is sent to each test-host using a simple peer-to-peer HTTP file transfer. When the software transfer is complete, the hosts execute the test-software  and  the  inserted  monitoring  code  will  relay  the  status of each node on the network back to the server. The user  can  access  this  information  in  a  dynamic  graphical  form via an associated Java applet or as text logs.


Nevertheless,the  importance  of  high  dependability  in  a  software  system  hasrecently increased, and exhaustive testing of software systems isbecoming  expensive  and  time-consuming,  and,  in  many  cases,sufficient  software  testing  is  not  possible.  In  particular,  it  isoften difficult to test parallel and distributed systems in the realworld after deployment, although reliable systems, such as high-availability servers, are parallel and distributed systems.



This framework implements a test bed environment using a semi-centralized peer-to-peer network as a substrate for sharing resources made available from standard PCs. This framework automates the process of test-case deployment using a combination of reflection and aspect oriented programming. This allows 'point-and-click' publishing of software onto the test-bed. Our framework also provides a common monitoring, control and logging interface for all nodes running on the network. Together, these features greatly reduce deployment-time for real-world test scenarios. 











\textbf{loading data from external sources:}
    In \frisbee{}, the service configurations are kept separately from the service template. When a service template 
    
    
    As shown in Figure~\ref{fig:tree} 
    
    
    When you are creating a ConfigMap based on a directory, kubectl identifies files whose basename is a valid key in the directory and packages each of those files into the new ConfigMap. Any directory entries except regular files are ignored (e.g. subdirectories, symlinks, devices, pipes, etc).
    

    Kubernetes is based on a rather opinionated configuration model. It assumes a single YAML that represent the entire state of the execution environment. Apart from service declarations, this file also includes ConfigMaps and Secrets that hold configuration or sensitive data that are used by other Kubernetes objects, such as Pods. Although this approach favors portability, it usually results into large configurations that are difficult to understand and maintain.
    
     For example, the Grafana service is defined in `monitoring/grafana/granafa.yml' whereas the configuration exists in `monitoring
    
    
    the Grafana configurations (including


ConfigMaps and Secrets hold configuration or sensitive data that are used by other Kubernetes objects, such as Pods. The source of truth of ConfigMaps or Secrets are usually external to a cluster, such as a configuration directory (e.g, /etc/grafana) or an SSH keyfile.

Adhering to separation of concerns, \frisbee{} allows to create a ConfigMap from multiple files in the same directory. When declaring a serv



Kustomize has secretGenerator and configMapGenerator, which generate Secret and ConfigMap from files or literals.



 For example, the declaration of a Grafana service would take 6 lines, whereas the configuration of Grafana would take a few thousand lines (e.g, including dashboards, datasources)





\textbf{setting cross-cutting fields for resources:}

It is quite common to set cross-cutting fields for all Kubernetes resources in a project. Some use cases for setting cross-cutting fields:

    setting the same namespace for all Resources
    adding the same name prefix or suffix
    adding the same set of labels
    adding the same set of annotations
    
Create a     
    

\textbf{composing and customizing collections of resources:}






Users still develop their application using familiar Kubernetes constructs with the added functionality of \frisbee{} not affecting portability. This means that a \frisbee{} enhanced description will run in any Kubernetes runtime environment without any alterations, however users will lose the functionality offered by \frisbee{}.




Fogify extends the docker-compose specificationso  that  it  encapsulates  a  wide  variety  of  Fog  infrastructureproperties such as computing resources, network capabilities,QoS  constraints,  and  placement  policies.  Users  still  developtheir  application  using  familiar  docker  constructs  with  theadded  functionality  of  Fogify  not  affecting  portability.  Thismeans  that  a  Fogify  enhanced  description  will  run  in  anydocker runtime environment without any alterations, howeverusers will lose the functionality offered by Fogify





\textbf{load data from external sources:}


separates the declaration of a server from the service configuration.

You can use kubectl create configmap 

For example,  that would normally take 6 lines, it may result into thousands of lines if we consider that dashboard definitions must be all included in a single file.

or sensitive data that are used by other Kubernetes objects, such as Pods.

all the configurations files for all the services. 

desired resources and 



that include dashboard definitions, datasource definition, and so on. 

with tons of  parameters. 

if we consider the dashboard definitions.

 In other words, 




For example, 

configuration files that hold configuration for the dashboards. 

include a lot of boilerplate parameters. 

Instead, \frisbee{} templates are designed with reusability in mind. 



 The source of truth of ConfigMaps or Secrets are usually external to a cluster, such as a configuration file or an SSH keyfile. 


For example, the definition of two services may result into thousands of lines as it should also include the configuration files for those services. 


 In addition, it forfeits reusability of defined resources. 


the same file will contain the service definitions, the configuration files for all the services, 




state of the cluster, in results  


When you use the 

contains all the necessary information for the runtime environment. Although this model is grounded on a "single source of truth", 



    
    
    The extension helps scaffold needed files, build 
    
    
     These resources may be 
  
  For example, the `template: [monitoring/redis]'
  
  The reasoning for deprecating this behavior is that a template is a "definition": it defines inputs and things to be done once instantiated. With this deprecated behavior, the same template object is allowed to be an "instantiator": to pass in "live" arguments and reference other templates (those other templates may be "definitions" or "instantiators").
  
  
  
\susubsection{Configurations}


\susubsection{Monitoring}


The template has the following features to simplify the use of off-the-shelf testing configurations.



Kustomize is a tool for customizing Kubernetes configurations. It has the following features to manage application configuration files:

    generating resources from other sources
    setting cross-cutting fields for resources
    composing and customizing collections of resources
    
    


















\newpage
\newpage




a global tester that has total control over the distributed system under test (SUT)


Grafana supports annotation of "request_start", "request_done", "failure"

Resource Constraints

Memory and CPU and natively supported by Kubernetes
Network & IOPS are implemented using Chaos-mesh


\subsection{Test Description}
        
        
        
        % Root-cause analysis (Workflow manifest -> Controller events -> Visualization)
        
        

    
        % Auto-generate testing scenarios
        Based on this codification, static analysis tool will be able to detect architectural issues automatically and recommend changes according to policies published in the \textit{hub}. 




\subsection{Testing Controller}
     
We currently support two \microflow{}s: Disjoint and Evolutionary. In \textit{Disjoint}, each phase is autonomous, with the containers starting together, perform a task, and then terminate before the next phase begins. As an example, a \textit{Disjoint} \microflow{} can be used for automating the execution of numerous short-living distributed tests. In \textit{Evolutionary} each phase is an incremental change to the state of a single long-running test. 

    full control over the course of testing, from a single configuration file
    
    In particular, our Testbed, calOpenIoT will research and p comprising IoT resources, which can deliver on-demand utility IoT services such as sensing as a service.


\subsection{Virtual Resources}



\subsection{Testing loop}

\subsection{Fault Injection}
    To support systematic fault injection, we use Chaos-Mesh, a fault-injection and network emulation infrastructure explicitly designed to study cluster-based servers. While evaluators using our methodology are free to use any fault-injection framework, Mendosus provides significant flexibility in emulating different LAN configurations and can inject a wide variety of faults, including link, switch, disk, node, and process faults. 
 

    While arbitrary fault injection seems appropriate for testing a system's robustness, there are two tricky issues when injecting faults for benchmarking purposes.

    The first issue is about duration. By performing the smallest measurable experiments, system operators can verify that specific failure scenarios are handled correctly – a network partition between database servers, for example. However, the fault must last long enough to allow all the desired properties to be observed and measured. The duration should be small enough to exclude irrelevant events, and large enough to amortize transient warm-up effects and deliver throughput that is relatively stable throughout the observation period. 

    The second issue is about injection time. Most systems today depend on asynchronous tasks, such as garbage collection, bitrot scrubbing, or replication, whose invocation time is difficult to predict. Given this uncertainty, the time of fault injection should be associated and driven by, an explicit state of the component under evaluation~\cite{koopman_whats_2002}. This is a critical property for achieving comparable conditions amongst iterations of load a test, and amongst two architecturally different systems. The challenge here is to determine how well internal states of a system can be inferred from knowledge of its external outputs (e.g, logs or monitoring tools). 





\subsection{Distributed Monitoring}
    One of the main concerns in monitoring distributed systems, is the ability to correlate observed behaviors with root events, and stitch them together in wonderful, insightful ways. The key for an effective correlation is following certain standards for collecting, managing, and processing metrics from the distributed nodes, network connections, and application-level information. 
    
    The end-to-end traceability of data flows through n-tier systems is a challenging task which becomes more important when systems increase in complexity. The Application Response Measurement defines concepts and APIs for measuring performance and correlating transactions between tiers.
    
    %; join, filter, aggregate, etc.  Such standardizations should belong to a global governance, to enable interoperability between polyglot domain datasets. Common concerns of such standardization efforts are field type formatting, identifying polysemes across different domains, datasets address conventions, common metadata fields, event formats such as CloudEvents, etc

    % . Yet, it should transparently integrate a mix of emulated devices into the existing management systems, in a scalable and automated manner;
    


\subsubsection{Contextualized Visualization}

    Using this model, operators can analyze the responsiveness of different design decisions against emerging failures and runtime conditions~\cite{10.5555/1251460.1251462}. 

    To provide contextualized information about the entire state of the system, \frisbee{} enriches container metrics with events triggered by the controller. A nice way to do that in Grafana is to use annotations. Annotations are descriptions of points in time that can be added to dashboards. They show as vertical lines in the panels and, when hovering over them, reveal a descriptive text and optionally a set of tags.
    







\subsection{Controller}
    It is very common to define manifests in form of . yaml files and send them to the Kubernetes API Server via commands such as kubectl apply -f my-file.
    
    
    

    %[1] The IT infrastructure managed by this process comprises both physical equipment, such as bare-metal servers, as well as virtual machines, and associated configuration resources. The definitions may be in a version control system. It can use either scripts or declarative definitions, rather than manual processes, but the term is more often used to promote declarative approaches. 
    
    


\subsection{Workflow Dependencies}
    
Many systems operate through distinct phases; setup, steady-state, and (optionally) shutdown. These phases have different performance characteristics. Setup may start with clean caches and store everything in memory. Steady-state may balance memory and I/O usage proportional to connected clients or request rate. Shutdown may perform I/O to persist data on the disk. The I/O can be proportional to the amount of processed data throughout the steady-state. For a fair comparison between systems, we need to ensure that evaluated systems have reached a steady-state before starting the \faultload{}.


    [ YCSB example ]

    Luckily, Cloud benchmarks like YCSB are also divided into two phases: load and transaction. Therefore, \faultload{}s remain pending, waiting for the clients to complete the load phase and start the transaction phase. However, this requires coordination among the distributed clients~\cite{10.1145/2038916.2038925}. 

    The event watcher has two parameters to control distributed coordination: a barrier-sync variable and the client coordination group's size for the phase. The barrier-sync is a structure used to track the number of clients entering or leaving a phase. The watcher uses a hierarchical namespace for synchronization and, for each client, it creates a corresponding directory in its namespace. Clients join a phase by contacting the watcher at the \texttt{/:phase/join/:clientID} and then wait for \texttt{/:phase/ready} to become True; if not, the client blocks and retries after a timeout. In parallel, the watcher creates a new entry with the client's identifier in the phase directory; phase barriers and the respective directories are created on the fly. If the total number of entries equals the group size, meaning all clients have joined the phase, the watcher changes the returned value of \texttt{/:phase/ready} to True. If not, it returns False, waiting for more clients to join. After clients have completed their tasks, they notify watcher about exiting the by calling \texttt{/:phase/done/:clientID}, and then join the next phase \texttt{/:next\_phase/join/:clientID}.












% Terminology. In this paper we define architecture erosion as the phenomenon that occurs when the implemented architecture of a software system diverges from its intended architecture. The implemented architecture is the model that has been realised or built-in within low-level design constructs and the source code.
% Architecture design documentation: ► Records architecture design and rationale with the intent of disseminating architectural knowledge to a wider audience and provides a point of reference for developers throughout system evolution
%Architecture analysis: ► Uncovers weaknesses in the intended architecture, in particular, sensitive points which can be easily violated in the implementation
% Architecture compliance monitoring: ► Establishes the means to validate whether the implementation is faithful to the intended architecture during both the development and subsequent maintenance phases of a system



\subsection{Testing Controller}
    \begin{itemize}
        \item Translates Experiment events into actions on the backend 
        \item Naming issues (fixed namespaces, service resolution)
        \item Backend actions are asynchronous (e.g, container creation of deletion)
        \item Respect time (from experiment description to runtime implementation)
        \item Repeatable experiments (e.g, confidence intervals)
    \end{itemize}
    
The \textbf{Endpoint} have the explicit control over both the request and completion path of I/O to backend services. Using a declarative management style API it allows for easy optimization of synchronous and asynchronous I/O, over a wide range of storage backend (e.g., filesystems, key/value databases, object-store, data pipelines, message queues). For example, an \textit{Endpoint} can improve bandwidth and resource utilization by buffering small files in the local memory, and collectively flush them in a single I/O operation. Similarly, it can act as a proximate cache for data that are normally stored on distant Clouds. 


\subsection{Syntax}
-- Each Wait command may accept an expected status. (e.g, Running, Failed, Terminated)
-- If the status is different, the experiment is aborted

Add Node
Remove Node
Wait (for nodes)
Sleep(...)






%n Kubernetes, a user creates Pods (one of Kuber-netes’ core resources) by specifying the Pod’s configuration ina YAML file and passing that file to thekubectlcommandline utility.  Similarly, we wantCNSBenchusers to launchnew instances by specifyingCNSBench’s configuration in aYAML file and passing that file tokubectl. To achieve that,ourCNSBenchimplementation follows theoperator designpattern, which is a standard mechanism for introducing newfunctionality into a Kubernetes cluster [31]. In this pattern, adeveloper defines anOperatorthat comprises a custom resourceand a controller for that resource. For our implementation ofCNSBench, we defined a customBenchmarkresource andimplemented a correspondingBenchmark Controller. Together,these two components form theCNSBenchOperator.  TheBenchmark resource specifies the I/O and control workloads,which the controller is then responsible for running




This provide the ability to combine templates into complex hierarchies that can be connected or combined as building blocks to create a fully virtualized platform. 

that maintain `just enough' properties to describe the application at hand.

A template needs to be carefully prepared to demand specific information in key places, since  are restricted to changing only those elements the template makes available. The template skeleton defines 


(e.g., application-specific monitoring) for the application at hand, and to dynamically alter that structure as conditions warrant, 
    
    \frisbee{} brings all the distributed intelligence of the running containers under the control of the users, by separating the control plane of the testbed from the testing runtime. The testing runtime 
    
    
    
    
    At its core, a container is an operating system virtualizationapproach that enables multiple isolated process groups to sharethe same kernel. The kernel exposes a mechanism to isolateboth the environment (namespaces) and the performance, i.e.,limit  access  to  resources  (cgroups).  Of  particular  interest  inthe context of workflows is the isolation of the environmentas  a  container  image.  While  the  kernel  does  not  providedirect support in this regard—it assumes the environment isavailable  as  a  mount  point—tools  such  as  Docker  can  beused to automatically build and share container images as aset of deterministic\ scripts that can import and modify othercontainer images in a layered fashion. Such an approach cangreatly  increase  the  portability  and  reusability  of  containerimages, which was the main reason for their wide adoption
    
    
    
    
    
    
    
    
    
    
    
\subsection{Services}

\textbf{Manifest}

\textbf{Controller}
\begin{itemize}
    \item Naming issues (e.g, fixednamespaces, service resolution)
\end{itemize}







\textbf{Platform}
\begin{itemize}
    \item Create services that are combinations of pods, containers, Ingress, services
\end{itemize}



\subsection{Virtual Resources}

\textbf{Manifest}

\textbf{Controller}

\textbf{Platform}
\begin{itemize}
    \item Kubernetes
    \item Chaos-mesh
\end{itemize}


\subsection{Tiers \& Placement}
% Why we need it 

\textbf{Manifest}

\textbf{Controller}

\textbf{Platform}


\subsection{Faultloads}
%Fault tolerance and high-availability

\textbf{Manifest}
\begin{itemize}
    \item Types of faultloads
\end{itemize}

\textbf{Controller}
\begin{itemize}
    \item Translate types into specific faults
\end{itemize}

\textbf{Platform}
\begin{itemize}
    \item Chaos-Mesh: inject failures
\end{itemize}


\subsection{Events}

\textbf{Manifest}
%Kubernetes: spin-up or remove instances

\textbf{Controller}
\begin{itemize}
    \item Translates events into action on the platform
    \item Backend actions are asynchronous (e.g, container creation or deletion)
    \item Respect time (from experiment description to runtime implementation)
\end{itemize}

\textbf{Platform}

\subsection{Dependent Execution}
\textbf{Manifest}
\begin{itemize}
    \item Wait
\end{itemize}

\textbf{Controller}
\begin{itemize}
    \item Distributed coordination
\end{itemize}

\textbf{Platform}
\begin{itemize}
    \item Notification events
\end{itemize}

\subsection{Cluster Visualization}

\textbf{Manifest}

\textbf{Controller}
\begin{itemize}
    \item Grafana dashboards
    \item Assign metrics agents into service
\end{itemize}

\textbf{Platform}
\begin{itemize}
    \item Deploy Metric agents as sidecars
\end{itemize}


\subsection{Context Execution}
\textbf{Manifest}

\textbf{Controller}
\begin{itemize}
    \item Dynamic Pause the runtime for debugging purposes
\end{itemize}

\textbf{Platform}
\begin{itemize}
    \item ctrl+z to pause 
\end{itemize}

\subsection{Confidence in Results}
\textbf{Manifest}
\begin{itemize}
    \item Declare acceptable error margin
\end{itemize}


\textbf{Controller}
\begin{itemize}
    \item Keep Prometheus + grafana, and reset environment
    \item Rerun experiments until error is below the given threshold
\end{itemize}

\textbf{Platform}
\begin{itemize}
    \item How to reset it
\end{itemize}


A key design goal of \frisbee{} is to be application agnostic. However, most existing benchmarks do not expose their metrics directly to Prometheus, and it is also possible for their output formats to variate significantly. To address these challenges, clients run a Telegraf agent that converts the client's output into Prometheus metrics and exposes those metrics in HTTP endpoints which Prometheus scrapes asynchronously.  Similarly, Telegraf agents running on the Kubernetes host node provide insights into the system's traffic, I/O patterns, and resource utilization. This information can be later used for comparing scalability factors (e.g. hotspots) and cost factors (e.g. I/O amplification). 



After passing the YAML file to the \frisbee{} command-line utility, the \frisbee{} controller performs the necessary actions to maintain the runtime's present state in sync with the desired state. More specifically, the Deployment Manager launches the containerized instances in an isolated testing environment and employs distributed coordination to ensure that the system has reached a steady-state.  Once the system is stable, the \faultload{} executor takes over and drives failure injection into the running services, as prescribed by the given \faultload{}. Both the deployment manager and \faultload{} executor perform their tasks by making calls to the infrastructure abstraction layer.


As shown in Figure~\ref{fig:architecture}, we decouple the \frisbee{} runtime from the \frisbee{} controller. We classify these containers into system services, dependent services, and clients. The system services are server instances whose recovery mechanisms we want to investigate (e.g., key/value stores). Dependent services provide essential functions required by system services (e.g. Zookeeper for distributed coordination). The clients are performance benchmarks that continuously hammer system services with requests (e.g. YCSB). 

The infrastructure interface layer is responsible for the creation, update, and termination of the containers. We presently use a Kubernetes-based driver for managing the containers. For operators that wish to run the benchmark in a more complex environment, including Kubernetes, Docker, vCenter, or any remote machine with ssh enabled, \frisbee{}'s powerful plugin model allows them to define their custom driver and run the benchmark without building code from scratch. 




The end-to-end traceability of data flows through n-tier systems is a challenging task which becomes more important when systems increase in complexity. The Application Response Measurement defines concepts and APIs for measuring performance and correlating transactions between tiers.  A three-tier architecture then will have three processing nodes. 




A scenario with distributed control can be centralized by exposing the requested behavior in an external interface of the tested application. In contrast, decentralization of a centralized test is more difficult. 
	
	

While the clients run benchmarks against system services, both in the absence and presence of faults, the watcher interacts directly with the distributed clients and collects metrics through well-defined HTTP endpoints. We currently collect Queries per Second (QPS) and tail latency. Moreover, the watcher enriches the collected metrics with events from the deployment management and the \faultload{} executor. This way, when operators use \frisbee{} for analyzing their systems, they will not have a simple visualization of the experiment's progress but an annotated representation of what exactly was happening at every different step. 

Additionally, the watcher performs statistical analysis on the client metrics to decide if the collected metrics have converged on a stable value. If not, it notifies the deployment manager to restore the testing environment and asks the executor to rerun the \faultload{}. This feedback loop continues until the metrics have converged or the number of retries has exceeded a maximum threshold.  At the end of the experiment, the aggregated reports from all iterations are available via the watcher dashboard.




\subsection{Architecture Overview}
    


%infrastructure and application emulation beforeundertaking   the   deployment   and   testing   on   real   testbeds.Emulation is a process that realizes the behavior of a platform,device or infrastructure on a host device or host infrastructure,at  a  fraction  of  the  real  deployment  cost.


\subsection{Hub}
    Adhering to the Open Science principle, we will create a systems development hub where community members, like researchers and engineers, will be able to share \textit{Atoms}, platform configurations, collections of policies, benchmarks, and best practices. Doing so makes it possible to reconstitute a platform configuration `anywhere, anytime'. A criterion that often undermines the success of a framework is its learning curve. In this view, we will create a database that associates configurations with application performance metrics. 



Services have Create, Remove, Wait, Stop, Kill, DependOn.
FAILURE have Create that takes a duration. After that, they are retracted automatically



    SDK for Go language offers a library for interacting with Grafana server from Go applications. It realizes many of HTTP REST API calls for administration, client, organizations. Beside of them it allows creating of Grafana objects (dashboards, panels, datasources) locally and manipulating them for constructing dashboards programmatically. It would be helpful for massive operations on a large set of Grafana objects.
    
    Library design principles

    SDK offers client functionality so it covers Grafana REST API with its requests and responses as close as possible.
    SDK maps Grafana objects (dashboard, row, panel, datasource) to similar Go structures but not follows exactly all Grafana abstractions.
    It doesn't use any logger, instead API functions could return errors where it need.
    Prefere no external deps except Go stdlib.
    Cover SDK calls with unit tests.
    
    


// watch will retry querying the state of the object until the condition is true.
	// For phase documentation check https://kubernetes.io/docs/concepts/workloads/pods/pod-lifecycle/#pod-phase
	


















Other than being a burdensome, labor-intensive, and error-prone task, this manual methods also forfeit experiments that are scalable, portable, and repeatable. 

Today's systems run so many distributed and asynchronous tasks that it is almost impossible to achieve identical conditions across different runs. 



Contrarily, Chaos Engineering toolkits~\cite{basiri2016chaos, chaomesh} that provide fault injection (e.g. randomly triggering faults) focus on functional testing (i.e. can the system recover ?) rather than the performance and recovery characteristics of the evaluated system.



Unfortunately, the design space can be so extensive that it is impractical to measure each fault's repercussions. 











%In this view, Frisbee is a controller that enriches Kubernetes with the missing features. 



%Until recently, data services were running on physical machines with statically assigned resources and sharing the network with a broad range of services such as Web search, e-commerce, storage backup, or video streaming. 



ensuring that a system meets its prescribed specification is a growing challenge confronting software developers. 


characterize scaling techniques (e.g. reactive vs. preventive), identify suboptimal (i.e. less effective) approaches, and compare the recoverability of different systems in the presence of failures.



%The result of these factors is that the workloads running in atypical shared cluster (and on each of its individual hosts) have ahighly diverse set of characteristics in 



With the scale and complexity of distributed systems rapidly increasing, testing becomes a 


Other than being a burdensome, labor-intensive, and error-prone task, this manual methods also forfeit experiments that are scalable, portable, and repeatable. 

-- all of which are 

 Time-based solutions are error-prone if the time is not large enough, and time-wasting if the time is large enough. Yet, both approaches forfeit experiments that are scalable, portable, and repeatable. 
 
 
 
 
 
 
 
 %> Cassandra doesn't do that automatically - it can guarantee consistency on
> read or write via ConsistencyLevel on each query, and it can run active
> (AntiEntropy) repairs. But active repairs must be scheduled (by human or
> cron or by third party script like http://cassandra-reaper.io/), and to
> be pedantic, repair only fixes consistency issue, there's some work to be
> done to properly address/support fixing corrupted replicas (for example,
> repair COULD send a bit flip from one node to all of the others)

he next time the test was run, theywould already know  what to do. They referred  to this as thelearning curve. Tasks and problems the operators would faceare initial configuration, reconfiguration, monitoring, diagnosisand repair, an preventative maintenance.








multi-tier structure that is quite accessible and powerful enough for creating distributed parallel applications with a minimal learning curve and debugging effort,



This  framework  automates  the  process of test-case deployment using a combination of Reflection and  Aspect  Oriented  Programming.  This  allows  ‘point-and-click’  publishing  of  software  onto  the  test-bed.  Our  framework  also  provides a common monitoring, control and logging interface for all nodes running on the network.  Automated  insertion  and  removal  of  test  code  also  ensures  that  the  testing  process does not compromise the correctness of the final system



Together, these features greatly reduce  deployment-time  for  real-world  test  scenarios.  Automated  insertion  and  removal  of  test  code  also  ensures  that  the  testing  process does not compromise the correctness of the final system

This  framework  automates   Reflection and  Aspect  Oriented  Programming.This  allows  ‘point-and-click’  publishing  of  software  onto  the  test-bed. 

approach for testing distributed systems, by creating an automated testbed that 



testbed environment based on Kubernetes. 

This system provides a new approach for tackling the problems related to distributed computing 
coupled with inherent safety and modularity allowing for further expansion of features.

In this paper, we propose a software testing environment, called Frisbee, using Kubernetes enriched with workflows, monitoring, with fault injection facilities.

This    framework    implements a test bed environment using a semi-centralized peer-to-peer   network   as   a   substrate   for   sharing   resources   made   available  from  standard  PCs.  


Distributed Computing is considered to be one of the challenging problems in computer science. The entry barriers are quite significant due to the inherent complexity which such systems have to provide. 












contains the initialization parameters for \frisbee{} objects (i.e, groups, tiers, and services), as well as the scheduling of Actions and Failures that will happen to these objects. 


failures that will happen to services (e.g. kill, partition, corruption), failure patterns (e.g. run a partition failure every 10 minutes), and callback functions that will be triggered upon certain events (e.g. push annotation to Grafana when a node has crashed).


\textbf{Failure Action}
Control Actions specify the flow of control. They analyze the current state and schedule the next Action based on given parameters.

\textbf{Control Actions}
Control actions defines what Action the controller will run next.


\textbf{Events}
Events are created to follow the status of an object, report changes, and allow a reaction to the changes.

The events are therefore "connected" in a flexible and customer-specific way to application events, without having to modify the standard part of the application.

These events can be used as triggering events for your own tasks or workflows. 

 

Group dependencies are syntactic sugar to Wait Actions that we will discuss in the Workflow. 


Scientific  workflow  systems  manage  the  composition  ofworkflow  tasks  along  with  their  data  dependencies.  Thesedependencies instruct the workflow system how the commu-nication between tasks should be done. 


\textbf{DAG}

    Kubernetes YAML files are a great way to define multiple containers and services that work together as a stack. But, it can be easy to end up with repeated blocks in stacks with lots of similar services or configurations. 


 The templates called from a DAG or steps template can themselves be DAG or steps templates. This can allow for complex workflows to be split into manageable pieces.
 
 
	






the workflow as a directed-acyclic graph (DAG) by specifying the dependencies of each task. 


As an alternative to specifying sequences of steps, you can define 





%The framework 

Templates only describe the provisioning of services and resources, lacking  information about the number of instances, their location, and their inter-dependencies.  


sequences of steps, you can define the workflow as a directed-acyclic graph (DAG) by specifying the dependencies of each task. 




The transition from one phase to another should be guarded since the YCSB loaders must block until all Redis servers are ready, and the YCSB runners must block until all YCSB loaders have finished. 


Supports (or aims to support) a variety of testing workflows bulb

    (full_moon = fully supported // new_moon = planned)

    Experimental/iterative development waning_gibbous_moon
    Debugging last_quarter_moon
    Comparative testing waning_gibbous_moon
    Backwards/forward-compatibility testing waning_gibbous_moon
    Interoperability testing new_moon
    Continuous integration new_moon
    Stakeholder/acceptance testing new_moon


    
        For example, operators can specify events for controlling the rate at which clients will join or leave the testbed, launch new servers , or schedule failure events that disrupt vital services. 
        
        
        
        
        
        
        
        
        
        
        
        The controller  polls the dependent containers

can be simpler to



 When designing , this is a good design pattern: always wait for any dependent services  to come up before running your main code.


in this example the main container polls the Nginx container until it is ready to service requests.




maintain for complex workflows . The controller blocks the execution of dependent actions until the dependencies are met. 
        
        
        
        
%Section~\ref{sec:faultload} introduces our proposed failure classification model,  Section~\ref{sec:conclusions} concludes the paper and briefly presents future goals. 

% [ ] In impact say about contextualized visualization

%factors outside the scope of conformance testing and OSI, e.g., performance requirements, may impact the behaviour of real systems which is not foreseen by the specification. 


%In the following subsections, approaches to testing interoperability, performance and quality-of-service are discussed. 

%Interoperability Testing Interoperability testing evaluates the degree of interoperability of implementations with one another. It involves testing both, the capabilities and the behaviour of an im-plementation in an interconnected environment and checking whether an implemen-tation can communicate with another implementation of the same or of a different type. Interoperability testing is not standardized. However, a couple of interoperabil-ity testing proposals and guidelines exist (Buehler, 1994), (Myungchul et aI, 1996), (EWOS ETG 028, 1993), (Hopkinson, 1996), (Gadre et aI, 1990) (Hogrefe, 1990). 
%157 

%The two main approaches to interoperability testing in the context of OSI are pas-sive and active testing (Gadre et al, 1990) (Hogrefe, 1990). The difference is that ac-tive testing allows controlled error generation and a more detailed observation of the communication, whereas passive testing on the other side involves testing valid be-haviour only. 


%The difference is that ac-tive testing allows controlled error generation and a more detailed observation of the communication, whereas passive testing on the other side involves testing valid be-haviour only. 

%If the third-party service is unavailable, you can virtualize the service, and remove the dependency on the actual service. If the service is down, you can still test by using the virtualized service. A customizable service virtualization tool will let you configure the expected responses from the service, so that you can test your application’s response to various situations.

 

% But IoT devices are often passive, so testers must understand what devices are being used, and know how they behave. 

%This means that the way of testing software must adapt to the requirements of  architectural paradigms

 
 
 
 %In the second phase, active testing uses the reports from these predictive analyses to explicitly control the underlying scheduler of the concurrent program to accurately and quickly discover real concurrency bugs, if any, with very high probability and little overhead.


 
%    Hence, users have centralized control (by editing the \textit{Manifest}) over the decentralized platform (the \textit{Proxies} remain autonomous and distributed). 


%Based on this codification, static analysis tool will be able to detect architectural issues automatically and recommend changes according to policies published in the \textit{hub}. 


%maximizes productivity by enabling


%repeatable, measurable and controllable experimenting environments, 

%It also provides an automated engine 


%This architectural style results in configurations that are easier to understand, develop, test, and more resilient to architecture erosion. It also facilitates troubleshooting. It is easier to detect, reason and fix bugs when changes are systematically mastered (or edited) in the \textit{Manifest}, rather than investigating the code of each component of the system to find the anomaly. Based on this codification, static analysis tool will be able to detect architectural issues automatically and recommend changes according to policies published in the \textit{hub}. 





%(i)decrease in the cost of testing by reduced demand for hardware;(ii)(iii) ability to test applications under conditions which mimic their respective production environments;

%To  the  best  of  our  knowledge,  there  is  noestablished  and  standardized  way  to  automate  this  process,which is cumbersome and shifts resources from service devel-opment to infrastructure configuration


%O Building platforms for automated testing is a well understood and solved problem in industry. Unfortunately, the tooling and techniques are usually tightly coupled to the business model, and therefore we cannot transplant them directly for generic usage.





%1.Autonomy:    Agents    automatically    monitor    a    distributed system during its runtime. 2.Intelligence:  Agents  reveal  most  of  defects  that  might  occur  by  performing  the  different  testing  techniques.  As  a  result,  they  generate  fresh  test  cases  that  enhance  the  performance  of  testing  execution. 3.Flexibility:    Agents    perform    different    testing    approaches  depending  on  the  changes  and  the  development of distributed systems. 4.Cooperation: Agents   communicate   with   each   other in the proposed framework and consult with the  testers  to  ensure  the  valid  execution  of  the  different testing techniques. 5.Reactivity:  Agents  reclaim  any  found  error  when  misbehavior of a distributed system occurs. 

%In the second phase, active testing uses the reports from these predictive analyses to explicitly control the underlying scheduler of the concurrent program to accurately and quickly discover real concurrency bugs, if any, with very high probability and little overhead





Analyzing the passive behavior of a system is essential 




We believe that this definition style results in deployments that are easier to understand, develop, test, and more resilient to architecture erosion. It also facilitates troubleshooting. It is easier to detect, reason and fix bugs when changes are systematically mastered (or edited) in a human-readable file, rather than investigating each component of the system to find the anomalies.



\frisbee{} topologies define the initialization parameters for Services, the logical and physical classes into which the Services can be grouped into, and the relationships between the classes



Reasoning about the system's performance in dynamically evolving environments is challenging in its own right. While existing benchmarks, such as YCSB~\cite{cooper2010benchmarking}, can help assess the performance of clients, they do not provide insights into system network traffic, I/O patterns, and resource utilization. This information is necessary for comparing system scalability (e.g., avoidance of hotspots), system continuity in the presence of failures~\cite{10.5555/1009382.1009743} (e.g., failure detection time and failover overhead), and the total cost of ownership (e.g., accounting for high memory requirements or increased I/O amplification). Additional challenges arise because distributed systems produce so many operation metrics that operators can easily overlook anomalies and reported errors. 


With this in mind, experiments are designed around fixed workloads that run over a known quantity of relatively homogeneous resources. System testers know the server where the application resides, its CPUs, memory, and network bandwidth. They start with understanding how the infrastructure is expected to behave and instrument test points against those expectations. 









\subsection{Testing process}\label{subsec:process}
language that reduces the effort to create experiments by establishing a comprehensive approach to express complex environments, testing plans, and arbitrary operating conditions.





These policies are intented to address the lack of `reservation' policies 


the assigned resources so to cause disk IO saturation and throttling at the file operation (IOPS) level. 
The root-cause of this issue is . The trigger of the failures is IO overload of the worker node OS disks. This leads to the OS disk (from the perspective of the kernel) becoming unresponsive, blocked in IOWait. As everything on Linux is a file (including network sockets) - CNI, Docker, and other services that network I/O will also fail as they are unable to read off of the disk.


he first, and most commonly adopted, is to facilitate informed placement.







There are two types of resource assignments: `limits' and `reservations'. If a reservation is set, Kubernetes reserves at least the request amount of that system resource specifically for that container to use.

By default, Kubernetes supports both types of assignments for CPU and Memory. It lacks capabilities for throttling Storage and Network devices. In \frisbee{}, we support throttling for CPU,Memory, Storage, and Network devices. The trait, however, is that due to the diversity and the `peripheral' nature of Storage and Network,  we can only guarantee `limitation' assignments.


 In the context of \name{}, we use `limits' to maximize the number of collocated IoT clients per host. Conversely, we use `reservations' to guarantee minimum requirements and minimize the interference between antagonizing containers on the same host. Next, we explain our approach to resource throttling and the respective validation methods. 
 
 
 
For each component Deployment, aspects of these services may be determined by properties in a DeploymentSpecification for a particular kind of ExecutionEnvironment.

\textbf{In Deployment}
Physical storage devices have limitations in terms of bandwidth and total number of file operations (IOPS) but this is usually constrained by the physical device itself. Cloud provisioned block and file storage devices also have limitations due to architecture or service limits (quotas).





 via the distribution of \textit{Instances} across the physical nodes and networks.


So, \frisbee{} provides primitives for users to control where to place Services, both in the Virtua


You can use topology spread constraints to control how Pods are spread across your cluster among 

For the implementation of realistic scenarios, we have found that we need to deploy groups of services that are partially isolated but still partially share an environment.


\frisbee{} allows to control how Services are spread across the cluster. That 



\textbf{Inter-Tier}
Inter-tier policies set placement constraints between different Tiers. Practically, this allows to create sub-clusters 


for resources in physical or virtual host, including properties for the Processor, Memory, 

\frisbee{} supports limits/quotas 



\textbf{Intra-Tier}



 Users may still develop their Services using familiar Kubernetes constructs with the added functionality of \frisbee{} not affecting portability. The means that a \frisbee{} enhanced description will run in any Kubernetes environment without any alternations; however, users will lose the convenience offered by \frisbee{}.



 \frisbee{} is built with portability in mind so that it can be easily adapted to different infrastructure capabilities, from a single workstation to numerous cluster nodes, as well as support software components developed in multiple languages. 
 
 
 Containers are a widely accepted standard, so there are already many pre-built images that can be deployed on Kubernetes. 








\subsubsection{State Dependencies}







\subsection{Distributed Monitoring}



\subsubsection{Interaction with Controller}







\subsubsection{Kubernetes Client}
* ConfigMaps
* Pods
* Services
* Ingress
* Faults

Kubernetes probes~\cite{probes}

These primitives may involve core functions of Kubernetes (such as Pods, Services, Ingress) or Custom Resource Definition (CRDs) that are extensions of the Kubernetes API. Through CRDs, we have seamless access to third-party applications, such as Chaos-Mesh for fault injection.

\subsubsection{Runtime Pods}


The sidecar pattern allows \frisbee{} users to determine the most suitable services for enriching the application at hand without changing the application or the application container.    


Agents 
    
    

The sidecar paradigm enables \frisbee{} to add monitoring capabilities to a Service without modifying the application, or the application container. 


achieve that, the Workflow performs the following steps: 
\begin{enumerate*}
    \item Identify states of each object
    \item Identify events and analyze the applicability of actions
    \item Construct dynamic model diagram, comprising of state transition diagrams
    \item Express each state in terms of object attributes
    \item Validate the state–transition diagrams drawn
\end{enumerate*}

%



Although resource throttling can mimic the performance profiles of various devices, it takes more advanced techniques to mimic the behavioral characteristics of real-world LAN, WAN, and Internet connections. 



Kubernetes is a Container orchestrator that abstracts away the concept of physical machines as a set of CPU and RAM resources that can be utilized, and makes all of them a single deployment target. Given a pool of machines and a declarative description (e.g, run 10 instances of my container image with 2 cpus and 3GB RAM each, and keep it running), Kubernetes will run them wherever it finds free CPU capacity, and restart them if they are unhealthy. 




Therefore, it is challenging to port these scripts for different user credentials or experimental platforms -- which can be very diverse, from processes running on a single physical machine to virtual machines rented on public clouds or machines from research systems such as PlanetLab. 
















Thus, users have an out-of-the-box solution for visualizing and querying the system's state in real-time. More important though, it the ability of Grafana to create alerts  





%Moreover, YAML anchors and aliases let users reference and use the same data multiple times within a single YAML document. %In contrast, we have found that Kubernetes templated Services can become cumbersome due to tight dependencies occurring when the hierarchy with more than one layer deep. 

%These co-located containers form a single cohesive unit of service—for example, one container serving data stored in a shared volume to the public, while a separate sidecar container refreshes or updates those files. The Pod wraps these containers, storage resources, and an ephemeral network identity together as a single unit.





\frisbee{} provides users the ability to define metrics that are not known beforehand, if that is useful for understanding the systems' behavior. The monitoring pipeline of \frisbee{} can seamlessly integrate custom metrics, as long as they are compatible with Prometheus format. 

One of the challenges 

treat agents and their respective dashboards as tightly coupled components that we handle as a package. 






These metrics may be captured by Telegraf's plugins, or by purpose-specific telemetry agents. For example, Cadvisor captures container-specific metrics, node-exporter captures host-specific metrics, mongo-exporter captures mongo metrics, and so on.  


 Any existing integration is included in the Grafana Agent, but must be installed for it to send metrics that can be viewed in Grafana Cloud.






\subsection{Referenced Objects}
The \textit{Service} is a high-level structure that hides the complexity of managing individual Kubernetes objects. For example, the configmap provides the configuration for the application, the Pod provides the runtime for the application, the discovery service gives Pods their internal IP addresses and a single DNS name, the ingress service makes the Pod accessible via the Internet, and so on. The purpose of a \frisbee{} \textit{Service} is to hide away the management of all the boilerplate configurations required for a deployment. 




\textit{Service} instances are owners of other objects. For example, a ReplicaSet is the owner of a set of Pods. The owned objects are called dependents of the owner object. Every dependent object has a metadata.ownerReferences field that points to the owning object.

The \textit{Service} abstraction it a high-level structure that 


Some Kubernetes objects 

Sometimes, Kubernetes sets the value of ownerReference automatically. For example, when you create a ReplicaSet, Kubernetes automatically sets the ownerReference field of each Pod in the ReplicaSet. In 1.8, Kubernetes automatically sets the value of ownerReference for objects created or adopted by ReplicationController, ReplicaSet, StatefulSet, DaemonSet, Deployment, Job and CronJob.

To create a \textit{Service}. 

The controller has two primary 


To achieve this, the Controller communicates via the Orchestrator Connector with the Kubernetes API. The connector translates the model specification to underlyling  orchestration primitives for the Cluster Orchestrator.  

When the Controller creates an 


Controller objects, such as Deployments and StatefulSets, contain a Pod template field. Pod templates contain a Pod specification which determines how each Pod should run, including which containers should be run within the Pods and which volumes the Pods should mount.

Controller objects use Pod templates to create Pods and to manage their "desired state" within your cluster. When a Pod template is changed, all future Pods reflect the new template, but all existing Pods do not.


Although the \textit{Service} description is something sim


Controller objects, such as Deployments and StatefulSets, contain a Pod template field. Pod templates contain a Pod specification which determines how each Pod should run, including which containers should be run within the Pods and which volumes the Pods should mount.

Controller objects use Pod templates to create Pods and to manage their "desired state" within your cluster. When a Pod template is changed, all future Pods reflect the new template, but all existing Pods do not.


There are two supporting concepts that provide backgrounds about how Kubernetes manages pods for applications:

    Garbage collection tidies up objects from your cluster after their owning resource has been removed.


Owners and dependents

Some Kubernetes objects are owners of other objects. For example, a ReplicaSet is the owner of a set of Pods. The owned objects are called dependents of the owner object. Every dependent object has a metadata.ownerReferences field that points to the owning object.

Sometimes, Kubernetes sets the value of ownerReference automatically. For example, when you create a ReplicaSet, Kubernetes automatically sets the ownerReference field of each Pod in the ReplicaSet. In 1.8, Kubernetes automatically sets the value of ownerReference for objects created or adopted by ReplicationController, ReplicaSet, StatefulSet, DaemonSet, Deployment, Job and CronJob.







understanding how the systems responds to external factors. For a realistic evaluation beyond the sweet-spot (most common usage pattern), 

the systems behavior beyond the sweet-spot. For the realistic evaluation of a distributed systems, we need to take into account external f

and how the responds

systematic disturbances  
On top of analyzing the  (sweet-spot), enables users to cause  while the system is running, in order to 



%\frisbee{} is available with an Open Source license at https://github.com/....

%Moreover, the analysis of a static system is essential during development and when trying to troubleshoot problems, but it provides few means of understanding systems whose behavior  or due to . 

 %experiments are non-reproducible due to the tight coupling of scripts with the underlying infrastructure. All
 
 %To deliver the best experience to end-users, they 
 
%While distributed algorithms are usually tested by simulation or verified formally, we can derive many additional insights from experimenting with a prototype implementation deployed on a realistic platform.

%The Achilles heel of such experimentation is the duplicated effort and skills required to create pipelines for . This problem 


%maximizes productivity by enabling a comprehensive , more clearly and concisely than scripting. It also integrates the necessary tooling to build, validate, deploy, and (re)configure the distributed services with minimal human intervention.



The other point is that once we know the correct answer, we can then agree to do the wrong thing because of time-to-market reasons. And that is an explicit tradeoff and not a consequence of never even considering the correct answer. And the ability to choose to do the wrong thing allowed flexibility and enabled the right long-term thing to be done. Without that ability, I have seen standoffs between engineering management, product management, and architects.


simulation of an IoT environment. Regarding the simulation, we focus on identifying the effectiveness of running a distributed database at both Edge and Cloud nodes, and if it is better to make replicas on other Edge nodes or to the Cloud.




If an application goes above the limit, it gets throttled (aka fewer CPU cycles). On the other hand, memory requests and limits are implemented differently, and it's easier to detect. You only need to check if your pod's last restart status is OOMKilled. But CPU throttling is not easy to identify, because k8s only exposes usage metrics and not cgroup related metrics.





\subsection{Resource Throttling}
finding the best-matching hardware configurations for the application at hand

Since Cloud services are billed by the pay-as-you-go principle, organizations can save huge investment costs.Hence,  they want to know,  what costs will arise by the usage of those services.  On the other hand,  Cloudproviders  want  to  provide  the  

Therefore,CloudSim a popular  event-based  framework by Calheiros et al.,  was developed  to model  and simulate theusage of IaaS (Infrastructure-as-a-Service) Clouds.  Metrics like usage costs, resource utilization and energyconsumption can be also investigated using CloudSim.  But this favored simulation framework does not pro-vide any mechanisms to simulate todays object storage-based Cloud services (STaaS, Storage-as-a-Service).In this paper, we propose a storage extension for CloudSim to enable the simulations of STaaS-component





\subsection{Portability}
Benchmark portability~\cite{tsai1996approach, wilson2002progress} is a critical topic that until now remains largely overlooked. It is not uncommon to spot two different papers in the literature whose authors use the same benchmark, the same deployment, and yet find that the published result variate significantly. The reason typically has to do with the experimentation platforms they use. Although the experimentation platforms can be documented and compared qualitatively, it is much harder to achieve repeatable results across different infrastructures. Since important decisions depend on reliable experimental data, it is necessary to enable reproducible experiments and verifiable results. Using Kubernetes as an abstraction layer, it is now possible to create a new generation of portable benchmarks. Some of the merits of this approach include:
\begin{itemize}
    \item Physical resources are replaced by virtual counterparts whose capabilities are well specified and therefore recreated amongst different Kubernetes deployments.
    \item There are several Chaos Testing tools, like Chaos-Mesh, which we can use for fault injection. These tools typically consist of a high-level part for selecting fault parameters and a low-level part designed to cause (or simulate) faults at the targeted components. 
    \item Experiments can seamlessly scale from a single workstation to clusters of commodity servers or even larger enterprise-grade servers. Equally, they may run on-premise or in the Cloud.
\end{itemize}


%and finally,  evaluating the portability of experiments over different infrastructures.



%We will use the following vocabulary when describing the language. The tester is the framework's user. The System Under Test (\textit{SUT})~\cite{ulrich1999test} is the system/application we want to evaluate. It is a YAML definition that combines the following abstractions:



and apply patches or other customization. 

In our approach, complex Services with a wider functionality consist of smaller services with specific behaviors and use their functionality. Composite Services may use more than one class of dependent side-services. Code~\ref{code:service} implements the Services of Figure~\ref{fig:example}, and demonstrates how to compose Services 


\paragraph{Input / Params:}



 \frisbee{}  parses the environment variables before the deployment, and if a variable is undefined, the controller rejects the experiment preemptively. These semantics are stronger than Kubernetes, where incorrectly parsed variables will not block the container from starting.
 
 
 Given that writing experiments revolve around reusable code segments, we encourage users to store their experiments for future execution rather than just using the SDK for `one-off' job submission. For this purpose, we designed the language with capabilities for code composition. 
 
 
 
By design, Groups are homogeneous and can only include instances of the same service. Although we experimented with Supergroup that encapsulates instances from different groups, we soon dropped it as it would cause ambiguities on the user's input. Instead, we adhered to Golang's principle of `accept interfaces, return structs'. The crux of the idea is that since \frisbee{} provides graceful abstraction at the level of actions (will be discussed later), there is no need to abstract upfront. In simple words, if an action needs to operate on multiple groups, it is more explicit to take these groups as input rather than a Supergroup with ambiguous semantics. Code~\ref{code:scenario} demonstrates the use of inputs, scheduling constraints, and dependent groups. 


Although users can programmatically generate the list of inputs to iterate over, these inputs must be declared upfront. As such, it is not possible for a service to join an existing group. This decision simplifies and semantics and prevent us from consistency issues. However, 


On top of resulting in scenarios that are easier to understand, develop, and evaluate, it also facilitates troubleshooting. It is easier to verify the global properties of the application once the whole state is represented in a single place, rather than investigating the code of different scripts to find the anomaly. 



Importantly, failures are recovery and repetatable. 


Whereas Actions mimic system fluctuations that occur naturally during the normal operation, Failures 

For example, failures are necessary for studying the failover of a Redis cluster. Specifically, a network fault can be seen as physical network interference, connectivity uncertainty, or even a malicious attack. 






%Events are control structures that define when and what command to run next. We support three different types of events:

%The added value is that managing dependencies at the level of a \textit{Group}, rather than at the level of individual Services, result in simpler configurations and allows for maximum parallelism when running multiple Services.


Through this architectural style, users have c

\subsubsection{Actions}
\CHECKnote{[fn] Describe actions [ Refer to Dependencies, and Schedule ]}



We frequently needed to open the terminal into the Redis servers during our experiments and perform troubleshooting activities (mostly related to configuration). However, troubleshooting a running Service is difficult due to updates in the terminal's output logs. For this reason, we included the Pause command that can suspend the execution of a Service, either for a duration or until it is resumed manually. Like all \frisbee{} commands, Pause can be used either as a "single-shot" via the \frisbee{} Shell or as part of a more complex Scenario. 



\subsubsection{Failure Injection}



In this language, the tester defines the services to run, the execution parameters, and the testing workflow.  The execution parameters include resource and placement constraints for services,  logical groups of Services, and inter-service dependencies (e.g., wait for execution or completion). The workflow expresses the desired state over the experiment over time. That includes elastic actions that change the underlying topology (e.g., add or remove a service), failures that will happen to services (e.g., kill, partition, corruption), failure patterns (e.g., run a partition failure every 10 minutes), and callback functions that will be triggered upon certain events (e.g., push annotation to Grafana when a node has crashed).






\paragraph{Logical Groups:}







%The majority of such benchmarks generate a single, stationary workload per run, which is not representative of cloud native environments. Few benchmarks have built-in mechanisms to dynamically increase the load, in order to discover the peak throughput where diminishing returns (e.g., due to thrashing) begin to take over. For example, measuring NFS throughput via SPEC SFS [64] and process scheduling throughput using AIM7 [68].Filebench [47, 67] comes with several canned configurations [62] and even has its own Workload Mod-eling Language (WML) [73].   It,  however,  is not distributed (cannot run in a coordinated manner across multiple containers) and, though WML is flexible for encoding stationary workloads, is still limited in creating dynamically changing workloads.  In our experience, adding support for distributed and temporally varying workloads to Filebench’s WML is a difficult task.  Therefore, in CNSBench, we exploited the orchestration capabilities of cloud native environments and delegated these tasks to a higher level (i.e.,  the CNSBench controller and the Kubernetes orchestrator itself). This further allowed us to support any existing benchmarks as canned I/O generators.



%One of the core CNSBench capabilities is to make it easy to run various mixes of I/O workloads.  This is needed since the alternative is to manually choose and assemble workloads together to form a representative combined workload; the diversity of workloads in cloud native environments makes this task infeasible.One potential use case for this task is to determine which storage configuration is best suited for a particular set of workloads. Another might be to help influence scheduling decisions, such as which workloads to run simultaneously.To demonstrate CNSBench’s orchestration capabilities, we ran multiple instances of three different work-loads:  (1) MEGAHIT [59], a bioinformatics tool that processes genetic data; (2) fio [20] for generating an intense I/O workload of mixed random reads and writes; and (3) the PostgreSQL [40] database with a work-load generated using its benchmark tool pgbench [38].  Each instance of the PostgreSQL workload ran a distinct pair of database and client.  Out of each of the workloads, fio was the most I/O intensive, followed by pgbench. Both fio and pgbench spent most of their time waiting for I/O, whereas MEGAHIT was mostly CPU bound.We tested four different workload ratios: a baseline with ten independent instances of each workload, andthen three additional ratios with ten instances of two of the workloads and five of the third. For MEGAHIT and fio we measured the total time to run a fixed load; for pgbench we measured the average throughput after running for ten minutes.  This was necessary since the different storage provider configurations performed significantly different, so it would be impractical to evaluate using a fixed amount of work.






Let us assume a cluster of 3 Redis masters replication to 3 Redis slaves, with 10 parallel YCSB client (loaders) inserting keys and 5 YCSB clients (runners) executing mixed queries against the inserted keys. Redis masters serve both read and write requests, while slaves serve only read requests. For resiliency reasons, the masters must reside on different failure domains than slaves. The evaluation workflow consists of three distinct phases; Setup, Load, Run. These phases have logical and timely dependencies that must be respected. The key ingestion does not start unless the servers (both masters and slaves) are up and running. Similarly, the queries must be postponed until the distributed loaders have completed ingesting the keys. 



The setup is like before, but instead of iperf, the servers are now running the Redis in-memory data structure store~\cite{redis}. The clients run the YCSB benchmark~\cite{cooper2010benchmarking}. 



% The second experiment is exploratory. The first is for validation, the second for demonstration, and the third is exploratory.
%Using Frisbee, we will try to understand the reasons behind those trends. 


%Using this tiered environment, we design experiments to answer the following questions:
%\begin{enumerate}
    %\item Is there merit in using powerful servers over a slow network?
    %\item How does a database server respond to transient clients and bursty traffic that dominate IoT?
    %\item What is the impact of running a distributed database at both Edge and Cloud nodes?
    %\item Does a fast network provide more stable performance than a slow one?
    %\item Is it better for an Edge to make replicas on other Edge nodes or to the Cloud?
%\end{enumerate}






Job

for bringing a task to completion.

It further lacks su

In \frisbee{} terms, it supports WaitExit but not WaitReady dependencies. They also lack support for failure injection and application monitoring. 

chaomesh




Netflix has released Chaos Mon-key [56] as open source19. Chaos Monkey randomly ter-minates virtual machines and containers running in thecloud. This approach’s intuition is that failures will occurmuch more frequently, so engineers are encouraged to aimfor resilience. 



Chaos Monkey does not provide the runtimeinfrastructure as we do, but it would complement our ap-proach very well. For instance, Chaos Monkey could beintegrated into MockFog’s experiment orchestration mod-ule. Another solution that complements MockFog is De-Fog [33].  
 


it lacks supports for workflows with more complex dependencies. 






they lack support for dependent workflows. Moreover, 


 
 Based on the papers, theprototypes also appear to be designed for single machinedeployment – which limits scalability – while MockFogis specifically designed for distributed deployment.
 
  
  
  Still, one could in-tegrate such testbed emulation approaches in MockFog’sinfrastructure module to support other execution environ-ments while still benefiting from automated experimentorchestration



 Missingsupport for experiment orchestration is also a key differ-ence between MockFog and MAMMOTH [30], a large scaleIoT emulator, Distem [49], a tool for building experimenttestbeds with Linux containers, and EmuEdge [60], andedge computing emulator that supports network replay.



DeFog comprises six Dockerized benchmarksthat can run on edge or cloud resources. From the Mock-Fog point of view, these benchmark containers are work-load generating application components, i.e., load genera-tors. Thus, they could be managed and deployed by Mock-Fog’s application management and experiment orchestra-tion module. Gandalf [29] is solely a monitoring solutionfor cloud deployments.  Azure, Microsoft’s cloud serviceoffer, uses Gandalf in production. It is therefore not partof the application engineering process (Figure 3) and couldbe used after running experiments with MockFog. Finally,MockFog can be used to evaluate and experiment withfog computing frameworks such as FogFrame [54] or UR-MILA [52].


computation and storage realism is usually overlooked.


EMU-IoT [44] is aplatform for the creation of large scale IoT networks. Theplatform can also orchestrate customizable experimentsand has been used to monitor IoT traffic for the predictionof machine resource utilization [43]. EMU-IoT focuses onmodeling and analyzing IoT networks; 

 Having only a singlehost for virtual machines significantly limits scalability
 
 
 
 WoTbench [22, 23]can emulate a large number of Web of Things devices ona single multicore server. As such, it is designed for ex-periments involving many power-constrained devices andcannot run experiments with many resource-intensive ap-plication components such as distributed application back-ends.

 
 Héctor [5] is a framework for automated testing of IoT ap-plications on a testbed that comprises physical machinesand a single virtual machine host. 


 
 Addi-tionally, network delays and failure rates can be definedto model a realistic, geo-distributed system. 
 


 

 
 




Yet, variable environmental noise and device wearing forfeit the reproducibility of results. Simulation is an alternative solution that is both cheaper and guarantees reproducibility. A simulator represents a system with mathematical models. It further provides programmable events through which operators can evaluate their systems under dynamically changing conditions. On the downside, simulators are usually inappropriate for testing real applications. Emulation is a technique for running real applications over virtual components designed to mimic real devices (e.g., throughput, operations per second). Unfortunately, most emulators today suffer from three main deficits: (1) they lack programmable events, (2) they offer limited scalability, (3) they do not support tiered architectures.



Classic storage benchmarks.Storage benchmarking is an oldand complex topic with many applicable techniques and intricatenuances [59]. Therefore, it is not surprising that the array oftools for benchmarking and corresponding studies is extensive.Filebench [60], fio [15], SPEC SFS [36], and IOZone [45] arejust a few examples of popular file system benchmarks. For acomprehensive survey of file system and storage benchmarkswe refer the reader to a study by Traeger et al. [63].The majority of such benchmarks generate a single, stationaryworkload per run, which is not representative of cloud nativeenvironments. Few benchmarks have built-in mechanisms to dy-namically increase the load, in order to discover the peak through-put where diminishing returns (e.g., due to thrashing) begin totake over. For example, measuring NFS throughput via SPECSFS [58] and process scheduling throughput using AIM7 [61].Filebench [42, 60] comes with several canned configura-tions [56] and even has its own Workload Modeling Language(WML) [66]. It, however, is not distributed (cannot run in acoordinated manner across multiple containers) and, thoughWML is flexible for encoding stationary workloads, is stilllimited in creating dynamically changing workloads. In ourexperience, adding support for distributed and temporally varyingworkloads to Filebench’s WML is a difficult task. Therefore,inCNSBench, we exploited the orchestration capabilitiesof cloud native environments and delegated these tasks to ahigher level (i.e., theCNSBenchcontroller and the Kubernetesorchestrator itself).  This further allowed us to support anyexisting benchmarks as canned I/O generators.RocksDB [48] is a popular key-value store with canned,preconfigured workloads using a dbbench driver to createrandom/sequential reads/writes and mixes thereof. One can runthese workloads in any order and configure their working-setsize. However, that is still a manual process with little flexibility,and no support for control operations (which is true for thepreviously mentioned benchmarks as well).Object storage benchmarks.In recent years the need totest the performance of cloud storage has motivated academiaand industry to develop several micro-benchmarks for thattask such as YCSB [46] and COSBench [67]. YCSB is anextensible workload generator that evaluates the performance ofdifferent cloud-serving key-value stores. COSBench measuresthe performance of cloud object storage services and comes withplugins for different cloud providers. Unlike these benchmarks,CNSBenchfocuses on workloads that run in containers andrequire a file system interface.



Systems testing and benchmarking is a well-established and prolific field. 






\subsection{Chaos Engineering}
Chaos Engineering is a production testing methodology pioneered by Netflix with the goal to build confidence in their geographically distributed video caches to withstand turbulent and unexpected conditions. The two key features of Chaos engineering~\cite{gunawi2011failure,zhang2019chaos,basiri2016chaos} are to: 
\begin{enumerate*}[(a)]
    \item form a hypothesis about the expected behavior of the system in the presence of a given failure, 
    \item and perform the smallest possible experiment on production instances. 
\end{enumerate*}

For example, Netflix hypothesizes that its platform can withstand arbitrarily failing services. To investigate this hypothesis, a `chaos experiment' consists of randomly shutting down a virtual machine and checking that this perturbation has no significant influence on the main business metric of Netflix: the number of served video streams per second. Netflix assumes that confidence in past experiments' results decreases as the system evolves, and has developed the NDBench~\cite{papapanagiotou2018ndbench} microbenchmark to automate the execution of long-running (infinite horizon) experiments with variable workloads, while ChaosMonkey (the Chaos suite of Netflix) causes random failures on the production services. s.








%predict the behavior of a distributed system if deploed on 

%emulate IoT devices by restricting the container's access to the host's CPU, Memory, and Storage resources so that the observed performance matches the performance of an actual device. 

%accurately predict the behavior of modern network services while employing an order of magnitude fewer

%While not technically or economically feasible, a comprehensive evaluation would require running a test system identically configured to and at the same scale as the original system. Thus, we need adequate test suites that can accurately predict the behavior of modern network services while employing an order of magnitude fewer hardware resources~\cite{gupta2011diecast}. This challenge can be divided into two complementary tasks: high-load emulation and device emulation.  Concerning the load emulation, the key idea is to mimic high-load by throttling the underlying resources and cause resource starvation/saturation on the worker nodes. This way, we can achieve the desired conditions with fewer load-generating clients, thus saving operational costs. Concerning device emulation, the idea is to . Along with the emulation of devices comes the emulation of network protocols. 


%capabilities for fault injection, distributed monitoring, and dynamic workloads described as directed acyclic graph


%enriches Kubernetes to support sequences of scheduled or conditional actions 
%Beyond the capabilities for 

%Our vision with \frisbee{} is to develop 


%a framework to transform a Kubernetes cluster into an experimentation platform. Our vision with \frisbee{} is to develop 

%capabilities for fault injection, distributed monitoring, and dynamic workloads described as directed acyclic graph

%It is designed from the ground up to facilitate the exploration, testing, and benchmarking, of distributed systems under various operating conditions and dependent workflows. It provides: infrastructure automation, such as 



%so we need network virtualization to programmatically emulate different network conditions and ensure that applications respond correctly without losing data. 



%Among many TaaS issues, this paper addressed the following four issues:

    %Clustering the tenant requests according to their similarity in terms of hardware, OSs, supporting kits and testing services, such that the configuration time and setup time are minimized.

    %Scheduling the clustered tasks such that the test requirements and deadline can be met.

    %Monitoring all testing resources and task status assigned.

    %Managing cloud resources including creating, maintaining and migrating processes and processors at runtime according to the scheduling decision.

%The structural abstractions of the testing process are a vital feature of an experimental platform. These abstractions are a result of a delicate equilibrium. They must be general enough not to limit the tester's expressiveness and cohesive enough to enable rapid prototyping without sacrifice the 



aggregate values tend to hide  

operation errors

modern benchmarks. 

that mixed workloads often exhibit artifacts, such as slow operation and operation errors, that aggregated values tend to hide, thus leading to invalid conclusions. We 

insights that can influence the way we evaluate our applications. The most prominent are 




we study  under the presence of a network partition.

experiments with 

experiment goes through various phases, with every phase characterized by a unique combination of 

examine the impact that variable I/O workloads can have on overall performance of a system. 

dynamic allocation of server resources, the effectiveness of recovery mechanisms, and the effects of tiered placement. 

We find numerous insights that can influence the way we evaluate our applications.


We find numerous insights that can influence the way we evaluate our applications. First, although aggregate values can reveal baseline performance characteristics, mixed workflows often exhibit artifacts, such as slow operation and operation errors, that aggregated values tend to hide. Thus, without granular monitoring, engineers may draw invalid conclusions and unfair comparisons. Second, even the most popular benchmark (YCSB) does not support failover for Redis, one of the most popular key/value stores. Lastly, we have already integrated \frisbee{} into the continuous testing pipelines of our team, so to run a repeatable set of performance tests whenever we make a commit to the code repository. Thus, beyond the functional testing, we have fast feedback that this change will not impact the product negatively. Given all the above, we foresee that platforms like \frisbee{} will play an essential role in designing and evaluating future systems and distributed applications.


we validate the mechanisms for throttling memory, CPU, and disk I/O.












% So we have pods running nginx in a flat, cluster wide, address space. In theory, you could talk to these pods directly, but what happens when a node dies? The pods die with it, and the Deployment will create new ones, with different IPs. This is the problem a Service solves.

%A Kubernetes Service is an abstraction which defines a logical set of Pods running somewhere in your cluster, that all provide the same functionality. When created, each Service is assigned a unique IP address (also called clusterIP). This address is tied to the lifespan of the Service, and will not change while the Service is alive. Pods can be configured to talk to the Service, and know that communication to the Service will be automatically load-balanced out to some pod that is a member of the Service.





\subsection{Containers}

An API, typically based on JavaScript Object Notation (JSON) or XML, is often layered on top of the transport protocol to make it easier for developers to interact with the device. Testers can use the protocols and APIs for automated testing, and the test design depends on which APIs and protocols are being used. The testing tool must be able to support these protocols and APIs in order to be effective.

\subsection{Resource Throttling}

% Thing : UFS21 
% Edge: SSDm2 (1 CPU)

\begin{table}[htbp]
\centering
\begin{tabular}{c c c c c} 
 \hline
 Storage Profile & Seq.Read & Seq.Write & Rand.Read & Rand.Writer \\ [0.5ex] 
 \hline\hline
 UFS 2.1 & 880 MB/s & 200 MB/s & 40K IOPS & 40K IOPS \\
 SSD M.2 & 2 GB/s & 700 MB/s & 170K IOPS & 130K IOPS \\ [1ex] 
 \hline
 \end{tabular} 

\caption{Performance profiles for IoT devices. Interoperability between the devices is feasible because 802.11ac is backward compatible with 802.11n}
\label{table:devices}
\end{table}


\subsection{Network Emulation}

Newer architectural paradigms represent a departure from the centralized Cloud model, where the nodes available to a single-tenant reside in a small number of well-interconnected data centers.


%Fast-moving data and increased load take a toll

%

Connected IoT devices rely on fast communication. Consequently, network status can have a significant effect on device performance. 


\subsection{Failure Injection}

Even, If developers put all of the stateful components in cloud services, they cannot necessarily simulate outages the same way. They will have to rely on the cloud provider's info to correlate storage events with application behaviors. Moreover, an apples-to-apples comparison is problematic, given numbers for different systems based on different infrastructures.  





\subsection{Resource Throttling}


 For example, if systems A and B share a control unit and system A is on a much faster processor complex, system A could monopolize the control unit because it can issue I/Os faster. By throttling devices owned by system A on the shared control unit, system B would not see as much contention at the control unit level.



\subsection{Workflow}

\subsubsection{Failure Injection}


detect, reason and fix bugs when changes are systematically mastered (or edited) as part of a Workflow, 






\subsection{Storage System Characteristics}
Clouds serving systems share common goals, despite the different architectures and design decisions. In general, these systems aim for:

\begin{itemize}
    \item \textbf{Scalability} is the ability of the system to accommodate larger loads just by adding resources either making hardware stronger (scale up) or adding additional nodes (scale out). 
    
    \item \textbf{Elasticity} is the ability to fit the resources needed to cope with loads dynamically usually in relation to scale out. In other words, elasticity means that we can add more capacity to a running system by deploying new instances of each component, or reduce costs by removing components. 
    
    \item \textbf{Availability} refers to system uptime, i.e. the storage system is operational and can deliver data upon request. For data centers, availability/uptime is a key metric for operations as any minute of downtime is costly. Historically, this has been achieved through hardware redundancy so that if any component fails, access to data will prevail. 
    
    \item \textbf{Durability}, refers to long-term data protection, i.e. the stored data does not suffer from bit rot, degradation or other corruption. Rather than focusing on hardware redundancy, it is concerned with data redundancy so that data is never lost or compromised.
\end{itemize}
 



\subsection{Metrics}

Go has a de facto standard format for benchmark data: the lines generated by the testing package when using go test -bench. For example, running compress/flate's benchmarks produces this output:

 %Below are a few of the most widely used representations.
\CHECKnote{[MM] citations?}

%can learn how components intermix and work together, and

\todo[inline]{Explain Phase 1, Phase 2}


  Additionally, self-healing systems should be able to anticipate conflicts trying to prevent possible failures.
\CHECKnote{[MM] "anticipate" as in "predict" ?}
 

 



%Mean Time To Repair - MTTRThis metric depicts the duration of the repair and recoverytime. This means that if the time between the initial failure andsubsequent repair putting the system back to working order is10  minutes,  then  the  MTTR  is  10  minutes.  Repair  can  come in  the  form  of  an  automatic  recovery  (e.g.  RAID  rebuilding)or manually by an operator

%In the first phase, evaluators use a fault-injection infrastructure to measure the impact of faults on the server's performance. In the second phase, evaluators use an analytical model to combine an expected fault load with measurements from the first phase to assess the server's performability. 





\subsection{Defining Steady State}


his CL fixes this by introducing a victim cache mechanism. Instead of clearing Pools, the victim cache is dropped and the primary cache is moved to the victim cache. As a result, in steady-state, there are (roughly) no new allocations, but if Pool usage drops, objects will still be collected within two GCs (as opposed to one). — Austin Clements


On my system BenchmarkFibWrong never completes. This is because the run time of the benchmark will increase as b.N grows, never converging on a stable value. BenchmarkFibWrong2 is similarly affected and never completes.

MaxHeap, which is not yet released but is being used and evaluated internally, lets the programmer set what the maximum heap size should be. Out of memory, OOMs, are tough on Go; temporary spikes in memory usage should be handled by increasing CPU costs, not by aborting. Basically if the GC sees memory pressure it informs the application that it should shed load. Once things are back to normal the GC informs the application that it can go back to its regular load. MaxHeap also provides a lot more flexibility in scheduling. Instead of always being paranoid about how much memory is available the runtime can size the heap up to the MaxHeap.

The other piece of this code is the GC Pacer. It is some of the great work that Austin did. It is basically based on a feedback loop that determines when to best start a GC cycle. If the system is in a steady state and not in a phase change, marking will end just about the time memory runs out.



// testFlakiness runs the function N+2 times and prints metrics diffs between
// the second and subsequent runs.
func testFlakiness(f func() Result, N int) {
	res := make([]Result, N+2)
	for i := range res {
		res[i] = f()
	}
	fmt.Printf("\n")
	for k, v := range res[0].Metrics {
		fmt.Printf("%v:\t", k)
		for i := 2; i < len(res); i++ {
			d := 100*float64(v)/float64(res[i].Metrics[k]) - 100
			fmt.Printf(" %+.2f%%", d)
		}
		fmt.Printf("\n")
	}
}

A flaky test is a test that both passes and fails periodically without any code changes. Flaky tests are definitely annoying but they can also be quite costly since they often require engineers to retrigger entire builds on CI and often waste a lot of time waiting for new builds to complete successfully.

x

Basically benchmark test suite of the testing package gives the benchmark reports likes time consumed, number of iteration/request(i.e. execution of function) of the tested function.

Causes of flakiness

There are many causes of flakiness but the few I highlight in my talk are:

    Inconsistent assertion timing – when your application state is not consistent between test runs you will notice that expect/assert statements fail randomly. The fix for this is to construct tests so that you wait for the application to be in a consistent state before asserting. I am not talking about “wait” statements either. You should have predicates in place to poll the application state until it reaches a known good state where you can assert.
    Reliance on test order – global state is the main culprit that causes tests to be reliant on other tests. If you see that you cannot run a test in isolation and it only passes when the whole suite is run then you have this problem. The solution is to entirely reset the state between each test run and reduce the need for global state.
    End to end tests – end to end tests are flaky by nature. Write fewer of them. Instead of having 500 end to end tests for your organization, have 5.
    
    
     
     
     To date, academic research has focused primarily on trying to identify which tests are flaky and which are reliable. Software engineering practice, however, shows that all real-world tests are flaky to some extent, even if they are implemented following best engineering principles. Thus, the right question to ask is not whether a particular test is flaky, but how flaky it is. To answer this question, we’ve developed a measure of test flakiness: the probabilistic flakiness score (PFS). Using this measure, we can now test the tests to measure and monitor their reliability, and thus be able to react quickly to any regressions in the quality of our test suite.
     
     Retrying those multiple times is time-consuming, and trying to modify the test is far more complex. We need a very reliable signal when code changes are made, so developers won’t waste time chasing down problems that don’t really exist. 
     
     
     
     
Test Flakiness - One of the main challenges of automated testing
Wednesday, December 16, 2020
By George Pirocanac
Dealing with test flakiness is a critical skill in testing because automated tests that do not provide a consistent signal will slow down the entire development process. If you haven’t encountered flaky tests, this article is a must-read as it first tries to systematically outline the causes for flaky tests. If you have encountered flaky tests, see how many fall into the areas listed.
A follow-up article will talk about dealing with each of the causes.
Over the years I’ve seen a lot of reasons for flaky tests, but rather than review them one by one, let’s group the sources of flakiness by the components under which tests are run:

    The tests themselves
    The test-running framework
    The application or system under Test (SUT) and the services and libraries that the SUT and testing framework depend upon
    The OS and hardware that the SUT and testing framework depend upon

This is illustrated below. Figure 1 first shows the hardware/software stack that supports an application or system under test. At the lowest level is the hardware. The next level up is the operating system followed by the libraries that provide an interface to the system. At the highest level, is the middleware, the layer that provides application specific interfaces.
In a distributed system, however, each of the services of the application and the services it depends upon can reside on a different hardware / software stack as can the test running service. This is illustrated in Figure 2 as the full test running environment.
As discussed above, each of these components is a potential area for flakiness.
The tests themselves
The tests themselves can introduce flakiness. Typical causes include:

    Improper initialization or cleanup.
    Invalid assumptions about the state of test data.
    Invalid assumptions about the state of the system. An example can be the system time.
    Dependencies on the timing of the application.
    Dependencies on the order in which the tests are run. (Similar to the first case above.)

The test-running framework
An unreliable test-running framework can introduce flakiness. Typical causes include:

    Failure to allocate enough resources for the system under test thus causing it to fail coming up. 
    Improper scheduling of the tests so they “collide” and cause each other to fail.
    Insufficient system resources to satisfy the test requirements.
    
    
    
    

The continued use of multiple approaches highlights both the value and inadequacy of each. Netbed, a descendant of Emulab, provides an experimentation facility that integrates these approaches, allowing researchers to configure and access networks composed of emulated, simulated, and wide-area nodes and links. Netbed's primary goals are ease of use, control, and realism, achieved through consistent use of virtualization and abstraction.By providing operating system-like services, such as resource allocation and scheduling, and by virtualizing heterogeneous resources, Netbed acts as a virtual machine for network experimentation. This paper presents Netbed's overall design and implementation and demonstrates its ability to improve experimental automation and efficiency. These, in turn, lead to new methods of experimentation, including automated parameter-space studies within emulation and straightforward comparisons of simulated, emulated, and wide-area scenarios.






Three experimental environments traditionally support distributed systems research: 
live testbeds, network simulators, network emulators. 








Network, CPU, Amplification


 
%Hence, additional instrumentation is required to obtain the inner state of a running system, in order to know when a replication process starts and when it ends. The same goes for other tasks like scrubbing. 



\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/architecture.pdf}
    \caption{Frisbee Architecture}
    \label{fig:architecture}
\end{figure}

%Here is an example of how we use Chaos Mesh to locate a TiDB system bug. In this example, we simulate Pod downtime with our distributed storage engine (TiKV) and observe changes in queries per second (QPS). Regularly, if one TiKV node is down, the QPS may experience a transient jitter before it returns to the level before the failure. This is how we guarantee high availability.


%Each MongoDB cluster can output its logs into this pipeline making it available for your favorite log aggregators. You can also push events into MongoDB Ops Manager for viewing, alerting and making performance tuning recommendations.










% [ In the above, the human operator requires to see the variation in the plots and interprets what is happening based on the knowledge of inter-workings of the system. We need something more automated ]

%Although these Hypothetical faultloads are deduced from the failure characteristics of systems under evaluation, they are system independent and assume no knowledge of the system's inner workings. 




One of the most common ways to benchmark a system is with a workload. 
Performance benchmarks have CPU, memory, I/O, and other intensive programs for testing different components of a system. These intensive programs use workloads specialized for testing responses to integer and floating-point arithmetic, network throughput, etc. Similarly, Cloud benchmarks run workloads to submit requests to Cloud services and measure the Queries per second and tail latency.


You specify both the java class and the parameter file on the command line when you run the YCSB Client. The Client will dynamically load your workload class, pass it the properties from the parameters file (and any additional properties specified on the command line) and then execute the workload. 


Confidence intervals are intrinsically connected to confidence levels. Confidence levels are expressed as a percentage (for example, a 95\% confidence level). It means that should you repeat an experiment or survey over and over again, 95 percent of the time your results will match the results you get from a population (in other words, your statistics would be sound!). 





Unreliable, also known as flaky, tests produce false or nondeterministic signals that undermine engineers’ trust and thus the effectiveness of the entire regression testing process. If a test sometimes passes and sometimes fails, without a change to the underlying product or app, it forces engineers to spend their time chasing down issues that may not even exist. This undermines their trust in the testing process. It is thus important to determine whether a test has become flaky.
     


%The  authors  chose  to  useexperts  to  perform  the  benchmarking  to  exclude  any  unnecessary faults. However as long as the same level of operatorsdo  the  testing  on  all  systems  to  be  benchmarked,  there  willbe  no  real  problem.  The  authors  stated  the  problem  withrepeatability was that once testers were exposed to a fault, theylearned how to solve it. The next time the test was run, theywould already know  what to do. They referred  to this as thelearning curve. Tasks and problems the operators would faceare initial configuration, reconfiguration, monitoring, diagnosisand repair, an preventative maintenance

 If a test sometimes passes and sometimes fails, without a change to the underlying product or app, it undermine engineers' trust and thus the effectiveness of the entire testing process.
 
  A test that fails randomly is commonly called a flaky test. Flaky tests hinder your development experience, slow down progress, hide real bugs and, in the end, cost money.
     
     Dealing with test flakiness is a critical skill in testing because automated tests that do not provide a consistent signal will slow down the entire development process.
     
     confidence issues transparently to the developer

To simplify development, 



A key design goal of our tool is extensibility of faultloads. The developer, however, should not be bogged with confidence issues. To simplify development of new faultloads, Frisbee framework provides a  that handles .

Benchmarks are 

Just like your test cases, benchmarks are placed inside the _test.go files, and instead of a function starting with Test it need to start with Benchmark.




%You must call your function b.N times, and that is why we are using a for loop to iterate till b.N times.



%   The final BenchmarkFib40 only ran two times with the average was just under a second for each run. As the testing package uses a simple average (total time to run the benchmark function over b.N) this result is statistically weak. You can increase the minimum benchmark time using the -benchtime flag to produce a more accurate result. 





\subsection{Tier1 - Tolerance}

\subsection{Tier1 - Fairness}

\subsection{Tier1 - Corrective Actions}
Consistent Behavior

\subsection{Tier1 - Predictive Actions}
Learning Curve 




\section{Challenges}

\subsection{Reliability versus Availability vs Serviceability}


 Definitions may vary in considered time window (e.g, Instantaneous versus Average Uptime availability), initial state (e.g, from bootstrap vs from steady state), or sources of downtime (e.g, preventive, predictive, or corrective maintenance). 




There is a difference between reliability and availability. Depending on a customer ’ssituation, benefits may favor reliability over availability or vice versa. For instance,reliability must have a higher precedence in cases where systems are placed inremote areas and maintenance is expensive.



Reliability measures the ability of a system to function continuously without interruptions. A high MTBF for a computer system indicates that on average, thesystem can operate for extensive periods of time without component failureinterruptions. On the other hand, availability, measures the ability of a system to support a committed application service level


High availability is often associated with fault-tolerant systems. The termfault-tolerantmeans a system can operate in the presence of hardware component failures.A single component failure in a fault-tolerant system will not cause a systeminterruption because the alternate component will take over the task transparently.


Reliability measures the ability of a system to function without interruptions, while availability measures the abilityof a system to provide a specified application service level to clients. Therefore,reliability provides a metric of how often a component fails, while availabilityincludes the effects of downtime any failures produce

The academic definition of reliability,R(t),is the probability of a system performingits intended function over a given time period,t. As an example, a system with a0.9999 reliability over one year has a 99.99% probability of functioning withoutfailures throughout an entire year.Reliability is only one of many factors that influences availability, for example,99.99% reliability does not mean 99.99% availability. Reliability measures the abilityof a system to function without interruptions, while availability measures the abilityof a system to provide a specified application service level to clients. Therefore,reliability provides a metric of how often a component fails, while availabilityincludes the effects of downtime any failures produce.

A commonly used metric for measuring reliability is referred to asMean TimeBetween Failure(MTBF), which is the average time interval (normally in hours)between two consecutive component failures. Reliability is improved when the timeinterval spanning separate failures is extended.

\subsection{Availability Metrics}

\subsection{Measuring Availability}





These assertions, and the general need for advancing benchmarking availability features and capabilities, provide sufficient justification for system recovery benchmarking.


guarantee that the  will follow the same sequence of steps, and it is thus 


restore itself from an abnormal (or “unhealthy”) state to the normative (“healthy”) state, without human intervention. Other than reducing recovery time from   



to regain its normative performance levels following a failure

to efficiently detect failures and , 

recover from them, 

and recover from failures, 


to  . 

reproducible and measurable, and can thus be benchmarked.





 This contradicts databases with no self-healing properties, where 


repeatable and verifiable tests.






Although most of the \frisbee{} primitives operate at the level of the Group, we frequently needed to address individual services. The problem is that even with a predictable naming pattern, things can go wrong when addressing the services directly. First,  the order in which service containers come up is random, so it is possible to refer to a service that is not yet created. Second, services may join or leave the environment randomly, thus making the reference invalid. Third, apart from being impractical, hard-coding the names of the services constrains the scalability of the experiment. For example, if we wish to scale an experiment from 10 clients to 100 clients, we can simply change the number of clients, not hard-code another 90 names. 

NFTAPE, a tool for composing automated fault injection experiments from available lightweight fault injectors, triggers, monitors, and other components, helps to solve these problems. We have conducted experiments using NFTAPE with several types of lightweight fault injectors, including driver-based, debugger-based, target-specific, simulation-based, hardware-based, and performance-fault injections. Two example experiments are described in this paper. The first uses a hardware fault injector with a Myrinet LAN; the other uses a Software Implemented Fault Injection (SWIFI) fault injector to target a space-imaging application

One of the early studies on evaluating
the robustness of a system through fault injection
was [Miller90], which evaluated the behavior of
UNIX systems by passing invalid argument strings
to various utilities

and fix the cause of the failure in the crashing service while addressing the behavior of the dependent services that failed as a result.

you're able to "break things on purpose" in order to learn how to build more resilient systems.


 in a controllable  

 
 
 

 is often a process of seeing what problems arise when a service fails in production, then 

  















However, there are 

This, however, cannot be generalized 

The irony in this definition is that makes it trivial to calculate availability for a given system, but it shatters all efforts for an apples-to-apples comparison between systems. 


The first challenging in adopting 

Assessing availability requires examining the reliability of the hardware running the system, as well as how quickly and effectively teams can restore system performance after a failure.





 there are a few technological trends that can helps us benchmark how fast a system detects and recovers from a failure. 


The first trend is that today more DevOps teams are leveraging the power of containerization and virtualization technologies like Kubernetes to manage containerized database clusters. This standardization of infrastructure not only allows us to have a common reliability reference for virtual resources, but it also allows us to inject failures at various levels including the disk, the network, or the software. 




 Such
benchmarks are intended to provide a relatively
objective set of data that can be used to compare
.



in quantification of availability in a 

It may be possible to characterize failure patterns for a given infrastructure, but there variability of modern data centers is yet to be modelled in a generic pattern. 





In this paper, we present a 


The focus of the work cited in the previous
paragraph has been system robustness – an
important attribute of availability.  general purpose computers today
implement quick recovery designs that enable a
system to reboot following a fatal fault event.
Typical designs include the ability to reboot around
failed hardware components without human
intervention. 






the recovery time of modern key/value databases under the precense of a variety of failures. 

how fast a system  to recover from an outage



event-driven and not time-driven. For example, to calculate 

fault injection should take 
 
 







 there are two technological trends that makes recovery time consistent, reproducible
and measurable, and can thus be benchmarked.







Although it is possible to quantify availability 

Secondary, 






In this paper we leverage two technological trends that make availability benchmarks feasible: self-healing and containerization. 

Mean Time Between Failures (MTBF) reflects the frequency at which the hardware running the system fails. The higher the time between failure, the more reliable the system. 







There are however two new technological trends can open new avenues in measuring availability. 









Ourexperience has shown that these steps are ,  and  can  thus  be  benchmarked, 


are more complex than performance benchmarks and 

In contrast to performance benchmarks that are implemented by sending requests from clients to the servers, 

Moreover,  is hard, 





[Why ]

In contrast to other benchmark suites, which are usually designed to report a particular performance point, 



However, With more businesses depending on key/value databases for their mission-critical data, there is a natural demand for availability benchmarks. Ιn contrast to the plethora of performance benchmarks, as of today, there is no existing industry-wide benchmark for availability. The reason is that availability is not something directly measurable, but is a function of two metrics: reliability of the hardware and human response time to failures. Unfortunately, none of them can be easily generalized, and therefore it is impossible to design benchmarks that yield repeatable results. There are however two technological trends that open new avenues in availability benchmarks: Containerization and Self-healing systems. 



since no single component can guarantee 100\% uptime (and even the most expensive hardware eventually fails),  



%The lack of such a benchmark continues to
%leave a gap in the evaluation process, and it is
%generally agreed throughout the industry that a
%method for benchmarking availability is needed. 



 much  likeperformance benchmarks (e.g. TPC, SPEC). A defined setof   measurements,   coupled   with   a   specification   forrepresenting  the  results  and  system  variables,  providesthe foundation for system recovery benchmarking



This definition, however, makes it challenging to create benchmarks that cover all possible systems and infrastructures. 








measure availability on different systems. The first reasons is that 


Reliability cannot be easily generalized since 





The first reason is that availability measurements require fault injection at the level of infrastructure -- and since 



bring the system back to its nominative performance level, prior to a disruption


 As of today there is not competent solution. 

%This paper describes a benchmark for measuring
system recovery on a non-clustered standalone
system. 

 outages and technical incidents matter more than ever before. Despite the, as of today there is not competent solution. 


 there is a . The reason that as of today there is not competent benchmark, is that availability is not . It is rather a function of two metrics that cannot be easily generalized: Mean-Time-Between-Failure (MTBF) and Mean-Time-To-Recover (MTTR). The former depends on the infrastructure running the system, and the latter on the maintenance team repairing the system after a failure. 



 This way, it becomes trivial to compare whether certain storage or processing tasks are better served by a single powerful machine, or by multiple less-powerful machines. 
 


Which is why it’s important for companies to quantify and track metrics around uptime, downtime, 

Availability is typically accounting for both the reliability and repairability properties of a system


equip their systems with self-healing properties. A self-healing system 

.  A self-healing system  Hence, by 


Software failures are design problems, not wear and tear problems. Software doesn't fail due to getting "worn out" with use. Software fails because of design errors. So, while an engine will fail from time to time (without preventative maintenance) due to parts wearing out, software will work perfectly until it encounters inputs it was not designed to handle, then it fails completely until those inputs are removed. [ Hardware fails due to design errors too, and there are MTBF models specifically aimed at this 'prototyping' phase. See the argument up top and the link to

In this paper, 



with each trying to reach no single points of failure, and intelligently rebalance, repair, and replicate while maintaining data integrity at all times.


In this context,  began flourishing.


and repairability are business-specific 

availability is based on two metrics that disallow repeatable experiments: 

However


Though there are multiple definitions for availability, the most applicant definition for Cloud systems is inherit availability. It describes the availability of a system that has reached a steady state, and considers only corrective maintenance downtime of the system~\cite{}. 

\begin{equation}
    A = \dfrac{MTBF} {MTBF + MTTR}
\end{equation}


Corrective maintenance is also referred to as the availability as seen by maintenance personnel, because it reflects the time it takes for 



In light of , MTTR depends on how fast a system 




 Hardware redundancy (e.g, RAID, network links) is one way to minimize the impact of a failure on a system.  Although hardware redundancy serve well small clusters, the large cost of deploying hardware at scale has forced Internet companies to adopt less-reliable commodity. As a result, the heterogeneity in both hardware components and workload introduced more complex failure models, making rectification of system faults more difficult, labor-intensive, expensive, and error-prone.

















As key/value databases become the defacto storage systems for distributed applications, adopting a fast, reliable, and cost-efficient solution becomes critical. 


As key/value databases become the defacto storage systems for distributed applications, there is a natural demand for availability benchmarks. 




Mean-Time-Between failures is a common metric used to describe the rate at which failures occur in a given infrastructure.


Although almost all self-healing systems are based on data redundancy, the various approaches differ greatly. 

Some 















0000000000000000000000000000000000000000000000000000000000



 







Mean time to repair is not always the same amount of time as the system outage itself. In some cases, repairs start within minutes of a product failure or system outage. In other cases, there’s a lag time between the issue, when the issue is detected, and when the repairs begin.

This metric is most useful when tracking how quickly maintenance staff is able to repair an issue. It’s not meant to identify problems with your system alerts or pre-repair delays—both of which are also important factors wh


Mean Time To Repair (MTTR) reflects the time it takes to repair a failure, and  The goal is to get this number as low as possible by increasing the efficiency of repair processes and teams. 



Unfortunately, reliability cannot be generalized for different infrastructures as they host host generations of heterogeneous hardware, both commodity and custom design. Equally, 



Unfortunately, MTBF cannot , and MTTR is not easily measurable as it involves human factor. Hence, it is challenging difficult to design a generic availability benchmark with repeatable results. 





we explore the potentials of designing availability benchmarks based on two technological trends: . We present 




This paper  for creating a generalized availability benchmark based 







In  today’s  always-on  world, there  that helps to strike the right balance among software stack complexity, hardware,and operation cost, reducing the total cost of ownership(TCO) in data centers. As of today there is not competent solution. 










different infrastructures have different components and therefore different, unique failure modes




 


R-Cubed was proposed as a more inclusive definition to the traditional Reliability, availability and serviceability (RAS) terms~\cite{1997HighAF}. 

In , reliability provides a metric of how often a component fails, while availability includes the effects of downtime any failures produce. Serviceability is synonymous  with recoverability - the  characteristic of a system’s reaction to faults, errors, or maintenance events. 


Both these factors affect 

Hence, variability in 


These auto reboot/quick recovery
mechanisms tend to execute the same sequence of
steps, and are thus both .
Predictability is critical to mission-critical
computing, and system recovery time is a critical
component of the overall availability picture. Thus,
there is real value in quantifying recovery time.


Developers traditionally rely on performance benchmarks for selecting the right database technology for their applications. 


There are however multiple reasons for which such benchmarks were feasible before. 
\begin{itemize}
    \item Foremost, for many years, human operators were handling the recovery of their database clusters manually. However, human response time is neither consistent not reproducible, and thus it cannot be benchmarked;
    \item Second, availability benchmarks require fault injection at the level of infrastructure. Although it is easy to kill a database instance, it is much harder to simulate a network partition in a real infrastructure;

\end{itemize}




In this section, we propose two benchmark tiers to assess performance, predict the impact of change, or otherwise optimize storage systems. 


\subsection{Tier1 - Scalability}
Vertical scaling, which is also known as scaling up, means adding resources (e.g,CPU, memory, storage) to a single node in a system. However, software can be reached before hardware bottlenecks, thus making the system saturated without achieving full utilization of resources. For example, I/O delays can cause thread pools to be exhausted, block misalignments in the stack may cause high write/read amplification factors, or centralized logging may block the system due to lock contention. Additionally, there may be a really bad fit between what the software does and what the resource is optimal for, e.g, use btrees over SSDs. 

To support huge datasets and very high request rates, cloud systems are architected to scale-out, so that large scale is achieved using large numbers of commodity servers, each running copies of the database software. However, a light workload running on scaled-out system can be even slower than on a single machine due to communication overhead. But the problem with a scale-up approach is that the performance doesn’t grow in linearly proportional to cost. A system with better performance will achieve the desired latency and throughput with fewer servers.

The Scaling tier aims to identify this bottlenecks by keeping the workload steady, and measuring throughput as we assign more resources to the node (scale-up), or by adding new nodes (scale-out)  until performance stops increasing.


\subsection{Tier2 - Elasticity}


An effective elastic system must: ...



\subsection{Tier3 - Availability}



A cloud database must be highly available despite failures,and the Availability tier measures the impact of failures on the system and the whole datacenter. These failure may be the resultof hardware failure (for example, a faulty network interfacecard), power outage, software faults, and so on. A properavailability benchmark would cause (or simulate) a varietyof different faults and examine their impact.

The simplest way to measure availability is tostart a workload, kill a server while the workload is running,and observe any resulting errors and performance impact.However, in a real deployed system, a variety of failures canoccur at various other levels, including the disk, the network,

Availability refers to the percentage of time that the infrastructure, system or a solution remains operational under normal circumstances in order to serve its intended purpose. The measurement of Availability is driven by time loss. 

Example: storage systems serve multiple applications, meaning that outages affects many different applications. Especially for hybrid OLAP/OTLP systems. 


In [7], a hi

erarchical framework, named R3
, is
established to benchmark availability. R3 represents the
three system attributes that are key to availability
identified in the framework. These attributes are 




\subsubsection{Metrics}
\begin{itemize}
    
\end{itemize}

The framework
provides for a benchmark that incorporates all defined
attributes, thus yielding a downtime-per-year metric.

\subsubsection{Methodology}

\begin{itemize}
    \item I/O contention: Injects I/O delays in accessing block devices
    \item Individual server going offline
    \item Network partition (increased delay)
\end{itemize}


\subsection{Tier5 - Reliability}
Reliability is driven by the frequency and impact of failures. Reliability can be considered a subset of Availability. Mathematically, the Availability of a system can be treated as a function of its Reliability. 

Cloud systems use replication for both availability andperformance. Replicas can be used for failover, and to spreadout read load. Some systems are also designed to split writerequests across replicas to improve performance, althougha consistency mechanism (such as eventual consistency inCassandra, or timeline consistency in PNUTS) is needed toavoid corruption due to write-write conflicts

\subsubsection{Metrics}
\begin{itemize}
    \item Blast radius (number of affected clients, per node)
    \item Fault tolerance (how many failures, and mode of failures the system can sustains)
    \item Mean Time To Repair (MTTR) (how long it takes for system to detect and recover a failure)
\end{itemize}

\subsubsection{Methodology}

\begin{itemize}
    \item Time skew: Simulates clock skew of the container to be tested.
    \item Device Failure
\end{itemize}




\subsection{Tier6 - Collocation}

\subsubsection{Metrics}

\subsubsection{Methodology}




\subsection{Tier7 - Version drifting}

\subsubsection{Metrics}

\subsubsection{Methodology}
Backward/Forward compatibility (e.g. Structure fields changing, being added, removed)











\subsection{Tier2 - Simulate Failures}
\subsubsection{Infrastructure failures}
Single Node
\begin{itemize}
    \item Kill pod or application instance to simulate a crash 
\end{itemize}

\subsubsection{Network failures}

\paragraph{Network Partition}
A common use is to run a distributed application such as a database or cluster and create network partitions, then observe the behavior of the nodes. For example in a leader election system, you could partition the leader away from the other nodes and ensure that the leader steps down and that another node emerges as leader.

\begin{itemize}
    \item Inject communication delays to simulate degradation or outages in a network. 
    \item Limited bandwidth to simulated increased network load 
    \item Network break down to simulates network partitions
    \item Random Packet drops or disorder (Most-once)
    \item Packet duplicates (least-once)
    \item Zones of nodes going offline 
\end{itemize}    

\subsection{Tier3 - Application deficits}

\paragraph{Hotspots}
Distributed databases shard data across multiple machines. These databases can suffer from unpredictable performance and low utilization due to imbalanced load across the machines. Load skew occurs naturally in many workloads and causes CPU and I/O imbalance, which degrades overall throughput and response time. Current databases address skew by resharding data across machines but this operation is expensive because it involves bulk migration of data, which affects foreground operations. 

\paragraph{Impact of background tasks}
Distributed LSM-based databases face throughput and latency issues due to load imbalance across instances and interference from background tasks such as flushing, compaction,and data migration. Background operations therefore can cause significant I/O and CPU bursts, leading to severe latency spikes, especially for queries spanning multiple nodes such as range queries.

\paragraph{Load Tolerance}
Some failure modes are only visible when the ratio of failures to total requests in a system crosses certain thresholds. 

The load balancing and request routing for FIT-decorated requests were evenly spread throughout our production capacity. This allowed increased resource consumption to be absorbed by normal operating headroom, which failed to trigger circuit breakers. We call this sort of experiment a “diffuse” experiment. It’s fine for verifying the logical correctness of fallbacks, but not the characteristics of the system during failure at scale.












\subsubsection{Transient Clients}

\subsubsection{Load-balancing Servers}




Typically application designers must decide on an acceptable latency, and provision enough servers to achieve the desired throughput while preserving acceptable latency.

are critical thresholds that are crossed only when a large portion of requests are highly latent or failing. These points usually surface during periods of high usage or load. 
 
 
 
\paragraph{Distributed Concerns}
 In this case, we want to identify and dispose unused resources to avoid waste and clutter. Some examples:
\begin{itemize}
    \item 
    \item When a fallback is more computationally expensive than the happy path, CPU usage increases.
    \item 
    \item While aggressive retries occur, you may have a self-inflicted, denial-of-service attack.
    \item Instead of increasing traffic, we decrease resources assigned to the service.
\end{itemize}
 
 
 
 As the scale of a distributed system increases, it eventually reaches a point where single node benchmarks, even with hundreds of threads, cannot saturate the system. 





The Scale-up performance tier of the benchmark focuses on the latency of requests when a database is under load. There is an inherent tradeoff between latency and throughput. On a given hardware setup, as the amount of load increases, the latency of individual requests increases as well since there is more contention for disk, CPU, network, and so on. Typically application designers must decide on an acceptable latency, and provision enough servers to achieve the desired throughput while preserving acceptable latency. 

This tier aims to characterize this trade off by measuring latency as we increase throughput, until the point at which the database instance is saturated and throughput stops increasing.


Load balancers experience a high number of software faults

Failures potentially cause loss of a large number of smallpackets.By correlating network traffic with link failure events,we estimate the amount of packets and data lost during failures.We find that most failures lose a large number of packets rela-tive to the number of lost bytes (Section 5), likely due to loss ofprotocol-specific keep alive messages or ACKs.


Network redundancy helps, but it is not entirely effective.Ideally, network redundancy should completely mask all fail-ures from applications. However, we observe that network re-dundancy is only able to reduce the median impact of failures (interms of lost bytes or packets) by up to 40% (Section 5.1)


Network utilization.Figure 2 shows thedaily 95th percentile uti-lization as computed using five-minute traffic averages (in bytes)



However, Internet companies become more cost-sensitive, and people adopt less-reliable, commodity, or custom ordered hardware. In this context, software-based fault-tolerance systems began to flourish, and indulged operators to care less about hardware dependability. 


\subsubsection{Tier4 - Durability}



typically involving the addition of CPUs, memory, or storage devices to a more powerful single computer. 



\subsubsection{Metrics}

\begin{itemize}
    \item Tail-latency (client-side) per increasing resources
    \item QPS (server-side) per increasing resources
\end{itemize}

\begin{itemize}
    \item Tail-latency (client-side) per number of nodes
    \item Total number of clients (without degraded performance) per number of nodes
    \item Balance across servers (hotspots) and avoid bottlenecks
\end{itemize}

\subsubsection{Methodology}
\begin{itemize}
    \item Different combinations of CPU, Memory, IOPS
\end{itemize}


\subsubsection{Metrics}

\begin{itemize}
    \item Recovery time after server going online/offline
\end{itemize}

\subsubsection{Methodology}
\begin{itemize}
    \item Hard disks failing (or filling up)
\end{itemize}





\begin{itemize}
    \item Tail-latency (client)
    \item QPS (server)
    \item Utilization (server)
    \item Time to recover  This section considers the time to repair (or duration) for fail-ures, computed as the time between a down notification for a net-work element and when it is reported as being back online
    \item Time between failures
    \item Service downtime
\end{itemize}



Some of Cassandra’s strengths that influenced this decision include:

    High Availability – Cassandra is a distributed database where all nodes are equivalent (i.e. there is no master node so clients can connect to any available node). Data is replicated at a configurable number of nodes, so that failure of some number of nodes (depending on the replication factor) will not result in loss of data. From the CAP theorem perspective (Consistency, Availability, Partition tolerance), Cassandra’s design provides tunable consistency at the read/write request level, which allows you to increase availability at the expense of consistency where it makes sense.

    Scalability – Cassandra has been shown to be linearly scalable. Since each node adds processing power as well as data capacity, it is possible to scale incrementally to very large data volumes and high throughputs by simply adding new nodes to the cluster.


    Multi-datacenter replication – Cassandra’s node replication and eventual consistency features are core to the functioning of this distributed system. These features were designed from the outset and have been improved and battle tested throughout its lifetime and are now considered highly reliable. These features were therefore easily extended to clusters that contain nodes in different geographical locations, and due to the eventual consistency model this includes support for true Active-Active clusters. In fact, Cassandra has the reputation of having the most robust, reliable multi-datacenter replication of any datastore in the industry. This is an important part of our multi-datacenter failover capability at VictorOps and was one of the major factors in the decision to go with Cassandra.






these differences

obtained performance depends on the machines where the servers of the system are running. 


It is not uncommon to notice that published 

Another problem is to achieve repeatability when designers run our benchmark on their premises. This issue is referred to as the . Until now, this 

for researchers to publish 

running the server of the system under evaluation on a workstation, will produce significantly 

YCSB on a workstation will yield significantly different results from running the same benchmark on a , and even more 



running the benchmark across heterogeneous infrastructures



measures a repeatable set of quantifiable results that  against which products/services can be compared. The purpose of benchmark testing results is to compare the present and future software releases with their respective benchmarks.

Although it just provides a simple key-value API, you can build your own logic on top of it.

The faults used will often begeneric,  but  can  go  in  great  detail  if  the  faultload  designer knows the inner workings of  the  system. 
A benchmark must be repeatable. For instance, , if the response times varies too much, system performance be benchmarked. 




 This paper attempts to solidify the technical issues involved in the long-standing debate about the representativeness of fault injection as a tool for measuring the dependability of general-purpose software systems. 

  exceptional operating conditions external to a module under test in terms of exceptional system state, exceptional parameters/return values at an API, failed system components, or exceptional human interface inputs


In order for a benchmark to be effective the faultload must be 

What’s  Wrong  with  Fault  Injection  as  a  BenchmarkingTool?


 it  must  repre-sent real-world scenarios. [12] addresses the debate on fault-injection  representativeness.



In  order  for  the  faultload  to  be  effective,  it  must  repre-sent real-world scenarios. [12] addresses the debate on fault-injection  representativeness.  The  topic  is  whether  a  




 Hypothetical faultloads can stray from the system’sreal-world failure characteristics.  One  gray  area  tofaultload representativeness is the level of independency fromthe  system.  For  a  benchmark  to  be  used  universally,  thefaultload cannot be too overly detailed

 






can stray from the system’sreal-world failure characteristics. The faults used will often begeneric,  but  can  go  in  great  detail  if  the  faultload  designerknows  the  inner  workings  of  the  system.  One  gray  area  tofaultload representativeness is the level of independency fromthe  system.  For  a  benchmark  to  be  used  universally,  thefaultload cannot be too overly detailed.




 Compared to performance benchmarking, avail-ability  is  still  in  its  infancy.   

 Numerous  factors  have  to  be  taken  into  account,  and  there  is  adebate as to how to include these factors in the benchmark. Thispaper will give the reader a basic understanding of the concepts    with   availability,   some   of   the   current   availabilityrepresentations, and briefly discuss some current research beingdone  in  this  area.
 
 
 
 
host artifacts (e.g, garbage collection, bitrot scrubbing) and network artifacts (e.g, rebalance, replication, negotiations), 
It is therefore possible for specific behavior that happens during a test to be falsely attributed to another task started in the meantime. For example, a degraded replication performance may be attributed to network issues whereas the real reason is the garbage collection started on the remote host.




\CHECKnote{[FN] 

In our testing framework, we:

    Observe the normal metrics and develop our testing hypothesis.
    Inject a list of failures into TiDB.
    Run various test cases to verify TiDB in fault scenarios.
    Monitor and collect test results for analysis and diagnosis.

Even with Chaos Mesh helping to inject failures, the remaining work can still be demanding—not to mention the challenge of automating the pipeline to make the testing scalable and efficient.



The difference between testing is that expects a yes - no whereas a benchmark must converge

Write table-driven tests 

 They allow you to write unit tests in a concise fashion, hopefully leading to greater test coverage at a lower line count. If done correctly, adding additional test cases is as simple as a new element in the test table.

In this paper we present \name{}, 

In this paper, we advance the state-of-the-art by developing a 2-phased methodology that combines fault-injection and analytical modeling to study and quantify the performability - a metric combining performance and availability - of cluster-based servers. 

This is why we built , , in order to study the recovery mechanisms of various systems. Our frameworks 





We are using this framework to benchmark key/value databases in terms of  To do so, we propose a two-phase methodology. In the first phase, performance benchmarks hammer database servers with requests 


At a high level, these methods can be assessed through the principles of Chaos Engineering. The core idea is to provoke the emergence of unanticipated failures within a managed time-frame in order to initiate the recovery process. In general, Chaos methodology dictates to form a hypothesis about what will happen if a failure arises, and then design the smallest possible experiment to validate or falsify the hypothesis in the system. Chaos experiments consist of


However, comparing the recovery mechanisms of two architecturally different systems requires a benchmarking approach rather than a testing approach. Benchmarks are based on workloads and metrics that are well understood and representative across different systems. In contrast, the 


Moreover, the Chaos policies for fault injection is based on time (e.g, every minute, after 10 minutes, at 12.00am). As such, there are no guarantees that two systems will be in comparable states at the time of injection. For example, at 12.00am one system may be in replication mode while the other system remains idle. Thus the comparison will not be fair. Similarly, for a given point in time, there are no guarantees that the same system will be in an identical state amongst test iterations. This last property is essential for repeatability.








In the first phase of our methodology, the server is benchmarked for performance and availability both in the presence and absence of faults





  The framework consists of a workload gener-ating client and apackageof standard workloads that coverinteresting parts of the performance space (read-heavy work-loads, write-heavy workloads, scan workloads, etc.).


developing a 2-phased methodology 

analytical modeling  the performability - a metric combining performance and availability - of  servers. In the first phase of our methodology, the server is benchmarked for performance and availability both in the presence and absence of faults. To support systematic fault-injection, we introduce Mendosus, a fault-injection and network emulation infrastructure designed specifically to study cluster-based servers. While evaluators using our methodology are free to use any fault-injection framework, Mendosus provides significant flexibility in emulating different LAN configurations and is able to inject a wide variety of faults, including link, switch, disk, node, and process faults. 


Our goal to create a standard benchmark to assist in the evaluation of availability of different cloud systems. 

to build a full Chaos Engineering testing loop for TiDB, our distributed database.



We present theYahoo! Cloud Serving Benchmark(YCSB)framework.  An im-portant aspect of the YCSB framework is its extensibility:the workload generator makes it easy to define new work-load types, and it is also straightforward to adapt the clientto benchmark new data serving systems. The YCSB frame-work and workloads are available in open source so thatdevelopers can use it to evaluate systems, and contributenewworkload packagesthat model interesting applications1.In this paper, we describe the YCSB benchmark, and re-port performance results for four systems: Cassandra, HBase,PNUTS, and a simple sharded MySQL implementation. Al-though our focus in this paper is on performance and elas-ticity, the framework is intended to serve as a tool for evalu-ating other aspects of cloud systems such as availability andreplication, and we discuss approaches to extending it forthese purposes




Benchmarks are having trouble adapting to widely distributed servers, particularly those with extra sensitivity to network topologies. The emergence of grid computing, in particular, complicates benchmarking since some workloads are "grid friendly", while others are not.



\begin{enumerate*}
    \item a monitoring tool to observe system's behavior over time
    \item a time-framed failure injection into the system
    \item an operator to examine the behavior before, during, and after the failure, and juxtapose the hypothesis with what actually happened in the system.
\end{enumerate*}





 For  this  reason,  werun  regular  exercises  on  a  weekly  basis  that  test  AvailabilityZone  outages,  split  brain  situations  (data  replication  gettingqueued  up)  or  regional  outage  simulations.  

It can also be used to discover new, unknown failure modes. While these artificial failures are typically injected into production systems, they’re done so in a controlled, relatively safe way.



take humans out of the failure-recovery loop. 

Regardless the technology, all these system share the goals of 




The most obvious differences are between the various data redundancy models, such as the erasure coding model used in [DATABASE] and [DATABASES] versus the more simple replication model of [Database], or asynchronous replication model of [DATABASE]. However, the number and types of failures a system can tolerate can be documented and compared qualitatively. 



%Still, the availability model may differ significant: Active-Passive, Active-Active or Multi-Active. 








%Vendor benchmarks tend to ignore requirements for development, test, and disaster recovery computing capacity. Vendors only like to report what might be narrowly required for production capacity in order to make their initial acquisition price seem as low as possible.


Although time-based fault injection may help in assessing the resiliency and fault tolerance of the system at a point in time, it does not guarantee that at that point the . 

Additionally, decisions about data partitioning and placement may have an impact on failure rate and blast radius. Moreover, some systems are designed with native self-healing support, as happens with [TIKV, COCKROADDB], while others may depend on the infrastructure to provide this quality. MongoDB, for example, achieves self-healing by sharding data into replicated clusters of nodes managed by Kubernetes. 




As such, Chaos experiments fall short of benchmarking qualities such as standardization of workloads and metrics, fair comparison among systems, and repeatability of experiments. 

Even with Chaos suites helping to inject failures, the remaining work can still be demanding 



Chaos Engineering is a emerging disciplined approach to proactive  of faults  in order to validate a system's ability to resist interruptions. 


Chaos engineering can be used to achieve resilience against:

Infrastructure failures
Network failures
Application failure


Zenko is designed with auto-scaling, self-healing, infrastructure checks and data availability in mind:

Auto-scaling: to handle sudden surges of traffic which are common at Tier 1 network providers, we chose Kubernetes for its native auto-scaling feature;
Self-healing: thanks to Kubernetes again, any pod that disappears will immediately be respawned elsewhere; together with microservices replica sets and auto-balancing of services on nodes, Zenko’s deployments are very resilient, even with several nodes gone;
Infrastructure checks: thanks to MetalK8s, our optimize K8s distribution, Zenko will not be deployed on a shaky network or an insufficient number of nodes, providing automatic protection from Network Chaos Monkey;
Data availability: the main purpose of Zenko is to give you multi-cloud control, so when one of its providers is down, an application can seamlessly failover to another using the S3 API; a single namespace over all clouds, with aggregated metadata search and replication workflows across all of them can, when used wisely, provide unlimited service availability.
All of that allows Zenko to pass the Chaos Engineering test: its components probe the hardware, scale up or down automatically, self-heal,


}



This requires re-examining old system properties and considering new system properties, possibly leading to the re-design of classic benchmarking metrics such as expressing performance as throughput and latency (response time). In this work, we address these requirements by focusing on four system properties: (i) elasticity of the cloud service, to accommodate large variations in the amount of service requested, (ii) performance isolation between the tenants of shared cloud systems and resulting performance variability, (iii) availability of cloud services and systems, and (iv) the operational risk of running a production system in a cloud environment. Focusing on key metrics for each of these properties, we review the state-of-the-art, then select or propose new metrics together with measurement approaches. We see the presented metrics as a foundation toward upcoming, future industry-standard cloud benchmarks.










combine an expected fault model [23,32], measurements from the first phase, and parameters of the surrounding environment to predict performability. Designers can use this model to study the potential impact of different design decisions on the server's behavior. 


that combines . Some of the challenges towards such an automated framework include: 
\begin{enumerate}
    \item Creation and management of the distributed testing environment
    \item Definition of the steady states of the system, in absence of faults
    \item Failure injection according to a faultload (akin to workload)
    \item Continuous testing until the observed metrics are 
\end{enumerate}


with regard to the apparent failures rather than the faults that caused that failures.  



computer   systems   in   the   dimensions   ofavailability, data integrity, disaster recovery, and security.

   
Yet another challenge is about achieving portability 
This entails difficulties in fair comparison among systems and reproducibility of the experiments. Other than being relevant across systems, the benchmark should also portable across different experimentation platforms. Although different experimentation setups can be documented and compared qualitatively, it is much harder to achieve reproducibility since different platforms have different components and therefore unique failure modes.



Along with that, different systems may require different kind of metrics. 

that a fair comparison among systems is at risk. 

we need to define standardized classes of faults that produce comparable information about the overall status of cloud systems






These metrics may provide  and can further be used for managerial decisions by operators and stakeholders.

Defining 

simplify the comparison of self-healing systems by developing a


  
%Clearly, because of the variability in the , we need some stati

%To amortize the temporal uncertainty

%Theypropose the use of a methodology called randomized multiple interleaved trails (RMIT) in whichcompeting alternatives that are being compared are interleaved in a round robin fashion. 
commonly used approaches to conducting experiments in clouds 


Operational risk evaluates whether cloud services run in thesystem as expected and, if not, the severity of the deviations. Given that cloud users want theirapplications to run with minimum performance degradation, providers may use metrics such theoperational risk to publicly present the capabilities of their systems.





Besides fault injection, 
and  — 

injecting failures into the system, but they still solve only a fraction of the comparison puzzle. 


At a high level, performance benchmarks can be used to measure the overall impact of recovery process into the system. However, performance benchmark are  What they measure is the difference between the submission time of a request and the time the service acknowledge it. Performance benchmark can therefore measure the impact of recovery process as inferred from its interference with the common path of the service,  





s deriving from their performance levels when running in cloud infrastructures.



To do so, we adopt a two-phase methodology~\cite{10.5555/1251460.1251462}. In the first phase, the server performance is benchmarked both in the presence and absence of faults.  To support systematic fault-injection, we use Chaos Mesh, a Kubernetes-native platform for 
fault-injection at various levels, including the node, network, disk, operating system, and process faults. 







Failure modes are the ways in which a process can fail.

When a system has many potential ways of failing, it has multiple failure modes or competing risks. The more complex a system is, the more failure modes there are. For example, a home fire alarm can fail because of a dead or missing battery, faulty wiring, defective detector, or defective alarm. An aircraft could have many failure modes.


The specific manner or way by which a failure occurs in terms of failure of the part, component, function, equipment, subsystem, or system under investigation.





%In a nutshell, our proposed model:
%\begin{enumerate*}
    %\item is 
    %\item is applicable to every system
    %\item is 
    %\item implies an order of severity
    %\item have a direct relationship with failure detection, rectification, and %prevention mechanisms
    %\item capable of revealing the resilience strengths and weaknesses for every try-catchblock
%\end{enumerate*}


To compare the recovery mechanisms of two architecturally different systems, there 












%    Run for an infinite duration in order to introduce failure scenarios and test long running maintenances such as database repairs.
    %Provide pluggable patterns and loads.
    %Support different client APIs.
    %Deploy, manage and monitor multiple instances from a single entry point.
    %Support multiple cloud platform due to integration with Cloud Foundry









High availability is a requisite for today’s high-end systems where downtime can result in catastrophic losses. 


Storage benchmarking tools and methodologies today suffer from a glaring gap—they are incomplete because they omit availability operations. 



any minute of downtime may cause service level agreement (SLA) violations and severe loss of revenue.


selling point for emerging datastores. 

Regardless of how well a system is designed, or how reliable the components are, failures cannot be eliminated completely.  Despite the phethora of benchmarks performance and scalability benchmarks, there no benchmark for measuring the recoverability of a system. 




We find that .. 









This flexibility enables rapid prototyping ofhardware and software techniques for latency-critical workloads.

 






With more businesses depending on key/value services for their mission-critical data, any minute of downtime may cause . 




 These services must exhibit several characteristics, including high performance, scalability, and availability. The performance and scalability of cluster-based servers have been studied extensively in the literature, e.g., [2,5,7]. In contrast, understanding designs for availability, behavior during component faults, and the relationship between performance and availability of these servers have received much less attention.




Many self-healing systems are currently vying for the attention of Cloud providers and data companies. At a high level, these solutions aim 




Regardless of how well a system is designed, or how reliable the components are, failures cannot be eliminated completely. 




\CHECKnote{[FN] Examples of self-healing systems}

To make informed choices between competing solutions, and enable DevOps to evaluate and tune the performance of these complex ecosystems, appropriate metrics, benchmarking tools, fault-injection tools, and methodologies are necessary. 











In our \name{} work, we focus on the recovery attribute. We consider the fact sustainability and predictability of performance are essential properties in mission-critical computing. It is therefore essential for a system not only to tolerate failures, but also to recover well and quickly after a system fault. It’s the difference between minimal downtime and significant downtime resulting in service level agreement (SLA) violations and severe loss of revenue~\cite{10.5555/1050517.1050538}. Our focus is on self-healing data stores whose remediation mechanisms tend to execute the same sequence of steps and are thus both consistent and measurable. 










An example of a chaos engineering system is Netflix ChaosMonkey, which randomly shuts down servers to make sure that the overall system is capable of spawning new ones automatically.


Decisive to this trend is the upraise of : a new scientific within software engineering that consists in specifying and evaluating resilience hypotheses by 1) injecting faults in a production system, 2) observing the impact of such faults, and 3) building new knowledge about the strengths and weaknesses of the resilience of  the system. 
 







Perhaps the greatest turnout 


%Additionally, since it is very challenging to reproduce the complexity and the scale of production environments in a staging environment, Chaos experiments are usually run in production.



 This standardization can only be achieved through an agreement (explicit or tacit) from the computer industry and/or by the user community. However, the contribution of the research community is essential to show possible solutions for the complex technical problems posed by robustness and recovery benchmarking.


there is no widely accepted 

 in the literature, e.g., [2,5,7]. In contrast, understanding designs for availability, behavior during component faults, and the relationship between performance and availability of these servers have received much less attention.



In contrast, understanding designs for availability, behavior during component faults, and the relationship between performance and 



Along with that, it is interesting 

Availability is a number that can help assessing the probability of receiving service when requested. For example, a system with 99.999\% availability will be inaccessible for at most 315 seconds per year. In general, availability comprises 










failure patterns observed in their data centers. Nevertheless, there is no industry-wide . This is reasonable since different infrastructures have different hardware, different environmental factors, different operational loads, and therefore different, unique failure patterns. 





or more precisely the number of failures occurring in a system over a given time interval.


is to , and eventually gain confidence that 





A significant benefit of analyzing recovery is that it can help system operators to strike the right balance among system availability, hardware reliability, and operating costs, reducing the total cost of ownership (TCO) in data centers. Additionally,




 


\CHECKnote{[MM] Consider moving the following 2 paragraphs to Introduction. Also consider omitting the paragraphs above (keep only citations?) }





%Control operations are an essentialpart of the cloud native storage workflow and are becoming in-creasingly more frequent as regular, non-privileged users are ableto issue control operations without involving a storage adminis-trator. 





%Reliability is only one of many factors that influences availability, for example,99.99% reliability does not mean 99.99% availability. Reliability measures the ability of a system to function without interruptions, while availability measures the ability of a system to provide a specified application service level to clients. Therefore,, while availabilityi ncludes the effects of downtime any failures produce

%Systems recovery and contingency planning is the series of processes



The key aspect that distinguishes benchmarking from testing is the standard nature . In contrast, 



The scenario we study is , and includes a temporally overloaded node and a subsequent restart of the node.  Iperf 

network failure with a subsequent restart

, in presence of a network failure and subsequent.

Resiliency revolves around creating a structure that can withstand or prevent loss of services due to an unplanned event. Disaster 

  Along with the results,  incorporates a conceptual recovery analysis as proposed in . Other than showing the practically of \name{}, the significant differences between the two patterns also underline the necessity to embody failure injection in next generation benchmarks. 


\CHECKnote{[FN] Continue to explain the graphs}



However, the outage experienced by the crashed node is temporal and can be addressed within seconds, whereas a network partition can be regarded as a permanent failure (with respect to experimental time scale). 



For example, Cassandra’s eventually consistent data model ensures that upon a split-brain scenario, network partitioned data service will continues to run storing and accessing data, albeit without having access to the full cluster. In this view, 


a crashed node will always cause disruptions to the connected users, while 

For example, 

and node repair features ensure that the consistency of the cluster will be automatically maintained over time.

%“Self-healing” –  This also makes it very easy to recover failed nodes, increase or decrease the size of the cluster as needed, and even do in place version upgrades (in most cases).




%Third, network errors do not al-ways impact network traffic or service availability, due to several factors such as in-built redundancy at network, data, and application layers. 
%The proposed  seeks to enable comparison in the dimensions of 

Thus, all failures affect the state of the system, but not all failure should be interpreted as . 








%Synthetic benchmarks do this by specially created programs that impose the workload on the component. Application benchmarks run real-world programs on the system. While application benchmarks usually give a much better measure of real-world performance on a given system, synthetic benchmarks are useful for testing individual components, like a hard disk or networking device. 

% On the client-side, testing frameworks like fio gives the user the ability to freely experiment with arbitrary I/O workloads, without having to write tailored tests again and again. The need to compare architecturally different systems with respect to a standard workload has motivated academia and industry to develop several 

%In our SRB work, we focus on the recovery attribute. We consider the fact that

 In general, availability is defined as a function of three key attributes~\cite{10.5555/1698155}: rate, robustness, recovery. 

Rate describes the frequency of failures. However, despite the numerous failure patterns identified in large data centers~\cite{8023108, oppenheimer2003internet, barroso2009datacenter, govindan2016evolve}, the definition of a widely accepted failure pattern remains an open challenge. This is due to the fact different infrastructures have different resources and therefore different, unique failure modes.

\subsection{Chaos Ecosystem}

Robustness represents the degree at which a failing component will not disrupt the entire system. 


Without realistic failure patterns to indicate `how often to fail', Netflix concluded that `the best defense against major unexpected failures is to fail often'~\cite{chang2015chaos, allspaw2012fault, zhang2019chaos}. In turn, this mindset led to concept to 


Moreover, because all the containers in the experiment share the same system clock, we can objectively measure the elapsed time between a client sending a message and until another client receives it. This measurement is impossible to achieve in a distributed deployment due to the clock skewing.


We believe that in the attempts to define ‘physical resilience’ it is essential to distinguish between the ability to resist deviation from the original state (‘robustness’) from the ability to recover after such deviation (‘resilience’ per se). This is because changes in robustness and resilience during aging may potentially differentially impact health and longevity. E.g., a universal feature of biological aging – the slowdown of metabolic, proliferative, information processing and other responses to stimuli - may improve robustness in relation to some health disorders (e.g., cancer) by reducing their risks, but may make worse regenerative response to damage and through this reduce resilience and contribute to physical senescence and increase in vulnerability to death in the very old. 


To do so, they need a near replica of a production environment to test codes, and 





distributed modelling these scenarios
for the emulation of computing paradigms (e.g., IoT, Edge,  Fog)

, and because modern applications have evolved, exhibiting higher density, diversity, dynamicity, and specialization than before. These factors can directly impact the performance of dependent applications and indirectly influence the I/O of collocated applications. 



Identifying these anomalies in in the earlier stages of the software lifecycle is critically helpful for developers and operators. While building testing environments works fine for small-scale experiments, 






Unlike existing approaches, Frisbee  The Frisbee runtime acts as a coordinator between the modeled environment and the containerized applications running on Kubernetes.  



Although the relevance of testing environments has escalated in recent years, existing solutions face significant challenges in expressing complex topologies and dynamic workflows.



In this way, SentiLog learns information embedded by developers from the source code. Our preliminary results show SentiLog is able to accurately predict anomalies and performs better than state-of-the-art log analysis solutions on two representative PFSes (Lustre and BeeGFS). This preliminary study shows sentiment analysis could be a promising method to analyze complex and irregular system logs.

placement constraints,  logical dependencies between components,  

analyzing PFSes system logs for detecting anomalies. Unlike existing solutions, SentiLog works by training a general sentimental, natural language model based on the logging-relevant source code collected from a set of PFSes. 


larger deployments faces significant challenges due to the large design space and irregularity of PFSes logs.

it isn't powerful enough to handle . 


However, applying them to parallel file systems logs faces significant challenges due to the large volume and irregularity of PFSes logs.

Until today, systems testing remains a manual process at both deployment and analysis levels. 


However, applying them to parallel file systems logs 

This is fine for smaller problems, but 


Kubernetes opens up new horizons  This paper presents a Frisbee-- a Kubernetes-based platform for . Frisbee consists of two main components. First, a language for expressing complex setups, dynamically changing request patterns and failures, logical any physical grouping, scheduling constraints, and dependent executions. 


%

%Analyzing the runtime logs to detect the anomalies of large-scale systems has been proven effective in many recent studies. However, applying them to parallel file systems logs faces significant challenges due to the large volume and irregularity of PFSes logs. 















Disaster recovery

Disaster recovery is the process of getting IT services back online after a failure or outage. These scenarios can be caused by anything from a natural disaster, global pandemic or a cyberattack. Getting back online can be a largely manual process that requires a high level of human orchestration. Disaster recovery has long been the way most banks deal with major system outages. However, recently, there has been a significant shift towards focusing on resilience rather than recovery.
IT resilience



\CHECKnote{[MM] ("chicken or egg" question) Is Kubernetes a solution for the Portability challenge, or is this work focused on containerized environments? }





\subsection{Portability}

We investigate near-optimal load balancing and auto-scaling solutions that can get the best delay performance while attaining high utilization in two-tier cloud storage systems. The first tier consists of a distributed cache composed of leased resources from a computing cloud (e.g., Amazon EC2) and the second tier consists of a persistent distributed storage (e.g., Amazon S3). At any point in time our solutions dynamically determine how many cache servers should be active as the incoming load, object popularities, and service rate of persistent storage are subject to change. We first present a load balancing solution for a given set of cache servers that can evenly distribute the load against workloads with an unknown Zipf distribution while keeping the overall cache hit ratios close to the maximum. Building on this load balancer, we then present our auto-scaling solution that uses the request backlogs in the caching tier to determine the number of active cache servers to be used in the next epoch. Via simulations, we show that the end-to-end design is quite effective in converging to the right amount of service capacity against the system dynamics.



In a growing number of domains, the provisioning of end-to-end services to the users depends on the proper interoperation of multiple systems, forming a new distributed system, often subject to timing constraints. To ensure interoperability and integrity, it is important to conduct integration tests that verify the interactions with the environment and between the system components in key scenarios. To tackle test automation challenges, we propose algorithms for decentralized conformance checking and test input generation, and for checking and enforcing the conditions (local observability and controllability) that allow decentralized test execution.











 interacts with 
to push annotations that provide . Thus, \frisbee{} users can reason about the performance and  

A report includes the test result and supplementary information for debugging, such as logs.


Examples of infrastructure metrics include CPU time, memory usage, heap usage, garbage collection, etc. Application-specific key performance indicators such as request/sec, latency, and request duration.

 is an example of an exporter that publishes hardware and OS metrics exposed by *NIX (UNIX, Linux, etc.) kernels. 

Report generation. 




In general, :
\begin{enumerate}[label=(\roman*)]
    \item Test configuration. The tester decides which scenarios to run, testing environments, and parameters.
    \item Environment preparation. The framework deploys the application and the test data on the target environments.
    \item Execution. The framework executes the tested application according to a predefined scenario; the test checks assertions about the application's state
    \item Report generation. A report includes the test result and supplementary information for debugging, such as logs.
    \item Clean up. The framework deletes generated artifacts from remote hosts.
\end{enumerate}











%As more and more companies are migrating (or planning to migrate) from on-premise to cloud, their focus is to design, architect, and build applications that can be easily scaled, deployed to the cloud and have the abilities to utilize the advantages of the computing models provided completely 

%Each microservice is designed to accomplish a single type of task, and is usually housed in containers. In order to execute its function, one service might need to request data from several other services inside the network. These characteristics enable a faster release, testing, and maintenance pace, compared to monolithic applications. 


%cannot be easily generalized to other experiments. 

%potentially use Argo workflows with  and bind their lifecycle with external scripts that invoke an . However, these 

%Therefore, it is necessary to come up with solutions that step beyond manual processes that , and come up with generilized





%It builds upon the basic Kubernetes resource and controller concepts, but includes domain or application-specific knowledge to 

%allowing you to think about your infrastructure in abstract terms, e



%The Operator pattern aims to capture the key aim of a human operator who is managing a service or set of services. Human operators who look after specific applications and services have deep knowledge of how the system ought to behave, how to deploy it, and how to react if there are problems.

%Thinking experiments in terms of a graph abstracts away the code details,

%For example, benchmarking a Key/value store consists of at least three steps: (i) deploy the servers, (ii) start ingesting keys only after all the servers are up and running (iii) run queries only after the key ingestion is complete. 

%Black-box testing is a high level of testing that involves testing from an external or end-user perspective. Grey-box testing is less intrusive and proves most useful at the integration testing level, such as when YCSB benchmark~\cite{cooper2010benchmarking} to validate the system's performance and .

%This convenience also facilitates the validation of research articles. ~\cite{tsai1996approach, wilson2002progress}. It is not uncommon to spot two different papers in the literature whose authors use the same benchmark, the same deployment, and yet find that the published result variate significantly~\cite{leitner2016patterns,schad2010runtime}. In our approach, the experimental workflow and the execution environment is documented in code, thus making it easy to reproduce the experiment across different infrastructures. 



%To ensure that the chances of these happening in the production is less or the impact is minimal, we have to 



 

%Any issue or deviation from the expected behavior in terms of these points need to be detected, debugged, and fixed as soon as possible with minimal effort and steps need to be taken so that those don't happen again.


%. Using , designers have modern ways to answer 

%For monolithic applications, most of the potential failure modes are known, can be identified, and thus can be handled in the code constructs. Yet, regression testing pipelines can ensure that these bugs will not appear again.



%perform experiments for testing the product performance (e.g., latency, effect of load-balancing/caching), comparing resiliency algorithms and recovery approaches after a failure, as well as evaluate the right deployment models and choose the best option that aligns well with their business goals. 

%That involves, trigger long-running maintenance jobs that may affect the performance, simulate adverse conditions like network partition that can bring the system to a halt, or artificial hardware constraints that can uncover long-term issues like memory leaks or heap pressure. 

%ut us complex to setup/execute


%Moreover, developers need to validate the effects of various actions throughout the experiment, in order to conclude whether the system behaves as expected to meet the business goals.





\subsection{Resource Throttling}
First, we validate the mechanisms for throttling memory, CPU, and disk I/O.

\begin{figure}[tbp]
    \centering
    \includegraphics[page=1, width=\columnwidth]{images/plots/cpu.pdf}
    \caption{CPU LZMA compression benchmarks.}
    \label{eval:resource:cpu}
\end{figure}

\paragraph{Memory \& CPU Performance}
To validate memory throttling, we develop a micro-benchmark that allocates chunks of 4MB at a time, until an out-of-memory (OOM) error occurs. Our metric is the size of the allocated memory until the error is thrown. For the validation of CPU, we use the 7~Zip Compression benchmark~\cite{p7zip}. As shown in Figure~\ref{eval:resource:cpu}, we perform multiple tests, and at each iteration, we change the number of virtual CPU cores allocated to the container. We measure the reported CPU usage during the tests, both from the perspective of the throttled container and the host. 


\begin{figure}[tbp]
    \centering
    \includegraphics[page=1, width=\columnwidth]{images/plots/fio.pdf}

    \begin{adjustbox}{max width=\columnwidth}    
    \begin{tabular}{c c c c c} 
    \hline
 Storage Profile & Seq.Read & Seq.Write & Rand.Read & Rand.Writer \\ [0.5ex] 
 \hline\hline
 SSD M.2 & 2 GB/s & 700 MB/s & 170K IOPS & 130K IOPS \\ 
 UFS 2.1 & 880 MB/s & 200 MB/s & 40K IOPS & 40K IOPS \\ [1ex] 
    \hline
    \end{tabular}     
    \end{adjustbox}

    \caption{fio benchmarks on emulated devices.}
    \label{eval:resource:disk}
\end{figure}

\paragraph{Disk I/O Performance}
For the I/O validation, we use the fio~\cite{axboe2014fio} benchmark to report sequential reads, sequential writes, random reads, and random writes. As a reference for the throttling parameters, we use the specification of UFS 2.1 and SSD M.2. The results and the disk specifications are shown in Figure~\ref{eval:resource:disk}. For sequential reads and writes, the results are straightforward. For example, throttling of 700 MB/s sequential writes will yield 734 MB/s throughput performance. The difference is less than 5\%. Understanding random reads and writes is a bit more complicated. Because random operations are defined in terms of I/O per second, the resulting throughput depends on the request size. In our measurements, we use the default 4K per request. For example, for the random reads of UFS, we would expect 160 MB/s, and the observed throughput is 164 MB/s, which is marginal. The only case that throttling does not meet the specified throttling parameters is in random writes for the SSD. This is because the expected throughput (170K * 4K = 520 MB/s) exceeds the raw performance of the virtual disk we used. 


\begin{figure}[tbp]
    \centering
    \includegraphics[page=1, width=\columnwidth]{images/plots/links/theoretical.pdf}
    \caption{iperf benchmarks on emulated network protocols.}
    \label{eval:resource:network}
\end{figure}

\paragraph{Network I/O Performance}
For the network baselines, we use containers running the iperf benchmark~\cite{tirumala1999iperf}, in a server-client architecture. We run multiple tests, and in each test, we evaluate a different profile of Figure~\ref{eval:resource:network}, for a different number of clients. The CPU, memory, and storage resources remain unthrottled, aiming to saturate the network in order to observe artifacts in bandwidth sharing. 












System Testing is carried out on the whole system in the context of either system requirement specifications or functional requirement specifications or in contest of both.






We believe that the systems community can benefit from \frisbee{} in many different ways. Firstly,  Third, the standardization of the execution environment would help experimenting with prescribed fault models to compare the continuity of different systems in the presence of failures. 

Second, experiments on distributed systems rarely involve individual services. Most commonly they involve groups of . These groups are commonly associated with ; and resource constraints. Yet, these groups 

As such, we need adequate primitives for the implementation of logical groups. That includes 1) reusable service templates, such as ; 2) 


Review the requirements you'll be using end-to-end testing to validate. Set up the test environments and outline the hardware /software requirements. Define all the processes of your systems and its integrated subsystems. Describe the roles and responsibilities for each system.

    
The engine consists of a controller, sidecars that are deployed , and existing open-source software, such as Prometheus~\cite{prometheus} and Grafana~\cite{grafana} for

% No need to write language specific testing frameworks
% Out-of-the-box monitoring Remove layers 



















The key performance indicators (KPIs) to be measured might vary based on the hypothesis. Some of the key measurements include, 

The blast radius needs to be carefully assessed and planned responsibly in an incremental way considering the risk of bringing down the production system leading to customer impact. 










validate the system via test cases

Even if Kubernetes extensions exist to address some missing features, combining them into an experiment requires significant domain-specific knowledge and can be time-consuming. For example, , is a Chaos Engineering tool that injects numerous faults into a , but 












an experiment typically consists of numerous services that perform a certain function as a logical group. For example, a group of 10 YCSB clients that

which are neither identical nor entirely different. For example, 

being able to reduce the number of cross-references in a graph has implications on the modeling and reasoning of an experiment. To achieve that, 

Doing so, minimize the exposure to cross-references, 

Motivated by the fact that experiments can be described as flow of actions, 

at, we replace the concept of 

 

By replacing the concept of individual services with 

 It is therefore necessary 
 


During our experiments we realized that exposing individual services to the end-user can only 

designing graphs at the granularity of services 

By bloating the graph with , 


track the performed functions in an experiment 

expansion of the Hypergiants inside other networks,

experiments are commonly designed at the level of individual services. These services, however, are not 

 especially eyeball networks, has implications on the modeling of Internet
structure and Internet traffic flow. 


This view challenges the research
community’s mental model of the value of peering and exchanged
traffic between networks and can impact the scope and consid-
erations of net neutrality regulation. It has also implications on
network performance, as crossing network boundaries comes at
a cost [28, 44, 69]. Moreover, operating servers within a network
improves the strategic position of Hypergiants as they are able to
control both the origin server within their network as well as the
servers within other networks and, thus, optimize content deliv-
ery to end users

 to form a group

the design of experiments can bloated by the scale of services. 


These patterns, however, are .




And then, there is the need to gather the results by retrieving the different metrics files (through FTP or NFS) and then perform statistical tests that they save by hand.

Besides that, 




In turn, these decisions require developers to distinguish expected from unexpected failures. For example, they have to distinguish broken connectivity caused by an injected partition fault from broken connectivity caused by a blocking service. The first is an expected effect of the experimenting workflow. The second is an unexpected effect potentially caused by a bug in the service.






\paragraph{Runtime Engine} 




\paragraph{Evaluation}
A methodology for the systematic evaluation of K/V stores under dynamically changing workloads, maintenance / failures operations, and placement / capacity constraints. 
Using Redis as a reference implementation, we consider the following scenarios:
\begin{enumerate*}[(a)]
    \item \textbf{load performance:} measure fluctuations in presence of dynamic workloads.
    \item \textbf{recovery performance:} effectiveness in failover activities upon a network partition.
    \item \textbf{Scalability:} measure rebalancing when new servers are added
    \item \textbf{Elasticity:} extends scalability with graceful termination of nodes.
    \item \textbf{Killing:} Like elasticity with ungraceful termination of nodes.
\end{enumerate*}
















 and choosing from a vast ecosystem of Kubernetes extensions, \frisbee{} provides a unified framework for researchers  



\paragraph{Dependent Deployment Primitives}
A consolidated language that consists of templates and execution workflows. Templates 

Unlike exist-
ing frameworks where multiple failures are only exer-
cised randomly [6, 35, 38], FATE is designed to systemat-
ically push cloud systems into many possible failure sce-
narios.

which renders testing and validation a very hard task to accomplish. It becomes 





its extensible design allows operators to create custom \faultload{}s and understand how a system would behave if deployed on various real-world environments (e.g., IoT, Edge, Cloud).


its automation pipelines would help researchers study what-if scenarios and choose the most appropriate algorithms while developing new systems or resiliency mechanisms. 


Although developers may partially address these limitations by combining various third-party extensions, their interconnection 

The configuration and installation process itself needs to ensure that logical dependencies are respected, and the interoperability of system components is thoroughly tested. This must be done for every different experiment. 


case runtime uncertainties (e.g.,  for adjustable workloads), infrastructure failures (e.g., simulation of network partition).  

 components for 

conducting experiments on distributed applications on top of Kubernetes. 

 Additionally,
our approach is amenable to using existing public datasets, enabling
us to apply it in a longitudinal study uncovering the growth in off-
net deployments

% Approach
In this paper, we introduce 



As such, it lacks  that makes the workflow to perform an experiment costly and precarious. For example, it lacks primitives for expressing dynamically changing request patterns and failures,  scheduling constraints, and irregularity of collected metrics.


Therefore, it lacks primitives for defining 


dynamically  and failures, logical and physical dependencies between groups of components, scheduled executions, or irregularity of collected metrics.






\paragraph{Declarative Experimenting Workflow}



























\frisbee{} provide a fundamentally different approach to running experiments. 


























 This provides a self-healing mechanism to address machine failure or maintenance.


testing such a system is a hard and repetitive task but nevertheless crucial for development.

 

Even so, , which makes it difficult to consistently repeat the exact same actions in order to debug a problem that might emerge in the system. 




Additionally, that requires intermixing configurations from multiple extensions, making it difficult to understand the relation between the most critical components and how they fit together. 

\paragraph{Challenges in running distributed experiments}






























\paragraph{Reproduce an experiment}
The portability of experiments~\cite{tsai1996approach, wilson2002progress} is another critical topic that until now remains largely overlooked. It is not uncommon to spot two different papers in the literature whose authors use the same benchmark, the same deployment, and yet find that the published result variate significantly~\cite{leitner2016patterns,schad2010runtime}. The reason is that practitioners tend to drive experiments on different environments (at the hardware level: x86/arm/…, CPU frequency, available memory, or at the software level: operating system, versions of libraries). Although the experimentation platforms can be documented and compared qualitatively, it is much harder to accurate reproduce an experiment across different infrastructures. 








\paragraph{Design an experiment}





\paragraph{Deploy an experiment}






%And then, there is the need to clean-up the experiment and revert any modified state on the host (e.g, iptables tampered for the simulation of network partition faults). 





Start everything together -- no notion of time.









 Once there is a running Kubernetes cluster, engineers can deploy their containerized applications on top of it. 




To do so, they create a Kubernetes Deployment configuration. The Deployment instructs Kubernetes how to create and update instances of your application. O

nce you've created a Deployment, the Kubernetes control plane schedules the application instances included in that Deployment to run on individual Nodes in the cluster.





The lack of these primitives makes it challenging to design experiments that go through multiple dependent phases.



 




and irregularity of collected metrics.


\paragraph{Design the experiment}

* Workflows



These experiments may involve deployment parameters (e.g, placement policies), integration with performance (CITE YCSB) and correctness benchmarks (CITEJepsen), or 




event-based architecture
triggers by lifecycle or performance thresholds

\paragraph{Testing Scale}

\paragraph{Portability of Experiments}



 \& Testing scale

The reason typically has to do with the experimentation platforms they use. Since important decisions depend on reliable experimental data, it is necessary to enable reproducible experiments and verifiable results.




\paragraph{Experiment specification}




















Our contributions are:

* We developed the first framework for describing experiments in Kubernetes

* We applied it to study Redis

* We found that ...




\paragraph{Deployment Abstractions}

\paragraph{Workflow Specification}

\paragraph{Declarative Testing Specification}

\paragraph{Runtime}

https://www.usenix.org/legacy/events/nsdi11/tech/nsdi11_proceedings.pdf#page=249
https://dsf.berkeley.edu/papers/dbtest12-bloom.pdf
\paragraph{Insights on systems}
 design, deployment, and evaluation



This view puts \frisbee{} in a unique position, , but also to 



where system designers can explore numerous
conditions and parameters through 



\paragraph{Failure testing}
Unlike existing frameworks where multiple failures are only exer-
cised randomly [6, 35, 38], FATE is designed to systemat-
ically push cloud systems into many possible failure sce-
narios. FATE achieves this by employing failure IDs as a
new abstractionforexploringfailures. Using failureIDs,
FATE has exercised over 40,000 unique failure scenarios,
and uncovers a new challenge: the exponential explosion
of multiple failures. We do so by introducing novel pri-
oritization strategies that explore non-similar failure sce-
narios first. This approach allows developers to explore
distinct recovery behaviors an order of magnitude faster
compared to a brute-force approach.

The main contributions of \frisbee{} are:
\paragraph{Language Specification} 




%\item A \textbf{Community Hub} for sharing topologies, testing plans, and results. 


%Creating a real kubernetes cluster requires having multiple machines either on premise or on a cloud platform. This is
%not always convenient if someone is just new to Kubernetes and trying to learn by playing around with Kubernetes.
%MicroK8s is a CNCF certified upstream Kubernetes deployment that runs entirely on your workstation or edge device.
%MicroK8s initially was built for offline development, prototyping, and testing of Kubernetes apps on a desktop before
%deployment to the cloud. One reason for MicroK8s’ facility at the edge is its ability to be delivered as a
%container-like snap — app packages for desktop, cloud, and IoT that are easy to install and
%secure with auto-updates — and installed on any one of the 42 Linux distributions that support snaps. This makes
%MicroK8s ideal for running on the vast variety of hardware that comprises the IoT.

%For those that don’t know, the TPM is a highly secure and sophisticated piece of hardware that has numerous tamper detections and protections in place. Attacking the TPM directly is very unlikely to bear fruit within the timeframe of testing. As a result, we must look at the trust relationships around the TPM and what it relies on. It is a distinct and separate chip from other components on the motherboard and may be susceptible to a variety of attacks. Our particular TPM in question is shown here:




%Additionally, that requires intermixing configurations from multiple extensions, making it difficult to understand the relation between the most critical components and how they fit together. 

%Moreover, there is no easy way to prevent anyone from over-utilizing the shared resources in multi-system configurations with shared channels, control units, or devices. 




%Service distribution makes system design, deployment, and evaluation a complicated and costly endeavor for researchers and engineers. 



%\frisbee{} allows users to 









%Beyond expressing experimental workflows, \frisbee{} integrates capabilities for throttling of computing and network resources, out-of-the-box monitoring of distributed applications and resources, and constrained-based placement of services. 



% Helm Charts are useful for addressing the complexities of installation and simple upgrades of particularly stateless applications like web apps. However when it comes to stateful applications there is more to the upgrade process than upgrading the application itself. If you have ever tried to upgrade a PostgreSQL database before, you know that upgrading PostgreSQL itself is the least of the problems. Dealing with the schema changes between database versions is where the main complexity lies, which often requires dumping the data and re-importing it back to the new version of the database in a controlled manner so that client applications aren’t affected. Therefore, Helm Charts often are insufficient for upgrading stateful applications and services (e.g. PostgreSQL or Elasticsearch) which require a complex and controlled upgrade processes beyond upgrading the application version. 




%Most cloud infrastructures that existed before Kubernetes provided a procedural approach (individual steps are defined, then automated) for automating deployment activities. By contrast, Kubernetes uses a declarative approach (only the end goal is defined) to describe the system’s desired state.

%Although similar systems exist, they do not delve further into protocol details,
%specific to the system under test. It is desirable to have the ability to trace
%messages between nodes that make part of the cloud system, for instance. This
%becomes an issue, due to the ideally platform independent nature of the testing
%framework


% This thesis’ contributions have brought us to a step closer into solving the problem
%mentioned above, through the development of a testing framework that is
%• generic enough to be adapted to various cloud data storage systems,
%• complete enough to comprise methods, techniques and algorithms that
%allow consistent and meaningful testing of such a system, and
%• scalable enough to be able to stress a heavy load handling system like a
%cloud storage system.
%The framework is autonomous and can be interacted with either through a
%command line or web interface – more details on the framework can be found in
%Section 3.1. It is ultimately a collection of software modules that are executed
%simultaneously and, through synchronization, manage to interpret and execute
%tests, which are described in Section 3.2


However, testing distributed systems can be tedious. 


which renders testing and validation a very hard task to accomplish.


It becomes 




Moreover, in multi-system configurations with shared channels, control units, or devices, there is no easy way to prevent anyone from accessing the shared resources, 













It also possible for the alternative infrastructure configurations to lead into invalid conclusions and unfair comparisons.







the rectification of faults becomes a burdensome, labor-intensive, and error-prone task. 



Identifying these anomalies in the earlier stages of the software lifecycle is critically helpful for developers to scrutinize the quality of a product before the actual deployment. 




However, research in this area is hampered by the lack of suitable tools that can 




















  after a major code change
  
  remediation techniques (e.g. reactive vs. preventive), identify suboptimal (i.e. less effective) approaches, and compare the recoverability of different systems in the presence of failures
  
  
  
  
  
  
  
  
  
  
  
  
  
 
system designers can assess distinct system characteristics such as 



The reason is that practitioners tend to drive experiments on different environments (at the hardware level: x86/arm/…, CPU frequency, available memory, or the software level: operating system, versions of libraries). Although the experimentation platforms can be documented and compared qualitatively, it is much harder with traditional methods to 














%by studying the Redis key/value store beyond its sweet spot. We consider dynamically changing request patterns, 


%However, Kubernetes lacks several features required for realistic experiments. 

%automated failover, homogeneous versus heterogeneous replication, and effects of tiered placement. We find that Frisbee minimizes human error, and makes regression testing easier, while leading to more concrete conclusions than traditional testing. 




Another important concern is that Kubernetes lacks monitoring capabilities. Although aggregated throughput can reveal baseline performance characteristics, mixed workloads often exhibit artifacts such as various types of operations, operation errors, and other "hiccups" that aggregated values tend to hide. Without monitoring granularity, engineers lack the insights to understand what is actually happening. 
%Kubernetes has a steep learning curve, and an static configuration systems that 
%interconnecting these extensions results in overly complicated deployments 


% Impact
Second, it would allow to perform mutation testing on configurations, to gain a more profound knowledge of what configurations would optimize the target objective (e.g., fast-access, storage efficiency, availability, or cost reduction) on adverse environments (e.g., IoT, Edge, Cloud). 

distills the requirements of an experimental platform and i

 based on the users' current requirements and preferences
 
 
 

Generally, the Kubernetes scheduler will automatically do a reasonable placement, such as spreading containers across physical nodes, so as not to place the container on a node with insufficient free resources. 

Despite the lower performance (compared to a physical deployment), a local deployment would still allow for interoperability testing and semantics validation of IoT services. 




We detected unusual behaviors and identified critical aspects that need improvement. Given that, we foresee that virtual testbeds like \name{} 




You can use different classifications of availabilities to present different conclusions about your system's availability. The difference can be potentially large and availability measurements can be misused or misleading to your company and your customers. If you use a different classification from the one your customer uses, you and your customer could have very different impressions of the system. Therefore, the choice of availability classification to use should be made carefully, taking into account your system and industry and how your company and your customers perceive availabil








We found that \frisbee{} effectively reduces the effort and time of running distributed tests while leading to more concrete conclusions than traditional testing.



 
and other "hiccups" 

Second, it would allow to perform mutation testing on configurations, to gain a more profound knowledge of 



for understanding how an application would behave if deployed in geographically distributed environments, such as Fog, Edge, and IoT computing.

Although aggregated throughput can reveal baseline performance characteristics, mixed workloads often exhibit artifacts 

\frisbee{} effectively reduces the effort and time of running distributed tests while leading to more concrete conclusions than traditional testing.



It provides capabilities for device emulation  network shaping  , and handling of dependencies related to time, service status, or performance threshold. Moreover, \frisbee{} provides out-of-the-box monitoring packages for the Linux machines, databases, and applications we used during our experiments.





and out-of-the-box monitoring for numerous applications. 


\frisbee{} provides out-of-the-box monitoring packages for the Linux machines, databases, and applications we used during our experiments.

resource management,  network shaping and monitoring, 




.We usedCNSBenchto evaluate two cloud native storagebackends—OpenEBS and Ceph—and found several differences.For example, our evaluation shows that the maximum rate ofcontrol operations varies significantly across storage technologiesand configurations by a factor of up to 8.5×.Future work.We plan to work on extending the library of I/Oworkloads with I/O “kernels” that represent microservices, andalso improve the benchmark specification language to make thesyntax more concise and avoid having to duplicate sub-workloads.Further, we will work on collecting I/O and control operationtraces from production environments, analyze them, and createcorresponding profiles forCNSBench. Our longer term plansincluding finding and fixing performance bugs usingCNSBench,and even developing our own efficient storage solution.We hope our benchmark will be adopted by storage and cloudnative communities, and look forward to contributions.

 The  evaluation  of  emulation  accuracy  displayed  3-8%deviation  between  emulated  and  real  Infrastructures.  Finally,we presented two real-world IoT workloads that demonstratethe usability, extensibility, and observability of Fogify.Our future work includes an extensive scalability evaluation,which  is  currently  only  bounded  by  the  Fogify  Controllerwith  performance  impacted  by  the  number  of  Fogify  agents,emulated, and 



But by running the benchmark on Kubernetes, we ensure reproducibility of the results. This is something quite novel that is missing from the literature. Although many people run YCSB benchmarks, the servers may run on different hardware and therefore produce completely different results. Instead, by running Frisbee on strictly defined virtual resources, we ensure the same behavior across different deployments. 


Internal usage of \frisbee{} has been fruitful, and shows that can improve productivity ...

 The experiments were focused on the interplay of device capabilities, network distances, and placement strategies.

\textbf{Acknowledgement.} This work is supported by the EUCommission within the scope of ETHER 894204 (H2020-MSCA-IF-2019) project. 





%Because a\frisbee{} experiment may consist of multiple domain. Some of which can be physical and other virtual. For this reason, the \frisbee{} controller runs externally to the Kubernetes, so to  to be able interoperability with with multiple kubernetes clusters.  

-- extent frisbee from nodes to API 

location or group of locations. A location can be a cloud provider zone, a cloud provider region, racks, or a nodes. For the realization of this feature, we designed the \frisbee{} controller to run externally to the Kubernetes, so to be able interoperability across different Kubernetes clusters. 




 





top level of integration that enables centralized control over the experimental platform (Kubernetes containers remain autonomous and distributed).


This is particularly useful for mimicking high-load conditions without adding complexity to the experiment. Instead of adding numerous clients hoping to increase the load on servers, we can instead reduce the server resources at runtime. As a result, the experiments involve fewer objects, thus reducing the ramification of workload interference. 






This allows users to characterize remediation techniques (e.g., reactive vs. preventive), identify suboptimal approaches, and assess the recoverability of different systems in the presence of failures.


Another reason is to stop testing iterations if the metrics have converged to a stable value (e.g., by calculating the margin of error). In that case, we are confident that the collected sample reflects what we would expect to find had we run infinite amounts of tests. Thus, no further tests are needed, as they would only increase the overhead without compensating for additional knowledge.  


Fortunately, the need for observability is well understood. Many modern applications have built-in mechanisms for exposing their internal state directly into API calls. For example, key/value stores like Redis provide API calls for getting statistics concerning the number of keys, the role of every node in the cluster, the number of clients, the number of connections, etc. In this case, Telegraf queries the application API and collects those metrics. However, some applications do not have such mechanisms, or users are only interested in the external output. For example, in the YCSB benchmark, we are only interested in knowing the aggregated reports. 


For most cases, it avails to assume that a containerized application is ready to start accepting traffic shortly after the Pod has reached a Running phase. However, this is not always true. A Service may spend some time in warm-up (e.g., load data). Similarly, it is not safe to assume that a Running Pod always reflects a responsive application. For example, a Service experiencing a deadlock is unable to process requests, albeit it is still alive from the perspective of the Pod. 

our prototype to understand the behavior of a Redis key/value deployment, beyond its most common usage pattern. We opted for Redis due to its popularity, and because is not based on cloud-based service model, so we could install and test it locally, enabling repeatable results. These experiments are crafted to be representative, illustrate the usability of the system, and 


This can cause misleading and inconsistent results. 



However, this feature is still under development due to the race conditions caused by the parallel creation of services.









\subsection{Deployment}


\subsection{Dependencies}


\subsection{Topology Changes}


\subsection{Failures}


\subsection{Observability}


\subsection{Portability}

\subsection{Test-cases}




testing suites that aim to take humans out of the testing loop and reduce the testing time from human timescales to significantly faster machine timescales 




These problems have motivated the industry to create automated testing suites that stress system performance and configuration under various  operational conditions. [ CONTINUE WITH A/B testing, deployments suites, ...]. Unfortunately, most of these tools are either closed-source or specific to the ecosystem of the cloud vendor.




\textbf{Heterogeneity in Resources and Networks:}

%By definition, instrumented tests on Android are those that run on  physical devices or emulators. In these tests, the use of mocks is  reduced and we gain the advantage of using the actual implementation of  the Android framework, thus enabling the use of classes such as *SharedPreferences*, *Context*, *Parcelable* and *Intent*. A characteristic of this layer is that the tests 

In addition to the testing scale, challenges include: emulation of nodes with heterogeneous hardware and the the ability to control the link quality, such as latency, bandwidth,  error rate,  etc.,  and  even reproduce node-to-node and node-to-network connections.

* Cause bootleneck to appear errors
* Cost of ownership

Physical resources are replaced by virtual counterparts whose capabilities are well specified and therefore recreated amongst different Kubernetes deployments.


\textbf{Failure Injection:}
There are several Chaos Testing tools, like Chaos-Mesh, which we can use for fault injection. These tools typically consist of a high-level part for selecting fault parameters and a low-level part designed to cause (or simulate) faults at the targeted components.


    
    
%it is common when using tools like [Docker Compose](https://docs.docker.com/compose/) to depend on services in other linked containers, however oftentimes relying on [links](https://docs.docker.com/compose/compose-file/#links) is not enough - whilst the container itself may have *started*, the *service(s)* within it may not yet be ready - resulting in shell script hacks to work around race conditions.

Dockerize gives you the ability to wait for services 





\textbf{Observability:}
Although most modern systems, such as Redis, provide API for statistics, these statistics must be obtained at near real-time in order to understand how the systems evolves over time. 

A key feature of the Controller is that it goes beyond simple testing by supporting real-time monitoring of the distributed Services to facilitates assessment of the running deployments. 




\textbf{Event-driven testing:}

Use grafana to create alerts, and use those alerts to the \frisbee{} Controller


\textbf{Portability:}
Testing portability~\cite{tsai1996approach, wilson2002progress} is a critical topic that until now remains largely overlooked. It is not uncommon to spot two different papers in the literature whose authors use the same benchmark, the same deployment, and yet find that the published result variate significantly. The reason typically has to do with the experimentation platforms they use. Although the experimentation platforms can be documented and compared qualitatively, it is much harder to achieve repeatable results across different infrastructures. 

Since important decisions depend on reliable experimental data, it is necessary to enable reproducible experiments and verifiable results. To this end, experimental configurations and resource profiles are hosted on a version control systems. It is a central hub where the application developers or vendors share their experiments so that their users can use them to increase the resilience of the applications in production.

Infrastructure as code (IaC) is the process of managing and provisioning computer data centers through machine-readable definition files, rather than physical hardware configuration or interactive configuration tools.

The emulation execution environment should be scalable from topologies with a limited number of nodes, capable to run on a single laptop or PC, to hundreds or thousands nodes, running on a whole cluster.





\textbf{Rapid Application Deployment:}

Our aim is  to  provide  a  framework  that  goes  beyond  thecurrent  state-of-the-art  in  Fog  emulators  so  that  users  canemulate  key  aspects  of  Fog  environments  with  minimumeffort. Specifically, Fogify enables service operators to solelyfocus  on  the  evaluation  and  testing  of  their  services,  withsimplified  deployment  and  management  of  scalable  IoT  mi-croservices  on  top  of  the  emulated  environment.  


%there is the need for funneling metrics from distributed components, running concurrently on different machines, into a single monitoring pipeline.





the standardization of \faultload{}s would help to experiment with prescribed fault occurrences 
A promising idea is to use Kubernetes for . 


Our benchmark, called \frisbee{}, treats failures as first-class citizens and 




Because of this dynamic nature, the testing space can be so large that traditional testing methods cannot keep pace. 


, there are unknown behaviors that are difficult to plan for due to the dynamic nature of the software and the Cloud, and it’s hard to test against these abnormalities. 





Determinism is an essential property of an automated testing suite. Unfortunately, it is onerous to achieve identical conditions over different test runs ~\cite{leitner2016patterns, schad2010runtime, herbst2018quantifying}. Physical machines with different performance characteristics (e.g. disks, processors, or network interfaces), interference between co-located processes, or the execution of background tasks (e.g.,garbage collection, scrubbing), may lead to temporal variations that cause the obtained metrics to vary significantly. 

The long answer is that we need to perform some fundamental statistical analysis to calculate the confidence interval and the margin of error for the collected sample (of metrics). Suppose the error is below a given threshold. 








\textbf{Placement Policies}




Emerging applications may consist of hundreds of geographically distributed services that run over heterogeneous devices and spread across hundreds of physical networks. 















parent's watchdog captures the event 

and updates the parent's state accordingly. 

When the controller schedules an action with dependencies, it automatically creates a watchdog that waits for an event before executing the action. When the Pod comes into the desired phase, the watchdog fires an event that is subsequently captured by the controller, which determines what to do next. The watchdog takes advantage of Kubernetes TCP and HTTP  readiness probes to detect and remedy such situations. For TCP probes, the watchdog sends requests to the open ports of the Service (defined in the Service description) and blocks until it receives a reply. In this case, we are confident that the application is actually ready to accept traffic. HTTP probes work the same way but use HTTP endpoints instead of ports. 


 Equally for 


a parent (e.g, service group) will become \textit{Running} only when all of its children become \textit{Running}. Equally, the parent will become \textit{Completed} only if all of the children is complete. 

Every Action is a child to the Workflow, and every component created 

These dependencies create a  with the lifecycle of parent nodes depending on the lifecycle of their children. The Workflow is the root of the DAG. 


For example, 

on the state of their children.  Similarly, for 


Frisbee components follow a defined lifecycle that consists of states like Pending, Running, Completed, or Failed. Typically, this lifecycle transcribes to the lifecycle of Kubernetes pods hosting the application container. For example, if the application exits with an error code, 

To respect these dependencies, when the Frisbee controllers creates a new component, 

As was described previously, a Pod in Kubernetes followed a predefined lifecycled. 


The management of logical dependencies transcribes to the lifecycle of Kubernetes pods hosting the service container [21]. A pod follows a defined lifecyclestarting in the Pending phase, moving through the ‘run-ning’ phase when all of its containers are ready, and thenthrough either the ‘succeeded’ or ‘failed’ phases dependingon whether any container in the Pod terminated in failure














 shows the service template used for the creation of the above scenario.. 

.  The \textit{valueFrom} points to externally defined templates used to compose the Service structure. For example, the field [mon/system, mon/redis] represents the templates of two side services for monitoring the Redis servers. In the case of duplicate fields, the last reference takes effect. Local fields always take precedence over any reference. We must note that Code~\ref{code:service} depicts a compacted example. The actual language is somewhat more verbose and adheres to the conventions of the Kubernetes API, including keywords such as Kind, Metadata, and Specs.



Instead, Quarkus is intended for greenfield development of new applications, but allowing developers to preserve their Java skills and programming experience when moving into the world of cloud-native applications. But to do so requires those developers to have access to many of the code libraries and frameworks that have evolved around Java over the past 25 years to provide key business functions and services.






because the labeling happens automatically at the level of a service rather than the level of nodes, the placement constraints are portable over different Kubernetes clusters, without requiring to tag the cluster nodes.


A drawback of this approach is that if a label is not matched, the Service will remain in the Pending phase until an appropriate node is found. To cope with that, \frisbee{} provides the option either to block waiting for the Service to be scheduled, which may never happen, or abort the experiment after a grace period. 







The \frisbee{} language is designed to help developers when preparing tests of distributed applications. It offers the following main abstractions: 
\begin{enumerate*}
    \item \textbf{Service}: describes the properties of a containerized application;
    \item \textbf{Group}:  describes the logical grouping of related services;    
    \item \textbf{Domain}: defines placement constraints for a service; 
    \item \textbf{Topology}: represents one or more interconnected domains;
    \item \textbf{Workflow}: defines a sequence of actions that may change topology at runtime;
    \item \textbf{Deployment:} maps the topology into physical nodes.
\end{enumerate*}


Observability allows engineers to infer the internal states of a system by observing its external outputs. With observability, engineers can get a holistic view of how different services communicate, as well as how transactions flow between different services. 

pays particular attention to the \textbf{observability of the distributed system}. It




%When no labels are defined, the domain provides the means to capture the relationship between services in order to evaluate the effects of distributed and collocated placement strategies.


%Failure conditions can be defined on a per-domain basis. 

%Altering network-level QoS will affect the traffic between all services within a domain (e.g., bandwidth sharing). Link-level changes will affect the network traffic from services across different domains (e.g., add latency to represent geographical distance).

%This distinction primarily characterizes whether the resources specified in the service description will be used as placement constraints by the Kubernetes scheduler or will be emulated by \frisbee{}. 

%\paragraph{Topology Domain}
%A topology domain provides a convenient way to emulate the operating conditions of an actual geo-distributed environment, even on a single host. Our motivation is to evaluate IoT, Fog, and Edge services under realistic environment assumptions, faults, and uncertainties. We support three features for modeling a topology domain: network QoS, network link, and failure patterns. Altering network-level QoS will affect the traffic between all services within a domain (e.g., bandwidth sharing). Link-level changes will affect the network traffic from services across different domains (e.g., add latency to represent geographical distance). For the emulation of failure conditions, we inject faults that influence the operation of services and networks. This includes unexpected termination of services, network partitions, and packet drops. 








-- which lets designers standardize on a platform and avoid vendor lock-in. 


can conduct experiments to credibly answer questions such as: (i) Will the product respond in the desired manner when put into production? (ii) Can the product degrade gracefully when there is a sudden server crash, or a service component goes down, or some dependent services become unavailable? (iii) Can the product manage a sudden spike in user requests? To answer such questions, designers








At its core, Kubernetes is designed to deploy and operate applications in a microservices architecture. That includes spreading the application load across physical nodes, balancing requests across different instances, migrating instances to another host if there is a shortage of resources, and so on. In contrast, managing the lifecycle of an experiment requires a different set of capabilities, such as handling the logical dependencies between jobs, scheduling actions that will alter the runtime environment, and validate their impact. 








tools suffer from three main deficits: (i) they assume that the system is already up and running, (ii) they are unsuitable for adding new components in the experiment, (iii) they do not validate the effects of the fault  -- 


testing cloud-native applications remains challenging because of their scale and complexity. 
TiDB evolves, the testing scale multiplies. We have multiple fault scenarios, against which dozens of test cases run in the Kubernetes testing cluster. 

The problem is that Kubernetes is not natively designed to run experiments! 

\paragraph{Challenges}

We could consider using is a container-native workflow engine, such as Argo~\cite{argo},  to help schedule new containers and provide a `timeline' for the experiment. Unfortunately, this approach implements each step in a workflow as a container, making it unsuitable for scheduling Chaos events like bringing down a service or simulating a network partition. 
\CHECKnote{Check revised text about the use of a workflow engine.}

One solution is to interconnect these tools via shell scripts that manually bind the lifecycle of mock-up containers with actions in Chaos-Mesh. Even then, developers still have to extract system-wise or application-specific metrics that factor into the evaluation and perform automated checks for deviation from expected behavior.  More importantly, they are hardly efficient or portable since scripts run outside the Kubernetes cluster.




 %The testing of cloud-native applications is often based on the practitioner's experience and intuition rather than the systemic approach required by benchmarks. 


For example, benchmarking a database requires (i) deploy and run the servers (ii) load keys (iii) run queries. Performing these steps manually, or interactively, is time-consuming and inefficient. The same is true for solutions that are based on time intervals:  A better solution is to describe testing scenarios in a workflow programming model, that remains 



Like with all the the distributed application, designers of cloud-native have to pay attention to non-functional aspects such as performance, scalability, availability, fault tolerance, reliability, and resiliency.



    separating the modeling of testing scenarios from the instrumentation code. This enabl
    
    That includes specifications for actions sequences, execution conditions, and test cases of system metrics.



Model-based testing presents several advantages. In this way, tests can be based on what the software should do and not on what the software does (Apfelbaum and Doyle, 1997). In this context, the development of supporting tools is mandatory. This requires us to adapt to changes, review the traditional testing techniques, and include some new and modern ways to foresee, detect, respond, debug, analyze and report problems.




 Resilience is how well a system withstands such faults – a highly resilient system, for example, one built with loosely coupled microservices that can themselves be restarted and scaled easily, overcomes such faults without impacting users. C

. These microservices run on a containerized and dynamically orchestrated platform (with the help of technologies like Kubernetes, Docker, etc), in dynamic environments provided by cloud platforms (e.g., AWS, Azure, or GCP). 


Using a broad range of Chaos Engineering tools, inspection tools, and application benchmarks, systems designers can simulate abnormal system conditions to figure out how a system will respond in runtime uncertainties

. These uncertainties may occur at the client-side , the server-side (e.g., partition faults), or any combination thereof. 




With fail-fast disabled, the workflow will allow a service to run to completion (either success or failure), regardless of the failed outcomes of branches in the DAG.


A pod follows a defined lifecycle starting in the Pending phase, moving through the `running' phase when all of its containers are ready, and then through either the `succeeded' or `failed' phases depending on whether any container in the pod terminated in failure. When a pod changes phase, a respective event is fired and is subsequently captured by the controller. For example, the creation of YCSB loaders will be blocked until all Redis servers have come into a `running' phase. Similarly, the creation of YCSB runners will be blocked until the Loaders have reached the `succeeded' phase.  If a Pod reaches a state other than the expected (e.g., one of the loaders fail), the workflow applies a fail-fast policy to stop scheduling new services. Then it waits until all `running' services are completed before failing the workflow itself. 
To achieve that, 


%Over the last few years, research efforts are mainly focused on tools for testing Performance, Scalability, Deployment models, and Availability, to name a few. However, an important aspect that has not been thoroughly investigated yet is automation. 
